A Cubic Regularization Approach for Finding Local Minimax Points in Nonconvex Minimax Optimization

Gradient descent-ascent (GDA) is a widely used algorithm for minimax optimization. However, GDA has been proved to converge to stationary points for nonconvex minimax optimization, which are suboptimal compared with local minimax points. In this work, we develop cubic regularization (CR) type algorithms that globally converge to local minimax points in nonconvex-strongly-concave minimax optimization. We first show that local minimax points are equivalent to second-order stationary points of a certain envelope function. Then, inspired by the classic cubic regularization algorithm, we propose an algorithm named Cubic-LocalMinimax for finding local minimax points, and provide a comprehensive convergence analysis by leveraging its intrinsic potential function. Specifically, we establish the global convergence of Cubic-LocalMinimax to a local minimax point at a sublinear convergence rate and characterize its iteration complexity. Also, we propose a GDA-based solver for solving the cubic subproblem involved in Cubic-LocalMinimax up to certain pre-defined accuracy, and analyze the overall gradient and Hessian-vector product computation complexities of such an inexact Cubic-LocalMinimax algorithm. Moreover, we propose a stochastic variant of Cubic-LocalMinimax for large-scale minimax optimization, and characterize its sample complexity under stochastic sub-sampling. Experimental results demonstrate faster convergence of our stochastic Cubic-LocalMinimax than some existing algorithms.

==> 20230217 CubicMinimax_ArXiV_underTMLRreview/assumption1.tex <==
\section{Proof of the relationship among the statements in Assumption 1}\label{sec_assum1}

We will prove that in \Cref{assum: f}, the item 2 and the statement that $g$ is lower semi-continuous can be derived from the rest of \Cref{assum: f}. 
\begin{proof}
	\noindent Since the sub-level set $\{x: (\Phi+g)(x)\le\alpha\}$ is closed, $\Phi+g$ is lower semi-continuous. Without item 2 and any assumption on $g$, Lemma \Cref{prop_Phiystar} holds which implies continuity of $\Phi$, so $g$ is lower semi-continuous.  
	
	%\noindent If the sub-level set $A=\{x: (\Phi+g)(x)\le0 \}$ is empty, then 0 is a lower bound of $\Phi+g$. Hence, we focus on the case where $A$ is non-empty convex set.\\
	
	\noindent Suppose $\Phi+g$ is not bounded below, then there is a sequence $\{x_t\}_t$ such that $(\Phi+g)(x_t)\le -t$. Since $x_t\in A$ and $A$ is compact, $\{x_n\}$ has at one convergent subsequence $x_{n(t)}\overset{t}{\to} x^*$. Since $\Phi+g$ is lower semi-continuous, $\Phi(x^*)+g(x^*)\le \mathop{\lim\inf}_{n\to\infty} \Phi(x_{n(t)})+g(x_{n(t)})=-\infty$. However, since $\Phi$ is continuous and $g$ is proper, $\Phi(x^*), g(x^*)>-\infty$, is a contradiction. Hence, $\Phi+g$ is not bounded below, that is, the item 2 of \Cref{assum: f} holds
\end{proof}

==> 20230217 CubicMinimax_ArXiV_underTMLRreview/coro1proof.tex <==



==> 20230217 CubicMinimax_ArXiV_underTMLRreview/experiments.tex <==
In this section, we do empirical studies contrasting our algorithm with the classical GDA algorithm on both synthetic problem and real-world application.

\subsection{Synthetic Minimax Problem}

We construct the following nonconvex-strongly-concave minimax problem:
\[
f_i(\textbf{x,y}) = w(x_3) - \frac{y_1^2}{40} + A_i x_1 y_1 - \frac{5y_2^2}{2} + B_i x_2 y_2
\]

where $A_i$ and $B_i$ are independent random variables from uniform distribution range from 0.5 to 1.5, $N=1000$ is the number of total sample,
$w(.)$ is W-shaped scalar functions whose exact form is shown in Appendix.
Then we consider the minimax problem with such expression below:
\begin{equation}
    \min\limits_{\textbf{x} \in \mathcal{R}^3} \max\limits_{\textbf{y} \in \mathcal{R}^2} f(\textbf{x,y}) =  \min\limits_{\textbf{x} \in \mathcal{R}^3} \max\limits_{\textbf{y} \in \mathcal{R}^2} \frac{1}{N}\sum^N_{i=1} f_i(\textbf{x,y})
\end{equation}

We first set initial point at $\textbf{x}=[0,0,1]^T$ and $\textbf{y}=[1,1]^T$, compare the different performance on batchsize 20,100,500.  

\begin{figure}[htbp]

\centering
\includegraphics[width=0.95\linewidth]{emsnewsletter-template/pictures/batchsize-contrast.png}

\caption{stochastic cubic GDA on different batchsize}\label{result1}
	
\end{figure}

Trough Figure 1 we can obviously see that stochastic cubic GDA can have a good performance on a small mini batch, which means we could do descent on a small mini-step and have a faster converge speed and lower total sample size.

Second we contrast stochastic cubic gda with stochastic gda under same initial point $\textbf{x}=[0,0,1]^T$ and $\textbf{y}=[1,1]^T$, with same batch-size = 100 and same learning rate $lr = 0.01$ at descent step.

\begin{figure}[htbp]

\centering
\includegraphics[width=0.95\linewidth]{emsnewsletter-template/pictures/cubic vs gda.png}

\caption{comparison $\Phi(x)$ of cubic GDA and classical GDA }\label{result1}
	
\end{figure}

Figure 2 shows stochastic cubic GDA has a obvious faster speed of convergence over classical GDA. It needs shorter time and less sample size to reach the minimax point, which illustrates cubic method really works. 

\subsection{Neural network simulation}

This section we compare the stochastic cubic GDA with the classical GDA using the example of a convolutional neural network. All these algorithms have a single-loop structure.

We decide to solve problem below using the MINST dataset.

\begin{equation}
    \min\limits_{\theta} \max\limits_{ \{ \xi_i \}_{i=1}^n} \frac{1}{n} \sum_{i=1}^n 
    \left[ \ell (h_{\theta} (\xi_i, y_i) ) - \lambda \Vert \xi_i - x_i \Vert^2 \right]
\end{equation}

where $n = 60k$ is the number of training samples, $\theta$ is the parameter of the neural network
and $(x_i, y_i)$ corresponds to the i-th image and label, respectively, $\xi_i$ refers to the adversarial sample corresponding to $x_i$, we choose cross-entropy loss function as $\ell$.

We set $\lambda$ = 2.0 that suffices to make the maximization part be strongly-concave. The network model we use is a convolution network that consists of two convolution blocks followed by two fully connected layers. Specifically, each convolution block contains a convolution layer, a max-pooling layer with stride step 2, and a ReLU activation layer. The convolution layers in the two blocks have 1, 10 input channels and 10, 20 output channels, respectively, and both of them have kernel size 5, stride step 1 and no padding. The two fully connected layers have input dimensions 320, 50 and output dimensions 50, 10, respectively.

In both algorithm, we randomly select a mini-batch with 512 size to do optimization. In validation step we randomly select 2000 images and labels as the test set. The learning rate of the ascent step in both algorithm is 0.1 and both do 20 steps of gradient ascend before do descend in each epoch. The descend learning rate in both algorithms is 0.01, while in stochastic cubic GDA we only do one step of cubic descend, in classical GDA we do 10 steps of gradient descend in each epoch. We use efficiency algorithm in this paper to estimate the cubic function, and the learning rate in solving the cubic problem is 0.1 and 0.001, respectively. Since it may be hard to evaluate the exact value of $\Phi(x)$, we run 100 gradient ascent steps to make $\xi$ close to the maximum and compute the loss as estimated $\Phi(x)$.

\begin{figure}[htbp]

\centering
\includegraphics[width=1\linewidth]{emsnewsletter-template/pictures/cubic vs gda2.png}

\caption{Left: comparison $\Phi(x)$ of three algorithms Right: comparison of robust test accuracy of three algorithms}\label{result2}
	
\end{figure}

Figure 3 (Left) compares the estimated objective function value achieved by both algorithms. It can be seen that cubic algorithm has a manifest superiority on the convergence over the other algorithm and is significantly faster. Figure 3 (Right) further demonstrates the advantage of stochastic cubic in robust test accuracy. It can be seen that the robust model trained by cubic method achieves a better robustness.

==> 20230217 CubicMinimax_ArXiV_underTMLRreview/intro.tex <==
\section{Introduction}
Minimax optimization (a.k.a.\! two-player sequential zero-sum games) is a popular modeling framework that has broad applications in modern machine learning, including game theory \citep{ferreira2012minimax}, generative adversarial networks \citep{goodfellow2014generative}, adversarial training \citep{Sinha2017CertifyingSD}, reinforcement learning \citep{qiu2020single,ho2016generative,MultiAgent_Jiaming}, etc. A standard minimax optimization problem is shown below, where $f$ is a smooth bivariate function.
\begin{align}
	\min_{x\in \mathbb{R}^m}\max_{y\in \mathbb{R}^n}~ f(x,y). \tag{P}
\end{align} 
In the existing literature, many optimization algorithms have been developed to solve different types of minimax problems. Among them, a simple and popular algorithm is the gradient descent-ascent (GDA), which alternates between a gradient descent update on $x$ and a gradient ascent update on $y$ in each iteration. Specifically, the global convergence of GDA has been established for minimax problems under various types of global geometries, such as convex-concave-type geometry ($f$ is convex in $x$ and concave in $y$) \citep{nedic2009subgradient,du2019linear,mokhtari2020unified,zhang2020suboptimality}, bi-linear geometry \citep{neumann1928theorie,robinson1951iterative} and Polyak-{\L}ojasiewicz geometry \citep{nouiehed2019solving,yang2020global}, yet these geometries are not satisfied by general nonconvex minimax problems in modern machine learning applications.  
Recently, many studies proved the convergence of GDA in nonconvex minimax optimization for both nonconvex-concave problems \citep{lin2019gradient,nouiehed2019solving,xu2020unified} and nonconvex-strongly-concave problems \citep{lin2019gradient,xu2020unified,chen2021proximal}.
{In these studies, it has been shown that GDA converges sublinearly to a stationary point where the gradient of an envelope-type function $\Phi(x):=\max_y f(x,y)$ vanishes.}

Although GDA can find stationary points in nonconvex minimax optimization, the stationary points may include candidate solutions that are far more sub-optimal than global minimax points. However, finding global minimax points is in general NP-hard \citep{jin2019local}. Recently, \cite{jin2019local} proposes a notion of local minimax point that is computationally tractable and is close to global minimax point. Specifically, a local minimax point $(x, y)$ is a stationary point that satisfies the following second-order non-degeneracy conditions (see  \Cref{def: local} for the formal definition). 
\begin{align*}
    \nabla_{\!22} f(x, \!y) \prec \zero, ~\big[\nabla_{\!11} f - \nabla_{\!12} f (\nabla_{\!22} f)^{-1} \nabla_{\!21} f\big](x,\!y) \succeq \zero.
\end{align*}

In the existing literature, several studies have proposed Newton-type GDA algorithms for finding such local minimax points. Specifically, \cite{Wang2020follow} proposed a Follow-the-Ridge (FR) algorithm, which is a variant of GDA that applies a second-order correction term to the gradient ascent update. In particular, the authors showed that any strictly stable fixed point of
FR is a local minimax point, and vice versa.  In another work \citep{zhang2021newtontype}, the authors proposed two Newton-type GDA algorithms that are proven to locally converge to a local minimax point at a linear and super-linear convergence rate, respectively. However, these second-order-type GDA algorithms only have asymptotic convergence guarantees that require initializing sufficiently close to a local minimax point, and they do not have any global convergence guarantees. 
Therefore, we are motivated to ask the following fundamental questions.
 \begin{itemize}[leftmargin=*,topsep=0pt]
 	\item {\bf Q:} {\em Can we develop globally convergent {GDA-type} algorithms that can efficiently find local minimax points in nonconvex minimax optimization? What are their convergence rates and complexities?}
 \end{itemize}

%Developing and analyzing such an algorithm is nontrivial due to the following reasons: 1) we need to have a good understanding and characterization of both the first-order and second-order information of nonconvex minimax problems; 2) we need to develop a computationally feasible and efficient GDA algorithm that can leverage the local curvature of the function to escape saddle points; 3) we aim to develop a unified analysis framework that can characterize the convergence rate of this algorithm under different types of nonconvex geometry of the minimax problem. 


In this work, we provide comprehensive answers to these questions. We develop deterministic and stochastic {Newton-type GDA} algorithms that globally converge to local minimax points in nonconvex-strongly-concave minimax optimization, and study their convergence rates and sample complexities under standard assumptions. We summarize our contributions as follows.

%\vspace{1mm}
\subsection{Our Contributions}
%\vspace{1mm}
We consider the standard minimax optimization problem (P), where $f$ is twice-differentiable with Lipschitz continuous gradient and Hessian, and is nonconvex-strongly-concave. In this setting, we first show that local minimax points of $f$ are equivalent to second-order stationary points of the
envelope function $\Phi(x):=\max_{y\in \mathbb{R}^n} f(x,y)$. Then, inspired by the classic cubic regularization algorithm, we propose a {cubic-regularized GDA} (named Cubic-GDA) algorithm to find local minimax points. The algorithm uses gradient ascent to update $y$, which is then used to estimate the gradient and Hessian involved in the cubic regularization update for $x$ (see \Cref{algo: prox-minimax} for more details).

%Specifically, we propose Cubic-GDA -- a \red{Newton-type GDA} algorithm that leverages the classical cubic regularization technique to escape saddle points. Different from the standard cubic regularization algorithm that uses the Hessian information of the function, the Hessian of $\Phi(x)$ is not directly available in nonconvex minimax optimization, and hence we develop a rigorous and computationally feasible scheme in Cubic-GDA to estimate the Hessian. 

\textbf{Global convergence.} We show that Cubic-GDA admits an intrinsic potential function $H_t$ (see \Cref{prop: lyapunov}) that monotonically decreases over the iterations. Based on this property, we prove that every limit point of $\{x_t\}_t$ generated by Cubic-GDA is a local minimax point. Moreover, to achieve an $\epsilon$-accurate local minimax point, Cubic-GDA requires $\mathcal{O}\big(\kappa^{1.5}\epsilon^{-3}\big)$ number of cubic updates and $\mathcal{O}\big(\kappa^{2.5}\epsilon^{-3}\big)$ number of gradient ascent updates, where $\kappa>1$ denotes the problem condition number. 

\textbf{Asymptotic convergence.} By leveraging the potential function, we also characterize the asymptotic convergence rates of Cubic-GDA under a class of {\L}ojasiewicz-type local gradient geometry. Specifically, depending on the sharpness parameter of the local geometry, the asymptotic convergence rate of Cubic-GDA ranges from sub-linear convergence to super-linear convergence. These asymptotic convergence rates are orderwise faster than those of the standard GDA established in \citep{chen2021proximal} under the same type of local geometry. 
%\footnote{Note that the geometry parameter $\theta$ in this paper corresponds to $\frac{1}{1-\theta}$ in \citep{chen2021proximal}.}. 

\textbf{Sample complexity.} We further develop a stochastic variant of Cubic-GDA that applies sub-sampling to improve the sample complexity in large-scale minimax optimization. In particular, we adopt time-varying batch sizes in a way such that the induced gradient inexactness and Hessian inexactness are adapted to the optimization increment $\|x_t - x_{t-1}\|$ in the previous iteration. Consequently, to achieve an $\epsilon$-accurate local minimax point, we show that stochastic Cubic-GDA requires querying $\widetilde{\mathcal{O}}\big(\kappa^{3.5}\epsilon^{-7}\big)$ number of gradient samples and $\widetilde{\mathcal{O}}\big(\kappa^{2.5}\epsilon^{-5}\big)$ number of Jacobian samples.

%\vspace{-2mm}
% \begin{table}[ht]
% 	\caption{\red{Move to KL section.} Comparison of potential function value gap $H(z) - H^*$ convergence rates of Cubic-GDA and GDA under different parameterizations of {\L}ojasiewicz gradient geometry.}\label{table: 1}
% 	\center
% 	\vspace{0mm}
% 	\begin{tabular}{ccc}
% 		\toprule
% 		{Geometry parameter} & {GDA \citep{chen2021proximal}} & {\bf Cubic-GDA (This paper)} \\ \midrule
% 		$\theta\in(2,+\infty)$   &\makecell{ Super-linear convergence} & \makecell{Super-linear convergence}   \\
% 		\midrule
% 		$\theta=2$  & \makecell{Linear convergence} & \makecell{ Super-linear convergence}  \\
% 		\midrule
% 		$\theta \in (\frac{3}{2}, 2)$  & \makecell{Sub-linear convergence} & \makecell{Super-linear convergence}  \\
% 		\midrule
% 		$\theta = \frac{3}{2}$  & \makecell{Sub-linear convergence}& \makecell{Linear convergence} \\
% 		\midrule
% 		$\theta \in (1,\frac{3}{2})$  & \makecell{Sub-linear convergence}& \makecell{Sub-linear convergence} \\
% 		\bottomrule
% 	\end{tabular}
% \vspace{-2mm}
% \end{table}

\subsection{Other Related Work}\label{sec: related_work}
%\vspace{-2mm}
\textbf{Deterministic GDA algorithms:}
% \red{Many studies characterized the convergence of GDA in nonconvex minimax optimization. Specifically,
%  \cite{lin2019gradient,nouiehed2019solving,xu2020unified} studied the convergence of GDA in the nonconvex-concave setting whereas \cite{lin2019gradient,xu2020unified} focused on the nonconvex-strongly-concave setting. 
%  In these general nonconvex settings, it is shown that GDA converges to a certain stationary point at a sublinear rate. Recently, \cite{chen2021proximal}
%  proved the parameter convergence of proximal-GDA in regularized nonconvex-strongly-concave optimization under the Kurdyka-{\L}ojasiewicz geometry. The convergence rates obtained there are orderwise slower than that of Cubic-GDA.}
\cite{yang2020global} studied an alternating gradient descent-ascent (AGDA) algorithm in which the gradient ascent step uses the current variable $x_{t+1}$ instead of $x_t$. \cite{xu2020unified} studied an alternating gradient projection algorithm which applies $\ell_2$ regularizer to the local objective function of GDA followed by projection onto the constraint sets. \cite{daskalakis2018limit,mokhtari2020unified,zhang2020suboptimality} analyzed optimistic gradient descent-ascent (OGDA) which applies negative momentum to accelerate GDA. \cite{mokhtari2020unified} also studied an extra-gradient algorithm which applies two-step GDA in each iteration. \cite{nouiehed2019solving} studied multi-step GDA where multiple gradient ascent steps are performed, and they also studied the momentum-accelerated version.  \cite{cherukuri2017saddle,daskalakis2018limit,jin2019local} studied GDA in continuous time dynamics using differential equations. \cite{adolphs2019local} analyzed a second-order variant of the GDA algorithm. 
In a concurrent work \citep{luo2021finding}, the authors proposed a Minimax Cubic-Newton algorithm that is similar to our Cubic-GDA but adopts a different output rule. {Specifically, in iteration $t$, they terminate the algorithm based on the current increment $\|s_{t+1}\|$. As a comparison, our Output II terminates the algorithm based on $\|s_t\|\vee \|s_{t+1}\|$. This output rule is critical to develop the practical and adaptive sub-sampling scheme for our stochastic Cubic-GDA. 
In addition, we also analyze the last-iterate convergence of Cubic-GDA with Output I. Moreover, we develop a stochastic version of Cubic-GDA and analyze its sample complexity.}

%They characterize the computation complexity under a special type of inexactness that approximates the inverse Jacobian using matrix Chebyshev polynomials. As a comparison, this study focuses on analyzing the global and local convergence properties of Cubic-GDA.

% 1.  We also study last-iterate convergence; output II is different, helps develop practical stochastic sampling scheme later

% 2. Analysis is based on potential function, 

% 3. We also study stochastic version


\textbf{Stochastic GDA algorithms: } \cite{lin2019gradient,yang2020global} analyzed stochastic GDA and stochastic AGDA, which are direct extension of GDA and AGDA to the stochastic setting. Variance reduction techniques have been applied to stochastic minimax optimization, including SVRG-based \citep{du2019linear,yang2020global}, SPIDER-based \citep{xu2020gradient}, SREDA \citep{xu2020enhanced}, STORM \citep{qiu2020single} and its gradient free version \citep{huang2020accelerated}. \cite{xielower} studied the complexity lower bound of first-order stochastic algorithms for finite-sum minimax problem.



\textbf{Cubic regularization (CR):} {The CR algorithm dates back to \citep{Griewank}, where global convergence is established.} In \cite{Nesterov2006}, the author analyzed the convergence rate of CR to second-order stationary points in nonconvex optimization. In \citep{Nesterov2008}, the authors established the sub-linear convergence of CR for solving convex smooth problems, and they further proposed an accelerated version of CR with improved sub-linear convergence. \cite{Yue2018} studied the asymptotic convergence properties of CR under the error bound condition, and established the quadratic convergence of the iterates. 
%{Recently, \cite{Hallak2020} proposed a framework of two directional method for finding second-order stationary points in general smooth nonconvex optimization. The main idea is to search for a feasible direction toward the solution and is not based on cubic regularization.}
Several other works proposed different methods to solve the cubic subproblem of CR, e.g., \citep{Agarwal2017,Carmon2016,Cartis2011a}.
Another line of work aimed at improving the computation efficiency of CR by solving the cubic subproblem with inexact gradient and Hessian information. In particular, \cite{Saeed2017} proposed an inexact CR for solving convex problem. Also, \cite{Cartis2011b} proposed an adaptive inexact CR for nonconvex optimization, whereas \cite{Jiang2017} further studied the accelerated version for convex optimization. Several studies explored subsampling schemes to implement inexact CR algorithms, e.g., \citep{kohler2017,Xu2017,Zhou2018,Wang2018}. 




==> 20230217 CubicMinimax_ArXiV_underTMLRreview/introduction_unused.tex <==
\section{Introduction}
A majority of machine learning applications are naturally formulated as nonconvex optimization due to the complex mechanism of the underlying model. Typical examples include training neural networks in deep learning \cite{Goodfellow2016}, low-rank matrix factorization \cite{RongGe2016,Bhojanapalli2016}, phase retrieval \cite{Candes2015,Zhang2017}, etc. In particular, these machine learning problems take the generic form
\begin{align*}
\min_{\xb\in \RR^d}~~f(\xb), \tag{P}
\end{align*}
where the objective function $f: \RR^d \to \RR$ is a differentiable and nonconvex function, and usually corresponds to the total loss over a set of data samples. 
Traditional first-order algorithms such as gradient descent can produce a solution $\bar{\xb}$ that satisfies the first-order stationary condition, i.e., $\nabla f (\bar{\xb}) = \zero$. However, such first-order stationary condition does not exclude the possibility of approaching a saddle point, which can be a highly suboptimal solution and therefore deteriorate the performance. 

Recently in the machine learning community, there has been an emerging interest in designing algorithms to scape saddle points in nonconvex optimization, and one popular algorithm is the cubic-regularized Newton's algorithm \cite{Nesterov2006,Agarwal2017,Yue2018}, which is also referred to as cubic regularization (CR) for simplicity. Such a second-order method exploits the Hessian information and produces a solution $\bar{\xb}$ for problem (P) that satisfies the second-order stationary condition, i.e., 
$$(\text{second-order stationary}):\quad \nabla f (\bar{\xb}) = \zero, ~\nabla^2 f(\bar{\xb}) \succeq \zero.$$
The second-order stationary condition ensures CR to escape saddle points wherever the corresponding Hessian matrix has a negative eigenvalue (i.e., strict saddle points \cite{Sun2015}). In particular, many nonconvex machine learning problems have been shown to exclude spurious local minima and have only strict saddle points other than global minima \cite{Baldi1989,Sun2017,RongGe2016,zhou2018}. In such a desirable case, CR is guaranteed to find the global minimum for these nonconvex problems. 
To be specific, given a proper parameter $M>0$, CR generates a variable sequence $\{ \xb_{k}\}_k$ via the following update rule
\begin{align}
	\text{(CR)}~ \xb_{k+1} \in \argmin_{\yb \in \RR^d} ~\inner{\yb - \xb_{k}}{\nabla f (\xb_{k})} + \frac{1}{2} (\yb - \xb_{k})^\ttop \nabla^2 f(\xb_{k})  (\yb - \xb_{k}) + \frac{M}{6} \|\yb - \xb_{k}\|^3. \label{eq: CR}
\end{align}
Intuitively, CR updates the variable by minimizing an approximation of the objective function at the current iterate. This approximation is essentially the third-order Taylor's expansion of the objective function. We note that computationally efficient solver has been proposed for solving the above cubic subproblem \cite{Agarwal2017}, and it was shown that the resulting computation complexity of CR to achieve a second-order stationary point serves as the state-of-the-art among existing algorithms that achieve the second-order stationary condition.
%is lower than that of gradient descent to achieve a first-order stationary point.

Several studies have explored the convergence of CR for nonconvex optimization. Specifically, the pioneering work \cite{Nesterov2006} first proposed the CR algorithm and showed that the variable sequence $\{\xb_{k} \}_k$ generated by CR has second-order stationary limit points and converges sub-linearly. Furthermore, the gradient norm along the iterates was shown to converge quadratically (i.e., super-linearly) given an initialization with positive definite Hessian. Moreover, the function value along the iterates was shown to converge super-linearly under a certain gradient dominance condition of the objective function. Recently, \cite{Yue2018} studied the asymptotic convergence rate of CR under the local error bound condition, and established the quadratic convergence of the distance between the variable and the solution set. 
Clearly, these results demonstrate that special geometrical properties (such as the gradient dominance condition and the local error bound) enable much faster convergence rate of CR towards a second-order stationary point. However, these special conditions may fail to hold for generic complex objectives involved in practical applications. Thus, it is desired to further understand the convergence behaviors of CR for optimizing nonconvex functions over a broader spectrum of geometrical conditions.

The Kurdyka-{\L}ojasiewicz (K{\L}) property (see \Cref{sec: pre} for details) \cite{Bolte2007,Bolte2014} serves as such a candidate. As described in \Cref{sec: pre}, the \KL property captures a broad spectrum of the local geometries that a nonconvex function can have and is parameterized by a parameter $\theta$ that changes over its allowable range.  In fact, the \KL property has been shown to hold ubiquitously for most practical functions (see \Cref{sec: pre} for a list of examples). 
The \KL property has been exploited extensively to analyze the convergence rate of various {\em first-order} algorithms for nonconvex optimization, e.g., gradient method \cite{Attouch2009,Li2017}, alternating minimization \cite{Bolte2014} and distributed gradient methods \cite{Zhou2016}.
But it has not been exploited to establish the {\em convergence rate} of second-order algorithms towards second-order stationary points.  
In this paper, we exploit the \KL property of the objective function to provide a comprehensive study of the convergence rate of CR for nonconvex optimization. We anticipate our study to substantially advance the existing understanding of the convergence of CR to a much broader range of nonconvex functions. We summarize our contributions as follows.
\vspace{-5pt}
\subsection{Our Contributions}
\vspace{-5pt}
We characterize the convergence rate of CR locally towards second-stationary points for nonconvex optimization under the \KL property of the objective function. Our results also compare and contrast the different order-level of guarantees that \KL yields between the first and second-order algorithms.
Also, our analysis characterizes the convergence property for a range of \KL parameter $\theta$,  which requires the development of different recursive inequalities for various cases.

\textbf{Gradient norm \& least eigenvalue of Hessian:}
We characterize the asymptotic convergence rates of the sequence of gradient norm $\{\|\nabla f(\xb_{k})\| \}_k$ and the sequence of the least eigenvalue of Hessian $\{\lambda_{\min} (\nabla^2 f(\xb_{k}))\}_k$ generated by CR. We show that CR meets the second-order stationary condition at a (super)-linear rate in the parameter range $\theta \in [\frac{1}{3}, 1]$ for the \KL property, while the convergence rates become sub-linearly in the parameter range $\theta \in (0, \frac{1}{3})$ for the \KL property.

\textbf{Function value gap \& variable distance:} 
We characterize the asymptotic convergence rates of the function value sequence $\{f(\xb_{k})\}_k$ and the variable sequence $\{\xb_{k}\}_k$ to the function value and the variable of a second-order stationary point, respectively. The obtained convergence rates range from sub-linearly to super-linearly depending on the parameter $\theta$ associated with the \KL property. Our convergence results generalize the existing ones established in \cite{Nesterov2006} corresponding to special cases of $\theta$ to the full range of $\theta$. Furthermore, these types of convergence rates for CR are orderwise faster than the corresponding convergence rates of the first-order gradient descent algorithm in various regimes of the \KL parameter $\theta$ (see \Cref{table: 1} and \Cref{table: 2}  for the comparisons). 

Based on the \KL property, we establish a generalized local error bound condition (referred to as the \KL error bound). The \KL error bound further leads to characterization of the convergence rate of distance between the variable and the solution set, which ranges from sub-linearly to super-linearly depending on the parameter $\theta$ associated with the \KL property.
This result generalizes the existing one established in \cite{Yue2018} corresponding to a special case of $\theta$ to the full range of $\theta$. 


\vspace{-5pt}
\subsection{Related Work}
\vspace{-5pt}
\textbf{Cubic regularization:} CR algorithm was first proposed in \cite{Nesterov2006}, in which the authors analyzed the convergence of CR to second-order stationary points for nonconvex optimization. In \cite{Nesterov2008}, the authors established the sub-linear convergence of CR for solving convex smooth problems, and they further proposed an accelerated version of CR with improved sub-linear convergence. Recently, \cite{Yue2018} studied the asymptotic convergence properties of CR under the error bound condition, and established the quadratic convergence of the iterates. Several other works proposed different methods to solve the cubic subproblem of CR, e.g., \cite{Agarwal2017,Carmon2016,Cartis2011a}.


\textbf{Inexact-cubic regularization:} 
Another line of work aimed at improving the computation efficiency of CR by solving the cubic subproblem with inexact gradient and Hessian information. In particular, \cite{Saeed2017,Jin2017} proposed an inexact CR for solving convex problem and nonconvex problems, respectively. Also, \cite{Cartis2011b} proposed an adaptive inexact CR for nonconvex optimization, whereas \cite{Jiang2017} further studied the accelerated version for convex optimization. Several studies explored subsampling schemes to implement inexact CR algorithms, e.g., \cite{kohler2017,Xu2017,Zhou2018,Wang2018}. 


\textbf{\KL property:} The \KL property was first established in \cite{Bolte2007}, and was then widely applied to characterize the asymptotic convergence behavior for various first-order algorithms for nonconvex optimization \cite{Attouch2009,Li2017,Bolte2014,Zhou2016,Zhou_2017a}. The \KL property was also exploited to study the convergence of second-order algorithms such as generalized Newton's method \cite{Frankel2015} and the trust region method \cite{Noll2013}. However, these studies did not characterize the convergence rate and the studied methods cannot guarantee to converge to second-order stationary points, whereas this paper provides this type of results.

\textbf{First-order algorithms that escape saddle points:} Many first-order algorithms are proved to achieve second-order stationary points for nonconvex optimization. For example, online stochastic gradient descent \cite{Ge2015}, perturbed gradient descent \cite{Jin2017}, gradient descent with negative curvature \cite{Carmon2016,Liu2017} and other stochastic algorithms \cite{Zhu2017}.



==> 20230217 CubicMinimax_ArXiV_underTMLRreview/jacobian.tex <==
\section{Compute Jacobian-Vector Product}\label{app: jacob}

In \Cref{algo: prox-minimax} (and similarly for \Cref{algo: prox-minimax-stoc}), the key step is the cubic regularization update, which requires solving the following generic cubic sub-problem.
\begin{align*}
    \mathop{\arg\!\min}_s \nabla_{1}f(x, y)^{\top}s + \frac{1}{2} s^{\!\top}G(x, y)s+\frac{1}{6\eta_x}\|s\|^3, ~~\text{where}~~G(x, y) = \big[\nabla_{11} f - \nabla_{12} f (\nabla_{22} f)^{-1} \nabla_{21} f\big](x,y).
\end{align*}
In the literature, many gradient-based cubic-solvers have been developed to efficiently solve cubic sub-problems, and their convergence guarantee and computation complexity are well established \citep{Carmon2016,Tripuraneni18}. In particular, when implementing these cubic-solvers to solve the above cubic sub-problem, one needs to query the Hessian-vector product $G(x,y)\cdot u$ for a general vector $u$. This quantity can be efficiently computed as we elaborate below. 

First, note that for any vector $v$, the Jacobian-vector products $\nabla_{k\ell} f(x,y)\cdot v$ for all $k,\ell\in\{1,2\}$ can be computed via standard auto-differentiation as follows
\begin{align*}
    \nabla_{k\ell} f(x,y)\cdot v = \nabla_\ell\big(\nabla_k f(x,y)^\top v\big), \quad \forall k,\ell\in\{1,2\}.
\end{align*}
Therefore, we can query the above Jacobian-vector product oracle to compute 
\begin{align*}
    z_{1} := \nabla_{11} f(x,y)\cdot u, \quad z_{2} := \nabla_{21} f(x,y)\cdot u.
\end{align*}
Then, we have  $G(x,y)\cdot u = z_{1} - \big[\nabla_{12} f (\nabla_{22} f)^{-1}\big](x,y)\cdot z_{2}$. Note that the quantity $z_{3} := (\nabla_{22} f(x,y))^{-1}\cdot z_{2}$ can be computed by solving the linear system 
\begin{align*}
    \nabla_{22} f(x,y)\cdot z_{3} = z_{2}
\end{align*}
using standard conjugate gradient solvers. Lastly, we query another Jacobian-vector product oracle to compute 
\begin{align*}
    z_{4}:=\nabla_{12} f(x,y)\cdot z_{3}.
\end{align*}
Finally, the Hessian-vector product can be computed as $G(x,y)\cdot u = z_{1} - z_{4}$.

==> 20230217 CubicMinimax_ArXiV_underTMLRreview/preliminary.tex <==
{\bf Notation:} For a bivariate function $f(x,y)$, we denote $\nabla_1 f, \nabla_2 f$ as the partial gradients with respect to the first and the second input arguments of $f$, respectively. We also denote the Jacobian blocks with regard to the two input arguments as $\nabla_{11} f, \nabla_{22} f, \nabla_{12} f, \nabla_{21} f$. We denote the $\max$ and $\min$ operators as $\vee$ and $\wedge$, respectively.

\section{Problem Formulation and Preliminaries}\label{sec: pre}

We consider the following standard minimax optimization problem (P), where $f$ is a nonconvex-strongly-concave bivariate function and is twice-differentiable. Throughout the paper, we define the envelope function $\Phi(x):=\max_{y\in \mathbb{R}^n} f(x,y)$.
\begin{align}
	\min_{x\in \mathbb{R}^m}\max_{y\in \mathbb{R}^n}~ f(x,y). \tag{P}
\end{align} 
Our goal is to develop algorithms that globally converge to local minimax points of (P), which are defined to satisfy the following set of conditions \citep{jin2019local}. 
\begin{definition}[Local minimax point]\label{def: local}
A point $(x, y)$ is a local minimax point of (P) if it satisfies 
\begin{enumerate}[leftmargin=*,topsep=0mm,itemsep=1mm]
    \item Stationary: $\nabla_1 f(x,y)=\zero,~ \nabla_2 f(x,y)=\zero$;
    \item Non-degeneracy: $\nabla_{22} f(x, y) \prec \zero$, and \\ $\big[\nabla_{11} f - \nabla_{12} f (\nabla_{22} f)^{-1} \nabla_{21} f\big](x,y) \succeq \zero$.
\end{enumerate}
\end{definition}
Local minimax points are different from global minimax points, which require $x$ and $y$ to be the global minimizer and global maximizer of the functions $\Phi(x)$ and $f(x, \cdot)$, respectively. 
In general minimax optimization, global minimax points can be neither local minimax points nor even stationary points \citep{jin2019local}.  
However, it has been shown that global minimax necessarily implies local minimax in nonconvex-strongly-concave optimization \citep{jin2019local}. Moreover, under mild conditions, many machine learning problems have been shown to possess local minimax points, e.g., generative adversarial networks (GANs) \citep{Nagarajan17,zhang2021newtontype}, distributional robust machine learning \citep{sinha2017certifiable}, etc. 



Throughout the paper, we adopt the following standard assumptions on the minimax optimization problem (P) \citep{lin2019gradient,jin2019local,zhang2021newtontype}.
\begin{assum}\label{assum: f}
	The minimax problem $\mathrm{(P)}$ satisfies:
	\begin{enumerate}[leftmargin=*,topsep=0mm,itemsep=1mm]
		\item Function $f(\cdot,\cdot)$ is $L_1$-smooth and function $f(x,\cdot)$ is $\mu$-strongly concave for any fixed $x$;
		\item The Jacobian mappings $\nabla_{11} f$, $\nabla_{12} f$, $\nabla_{21} f$, $\nabla_{22} f$ are $L_2$-Lipschitz continuous;
		\item Function $\Phi(x):=\max_{y\in \mathbb{R}^n} f(x,y)$ is bounded below and has compact sub-level sets.
	\end{enumerate}
\end{assum} 

To elaborate, {item 1 considers the class of nonconvex-strongly-concave functions $f$ that has been widely studied in the minimax optimization literature \citep{lin2019gradient,jin2019local,xu2020unified,lu2020hybrid}}, and it is also satisfied by many machine learning applications. 
Item 2 assumes that the block Jacobian matrices of $f$ are Lipschitz continuous, which is a standard assumption for analyzing second-order optimization algorithms \citep{Nesterov2006,Agarwal2017}. Moreover, item 3 {guarantees that the minimax problem has at least one solution.} 

Under \Cref{assum: f}, the following properties regarding the gradient of the minimax problem (P) have been proved in the literature. Throughout, we denote $\kappa=L_1/\mu$ as the condition number. 
\begin{restatable}{proposition}{prop1}{\citep{lin2019gradient}}\label{prop_1}
	Let \Cref{assum: f} hold. Then, the mapping $y^*(x):=\arg\max _{y\in \mathbb{R}^n}f(x,y)$ is unique for every fixed $x$. 
	Moreover, it holds that
	\begin{enumerate}[leftmargin=*,topsep=0mm,itemsep=1mm]
		\item Mapping $y^*(x)$ is $\kappa$-Lipschitz continuous; \label{item: ystar_lipschitz}
		\item Function $\Phi(x)$ is $L_1(1+\kappa)$-smooth and $\nabla\Phi(x)=\nabla_1 f(x,y^*(x))$. \label{item: Phi_Lsmooth}
	\end{enumerate}
\end{restatable}



% \begin{definition}(Subdifferential and critical point, \cite{rockafellar2009variational})\label{def:sub}
% 	The Frech\'et subdifferential $\widehat\partial h$ of function $h$ at $x\in \dom h$ is the set of $u\in \mathbb{R}^d$ defined as
% 	\begin{align*}
% 	\widehat\partial h(x) := \Big\{u: \liminf_{z\neq x, z\to x} \frac{h(z) - h(x) - u^\intercal(z-x)}{\|z-x\|} \ge 0 \Big\},
% 	\end{align*}
% 	and the limiting subdifferential $\partial h$ at $x\in\dom h$ is the graphical closure of $\widehat\partial h$ defined as:
% 	\begin{align*}
% 	\partial h(x) := \{ u: \exists x_k \to x, h(x_k) \to h(x), \red{u_k \in \widehat{\partial} h(x_k), u_k \to u} \}.
% 	\end{align*}
% 	The set of \textbf{critical points} of $h$ is defined as $\mathbf{\crit}\!~h := \{ x: \zero\in\partial h(x) \}$. 
% \end{definition}
% Throughout, we refer to the limiting subdifferential as subdifferential. We note that  subdifferential is a generalization of gradient (when $h$ is differentiable) and subgradient (when $h$ is convex) to the nonconvex setting. In particular, any local maximizer of $h$ must be a critical point.
 
%so the critical point defined in \Cref{def:sub} also generalizes its usual definition for smooth or convex functions. 




















==> 20230217 CubicMinimax_ArXiV_underTMLRreview/proposition1proof.tex <==
%In this supplementary material, we present the proof of all the results claimed in the paper. 

\section{Supporting Lemmas}
We first prove the following auxiliary lemma that bounds the spectral norm of the Jacobian matrices. 
\begin{lemma}\label{lemma_HessBound}
    Let \Cref{assum: f} hold. Then, for any $x\in \mathbb{R}^m$ and $y\in \mathbb{R}^n$, the Jacobian matrices of $f(x,y)$ {and $G(x,y)=\big[\nabla_{11} f - \nabla_{12} f (\nabla_{22} f)^{-1} \nabla_{21} f\big](x,y)$} satisfy the following bounds.
    \begin{align}
        &\|[\nabla_{22} f(x,y)]^{-1}\|\le \mu^{-1}, \label{HessInv_up}\\
        &\|\nabla_{12} f(x,y)\|=\|\nabla_{21} f(x,y)\|\le L_1, \label{Hess_below}\\
        &{\|\nabla_{11} f(x,y)\|\le L_1,} \label{Hess_below2}\\
        &{\|G(x,y)\|\le L_1(1+\kappa).}\label{G_up}
    \end{align}
    The same bounds also hold for $\widehat{\nabla}_{11} f$, $\widehat{\nabla}_{12} f$, $\widehat{\nabla}_{21} f$, $\widehat{\nabla}_{22} f$  and $\widehat{G}$ defined in Section \ref{sec: stoc} under \Cref{assum: fi}.
\end{lemma}
\begin{proof}
    We first prove \cref{HessInv_up}. Consider any $x\in \mathbb{R}^m$ and $y\in \mathbb{R}^n$. By \Cref{assum: f} we know that $f(x,\cdot)$ is $\mu$-strongy concave, which implies that $-\nabla_{22} f(x,y)\succeq \mu I$. Thus, we further conclude that 
    $$\|[\nabla_{22} f(x,y)]^{-1}\|=\lambda_{\max}\big([-\nabla_{22} f(x,y)]^{-1}\big)=\Big(\lambda_{\min}\big(-\nabla_{22} f(x,y)\big)\Big)^{-1}\le \mu^{-1}.$$
    
    %Define the Frobenius norm of a matrix $A=[a_{ij}]$ as $\|A\|_F:=\sqrt{\sum_{ij}a_{ij}^2}$. Then, and $u\in \mathbb{R}^d$ ($d$ is the dimensionality of $\mathbb{R}^n$)
    Next, we prove eq. \eqref{Hess_below}. Consider any $x, u\in \mathbb{R}^m$ and $y\in \mathbb{R}^n$, we have
    \begin{align}
        \|\nabla_{21} f(x,y)u\|=&\Big\|\frac{\partial}{\partial t}\nabla_2 f(x+tu,y)\Big|_{t=0}\Big\|\nonumber\\
        =&\Big\|\lim_{t\to 0} \frac{1}{t}\big[\nabla_2 f(x+tu,y)-\nabla_2 f(x,y)\big]\Big\|\nonumber\\
        =& \lim_{t\to 0} \frac{1}{|t|}\big\|\nabla_2 f(x+tu,y)-\nabla_2 f(x,y)\big\| \nonumber\\
        \le& \lim_{t\to 0} \frac{L_1}{|t|}\big\|tu\big\|=L_1\|u\|,
    \end{align}
    which implies that $\|\nabla_{21} f(x,y)\|\le L_1$. Since $f$ is twice differentiable and has continuous second-order derivative, we have $\nabla_{12} f(x,y)^{\top}=\nabla_{21} f(x,y)$, and hence eq. \eqref{Hess_below} follows. {The proof of eq. \eqref{Hess_below2} is similar.
    
    Finally, eq. \eqref{G_up} can be proved as follows using eqs. \eqref{HessInv_up}\&\eqref{Hess_below}.
    \begin{align}
        \|G(x,y)\|\le \|\nabla_{11} f(x,y)\| + \|\nabla_{12} f(x,y)\| \|\nabla_{22} f^{-1}(x,y)\| \|\nabla_{21} f(x,y)\| \le L_1 + L_1\mu^{-1} L_1 =L_1(1+\kappa). \nonumber
    \end{align}
    The proof is similar for the stochastic minimax optimization problem (Q) in Section \ref{sec: stoc} under \Cref{assum: fi}.
    }
\end{proof}

The following lemma restates Lemma 3 of \cite{wang2018note}. 
\begin{lemma}\label{lemma_CRsol}
    The solution $s_{k+1}$ of the cubic regularization problem in Algorithm \ref{algo: prox-minimax} satisfies the following conditions, 
    \begin{align}
        \nabla f(x_t,y_{t+1})+G(x_t,y_{t+1})s_{t+1}+\frac{1}{2\eta_x}\|s_{t+1}\|s_{t+1}=&~ \zero, \label{eq: CRcond1}\\
        G(x_t,y_{t+1})+\frac{1}{2\eta_x}\|s_{t+1}\|I\succeq& ~\mathbf{O}, \label{eq: CRcond2}\\
        \nabla f(x_t,y_{t+1})^{\top}s_{t+1}+\frac{1}{2}s_{t+1}^{\top}G(x_t,y_{t+1})s_{t+1} \le& -\frac{1}{4\eta_x}\|s_{t+1}\|^3. \label{eq: CRcond3}
    \end{align}
\end{lemma}

\begin{restatable}{lemma}{lemmaIfErrSmallNoKL}\label{lemma_ifErrSmall_noKL}
    Suppose the gradient $\nabla_1 f(x_t, y_{t+1})$ and Hessian $G(x_t,y_{t+1})$ involved in the cubic-regularization step in Algorithm \ref{algo: prox-minimax} satisfy the following bounds for all $t\le T'-1$ with $T'=\min\{t\ge 0: \|s_{t-1}\|\vee \|s_t\|\le\epsilon'\}$:
    \begin{align}
        &\|\nabla\Phi(x_t)-\nabla_1 f(x_t, y_{t+1})\| \le \beta(\|s_t\|^2+\epsilon'^2),\label{eq: grad_goal_noKL}\\ 
        &\|\nabla^2\Phi(x_t)-G(x_t,y_{t+1})\| \le \alpha(\|s_t\|+\epsilon'). \label{eq: Hess_goal_noKL}
    \end{align}
    
    Then, choosing $\eta_x\le (9L_{\Phi}+18\alpha+28\beta)^{-1}$, the sequence $\{x_t\}_t$ generated by Algorithm \ref{algo: prox-minimax} satisfies that for all $t\le T'-2$,
    \begin{align}
        &H_{t+1}-H_t \le -(L_{\Phi}+\alpha+\beta)(\|s_{t+1}\|^3+\|s_t\|^3), \label{eq: Hdec2_noKL}
    \end{align}
    where $H_t=\Phi(x_t)+(L_{\Phi}+2\alpha+3\beta)\|x_t-x_{t-1}\|^3$. The same conclusion holds for Algorithm \ref{algo: prox-minimax-stoc} by replacing $\nabla_1 f(x_t,y_{t+1})$, $G(x_t,y_{t+1})$ with their stochastic estimators $\widehat{\nabla}_1 f(x_t,y_{t+1})$, $\widehat{G}(x_t,y_{t+1})$ respectively. 
\end{restatable}

\begin{proof}
The proof logic follows that of the proof of Theorem 1 in \cite{wang2019stochastic}.
By the Lipschitz continuity of the Hessian of $\Phi$, we obtain that
\begin{align}
    &\Phi(x_{t+1})-\Phi(x_t) \nonumber\\
    &\le \nabla \Phi(x_t)^{\top} (x_{t+1}-x_t) + \frac{1}{2}(x_{t+1}-x_t)^{\top} \nabla^2 \Phi(x_t)  (x_{t+1}-x_t) + \frac{L_{\Phi}}{6} \|x_{t+1}-x_t\|^3 \nonumber\\
    &= \nabla_1 f(x_t, y_{t+1})^{\top} s_{t+1}  + \frac{1}{2}s_{t+1}^{\top} G(x_t,y_{t+1}) s_{t+1} + \frac{L_{\Phi}}{6} \|s_{t+1}\|^3 \nonumber\\
    &\quad +\big(\nabla \Phi(x_t)-\nabla_1 f(x_t, y_{t+1})\big)^{\top} s_{t+1} + \frac{1}{2}s_{t+1}^{\top} \big(\nabla^2 \Phi(x_t)-G(x_t,y_{t+1})\big) s_{t+1}\nonumber\\
    &\stackrel{(i)}{\le}  \Big(\frac{L_{\Phi}}{6}-\frac{1}{4\eta_x}\Big)\|s_{t+1}\|^3 +
    \beta \|s_{t+1}\|(\|s_t\|^2+\epsilon'^2) + \frac{\alpha}{2}\|s_{t+1}\|^2(\|s_t\|+\epsilon') \nonumber\\
    &\stackrel{(ii)}{\le} \Big(\frac{L_{\Phi}}{6}-\frac{1}{4\eta_x}\Big)\|s_{t+1}\|^3 + \Big(\frac{\alpha}{2}+\beta\Big)(2\|s_{t+1}\|^3+\|s_t\|^3+\epsilon'^3) \nonumber\\
    &\stackrel{(iii)}{\le} \Big(\frac{L_{\Phi}}{6}-\frac{1}{4\eta_x}\Big)\|s_{t+1}\|^3 + \Big(\frac{\alpha}{2}+\beta\Big)(3\|s_{t+1}\|^3+2\|s_t\|^3) \nonumber\\
    &\le -\Big(\frac{1}{4\eta_x}-\frac{L_{\Phi}}{6}-\frac{3\alpha}{2}-3\beta\Big)\|s_{t+1}\|^3 + (\alpha+2\beta)\|s_t\|^3, \nonumber\\
    &\stackrel{(iv)}{\le} -(2L_{\Phi}+3\alpha+4\beta)\|s_{t+1}\|^3 + (\alpha+2\beta)\|s_t\|^3\nonumber
\end{align}
where (i) uses eqs. \eqref{eq: CRcond3}, \eqref{eq: grad_goal_noKL}\& \eqref{eq: Hess_goal_noKL}, (ii) uses the inequality that $ab^2\le a^3\vee b^3\le a^3+b^3, \forall a,b\ge 0$, (iii) uses $\epsilon'^3\le \|s_t\|^3\vee\|s_{t+1}\|^3\le \|s_t\|^3+\|s_{t+1}\|^3, \forall 0\le t\le T'-2$ based on the termination criterion of $T'$, and (iv) uses $\eta_x\le (9L_{\Phi}+18\alpha+28\beta)^{-1}$. Eq. \eqref{eq: Hdec2_noKL} follows from the above inequality by defining $H_t=\Phi(x_t)+(L_{\Phi}+2\alpha+3\beta)\|x_t-x_{t-1}\|^2$. 

Note that the cubic-regularization step in Algorithm \ref{algo: prox-minimax-stoc} 
simply replaces $\nabla_1 f(x_t,y_{t+1})$, $G(x_t,y_{t+1})$ in Algorithm \ref{algo: prox-minimax} with their stochastic estimators $\widehat{\nabla}_1 f(x_t,y_{t+1})$, $\widehat{G}(x_t,y_{t+1})$ respectively. Hence, eq. \eqref{eq: Hdec2_noKL} holds for Algorithm \ref{algo: prox-minimax-stoc} after such replacement in eqs. \eqref{eq: grad_goal_noKL} \& \eqref{eq: Hess_goal_noKL}.
\end{proof}

\begin{lemma}\label{lemma_general_rate}
    Suppose all the conditions of Lemma \ref{lemma_ifErrSmall_noKL} hold. If $T\ge \frac{\Phi(x_0)-\Phi^*+(L_{\Phi}+3\alpha+4\beta)\epsilon'^2}{(L_{\Phi}+\alpha+\beta)\epsilon'^3}$ in Algorithm \ref{algo: prox-minimax}, then $T'=\min\{t\ge 1: \|s_{t-1}\|\vee \|s_t\|\le\epsilon'\}\le \frac{\Phi(x_0)-\Phi^*+(L_{\Phi}+3\alpha+4\beta)\epsilon'^2}{(L_{\Phi}+\alpha+\beta)\epsilon'^3}\le T$. Consequently, the Output II of Algorithm \ref{algo: prox-minimax} has the following convergence rate
    \begin{align}
        &\|\nabla \Phi(x_{T'})\| \le \Big(\frac{1}{2\eta_x}+L_{\Phi}+2\alpha+2\beta\Big) \epsilon'^2, \label{eq: grad_rate_early}\\
        &\nabla^2 \Phi(x_{T'}) \succeq -\Big(\frac{1}{2\eta_x}+L_{\Phi}+2\alpha\Big)\epsilon'I. \label{eq: Hess_rate_early}
    \end{align}
    The same conclusion holds for Algorithm \ref{algo: prox-minimax-stoc} by replacing $\nabla_1 f(x_t,y_{t+1})$, $G(x_t,y_{t+1})$ in the conditions \eqref{eq: grad_goal_noKL} \& \eqref{eq: Hess_goal_noKL} with their stochastic estimators $\widehat{\nabla}_1 f(x_t,y_{t+1})$, $\widehat{G}(x_t,y_{t+1})$ respectively. 
\end{lemma}
\begin{proof}
The proof logic follows that of the proof of Theorem 1 in \cite{wang2019stochastic}.
%The proof logic is similar to the end of the proof of Theorem 1 in \cite{wang2019stochastic}. 

Suppose $T'\le T$ does not hold, i.e., $\|s_{t-1}\|\vee \|s_t\|>\epsilon', \forall 1\le t\le T$, which implies that eq. \eqref{eq: Hdec2_noKL} holds for all $0\le t\le T-1$ based on Lemma \ref{lemma_ifErrSmall_noKL}.

On one hand, telescoping eq. \eqref{eq: Hdec2_noKL} over $t=0,1,\ldots,T-1$ yield that
\begin{align}
    H_0-H_T&\ge
    (L_{\Phi}+\alpha+\beta)\sum_{t=0}^{T-1}(\|s_{t+1}\|^3+\|s_t\|^3) \nonumber\\
    &\ge (L_{\Phi}+\alpha+\beta)\sum_{t=0}^{T-1}(\|s_t\|\vee\|s_{t+1}\|)^3 \nonumber\\
    &> T(L_{\Phi}+\alpha+\beta)\epsilon'^3\nonumber\\
    &\ge \Phi(x_0)-\Phi^*+(L_{\Phi}+3\alpha+4\beta)\epsilon'^2.  \label{eq: Hdiff_low}
\end{align}
On the other hand, recalling the definition of $H_t$ in Lemma \ref{lemma_ifErrSmall_noKL}, we have
\begin{align}
    H_0-H_T&=\Phi(x_0)-\Phi(x_T)+(L_{\Phi}+2\alpha+3\beta)(\|s_0\|^2-\|s_T\|^2) \nonumber\\
    &\stackrel{(i)}{\le} \Phi(x_0)-\Phi^*+(L_{\Phi}+3\alpha+4\beta)\epsilon'^2, \label{eq: Hdiff_up}
\end{align}
where (i) uses $\|s_0\|=\epsilon'$ and $\Phi(x_T)\ge \Phi^*=\min_{x\in\mathbb{R}^m}\Phi(x)$. Note that eqs. \eqref{eq: Hdiff_low} \& \eqref{eq: Hdiff_up} contradict. Therefore, we must have $1\le T'\le T$ for any $T\ge \frac{\Phi(x_0)-\Phi^*+(L_{\Phi}+3\alpha+4\beta)\epsilon'^2}{(L_{\Phi}+\alpha+\beta)\epsilon'^3}$, which implies that $T'\le \frac{\Phi(x_0)-\Phi^*+(L_{\Phi}+3\alpha+4\beta)\epsilon'^2}{(L_{\Phi}+\alpha+\beta)\epsilon'^3}\le T$.  

Finally, we conclude that 
\begin{align}
&\|\nabla \Phi(x_{T'})\|\nonumber\\
&\overset{(i)}{=}\Big\|\nabla \Phi(x_{T'})-\nabla f(x_{T'-1},y_{T'}) -G(x_{T'-1},y_{T'}) s_{T'} -\frac{1}{2\eta_x}\|s_{T'}\|s_{T'}\Big\| \nonumber\\
&\le \|\nabla \Phi(x_{T'})-\nabla \Phi(x_{T'-1})-\nabla^2 \Phi(x_{T'-1})s_{T'}\| + \|\nabla \Phi(x_{T'-1})-\nabla f(x_{T'-1},y_{T'})\|\nonumber\\
&\quad + \|\nabla^2 \Phi(x_{T'-1})s_{T'}-G(x_{T'-1},y_{T'}) s_{T'}\| + \frac{1}{2\eta_x}\|s_{T'}\|^2 \nonumber\\
&\overset{(ii)}{\le} \Big(L_{\Phi}+\frac{1}{2\eta_x}\Big)\|s_{T'}\|^2  +\beta(\|s_{T'-1}\|^2+\epsilon'^2) +\alpha(\|s_{T'-1}\|+\epsilon')\|s_{T'}\|\nonumber\\
&\overset{(iii)}{\le} \Big(\frac{1}{2\eta_x}+L_{\Phi}+2\alpha+2\beta\Big) \epsilon'^2, \label{eq: grad_bound_general}
\end{align}
where (i) uses eq. \eqref{eq: CRcond1}, (ii) uses eqs. \eqref{eq: grad_goal_noKL} \& \eqref{eq: Hess_goal_noKL} and the item \ref{item: ddPhi} of \Cref{prop_Phiystar} that $\nabla^2\Phi$ is $L_{\Phi}$-Lipschitz, and (iii) uses $\|s_{T'-1}\|\vee \|s_{T'}\|\le\epsilon'$. Also,
\begin{align}
\nabla^2 \Phi(x_{T'}) &\overset{(i)}{\succeq}  G(x_{T'-1},y_{T'})-\|G(x_{T'-1},y_{T'})-\nabla^2 \Phi(x_{T'})\|I \nonumber\\
&\overset{(ii)}{\succeq} -\frac{1}{2\eta_x}\|s_{T'}\|I -\|G(x_{T'-1},y_{T'})-\nabla^2 \Phi(x_{T'-1})\|I -\|\nabla^2 \Phi(x_{T'})-\nabla^2 \Phi(x_{T'-1})\|I \nonumber\\
&\overset{(iii)}{\succeq} -\Big(\frac{1}{2\eta_x}+L_{\Phi}\Big)\|s_{T'}\|I-\alpha(\|s_{T'-1}\|+\epsilon')I \nonumber\\
&\overset{(iv)}{\succeq} -\Big(\frac{1}{2\eta_x}+L_{\Phi}+2\alpha\Big)\epsilon' I, \label{eq: Hess_bound_general}
\end{align}
where (i) uses Weyl's inequality, (ii) uses eq. \eqref{eq: CRcond2}, (iii) uses eq. \eqref{eq: Hess_goal_noKL} and the item \ref{item: ddPhi} of \Cref{prop_Phiystar} that $\nabla^2\Phi$ is $L_{\Phi}$-Lipschitz, and (iv) uses $\|s_{T'-1}\|\vee \|s_{T'}\|\le\epsilon'$. 
\end{proof}

\iffalse
\begin{restatable}{lemma}{lemmaNtnoKL}\label{lemma_Nt_noKL}
Run Algorithm \ref{algo: prox-minimax} with hyperparameter choices $\epsilon'\le \frac{\alpha L_1}{\beta L_G}$ and $\eta_{y}=\frac{2}{L+\mu}$ and sufficiently large number of inner iterations $N_t$ as follows, then the conditions \eqref{eq: grad_goal_noKL} \& \eqref{eq: Hess_goal_noKL} hold and thus eq. \eqref{eq: Hdec2_noKL} holds. 
\begin{align}
    \left\{ \begin{gathered}
    N_0\ge 2\kappa\ln\big(L_1\|y_0-y^*(x_0)\|/(2\beta\epsilon'^2)\big)\hfill\\
    N_t\ge \kappa\ln\Big(\frac{2L_1\alpha\|s_{t-1}\|+L_1(\alpha+L_G\kappa)\|s_t\|}{L_G\beta\epsilon'^2}\Big); t\ge 1.\\
    \end{gathered}  \right. \label{Nt_noKL}
\end{align}
\end{restatable}
\begin{proof}
    We first bound the term $\|y_{t+1}-y^*(x_t)\|$, which corresponds to the optimality gap of the maximization problem. Note that $y^*(x_t)\in \mathbb{R}^n$ is the unique maximizer of the strongly concave function $f(x_t,y)$. 
    Note that $y_{t+1}$ is obtained by applying $N_t$ gradient ascent steps starting from $y_t$. Hence, by the convergence rate of gradient ascent algorithm under strong concavity, we conclude that with learning rate $\eta_{y}=\frac{2}{L+\mu}$,
    \begin{align}
    	\|y_{t+1} - y^*(x_{t}) \| \le&  (1-\kappa^{-1})^{N_t}\|y_{t} - y^*(x_{t})\| \label{eq: 8}
    \end{align}
    
    We will prove by induction that for any $t\ge 0$,
	\begin{align}
    \|y_{t+1}-y^*(x_t)\|\le& \min\Big(\frac{\alpha(\|s_t\|+\epsilon')}{L_G},\frac{\beta(\|s_t\|^2+\epsilon'^2)}{L_1}\Big). \label{eq: yerr_t}
    \end{align}

    %We consider the following three cases.
    
    %(Case 1) 
    When $t=0$, on one hand, eq. \eqref{eq: 8} implies that
    \begin{align}
        \|y_1-y^*(x_t)\|&\le \|y_0-y^*(x_0)\|\exp\big(N_0\ln(1-\kappa^{-1})\big) \nonumber\\
        &\overset{(i)}{\le} \|y_0-y^*(x_0)\|\exp\Big(-\ln\Big(\frac{L_1\|y_0-y^*(x_0)\|}{2\beta\epsilon'^2}\Big)\Big) \le \frac{2\beta\epsilon'^2}{L_1} \label{eq: yerr_0a}
    \end{align}
    where (i) uses $\ln(1-x)\le -x<0$ for $x=\kappa^{-1}\in(0,1)$ and $N_0\ge 2\kappa\ln\big(L_1\|y_0-y^*(x_0)\|/(2\beta\epsilon'^2)\big)$. 
    
    On the other hand, the right side of eq. \eqref{eq: yerr_t} is simplified as follows. 
    \begin{align}
        \min\Big(\frac{\alpha(\|s_0\|+\epsilon')}{L_G},\frac{\beta(\|s_0\|^2+\epsilon'^2)}{L_1}\Big) \overset{(i)}{=}  \min\Big(\frac{2\alpha\epsilon'}{L_G},\frac{2\beta\epsilon'^2}{L_1}\Big)\overset{(ii)}{=} \frac{2\beta\epsilon'^2}{L_1} \label{eq: yerr_0b}
    \end{align}
    where (i) uses $\|s_0\|=\epsilon'$ and (ii) uses $\epsilon'\le \frac{\alpha L_1}{\beta L_G}$. Hence, eqs. \eqref{eq: yerr_0a}\&\eqref{eq: yerr_0b} imply that the error bound \eqref{eq: yerr_t} holds for $t=0$.
    
    %(Case 2) 
    Suppose the error bound \eqref{eq: yerr_t} holds for $t=k-1$. Then, on one hand, eq. \eqref{eq: 8} implies that
    \begin{align}
        &\|y_{k+1} - y^*(x_{k}) \| \nonumber\\
        &\le  (1-\kappa^{-1})^{N_k}\|y_{k} - y^*(x_{k})\| \nonumber\\
        &\le  (1-\kappa^{-1})^{N_k}\|y_{k} - y^*(x_{k-1})\| + (1-\kappa^{-1})^{N_k}\|y^*(x_{k-1}) - y^*(x_{k})\| \nonumber\\
        &\overset{(i)}{\le} \exp\big(N_k\ln(1-\kappa^{-1})\big) \Big(\min\Big(\frac{\alpha(\|s_{k-1}\|+\epsilon')}{L_G},\frac{\beta(\|s_{k-1}\|^2+\epsilon'^2)}{L_1}\Big)+\kappa\|s_k\|\Big) \nonumber\\
        &\overset{(ii)}{\le} \exp\Big(-\ln\Big(\frac{2L_1\alpha\|s_{k-1}\|+L_1(\alpha+L_G\kappa)\|s_k\|}{L_G\beta\epsilon'^2}\Big)\Big) \Big(\frac{\alpha(\|s_{k-1}\|+\epsilon')}{L_G} + \kappa\|s_k\|\Big) \nonumber\\
        &= \frac{L_G\beta\epsilon'^2}{2L_1\alpha\|s_{k-1}\|+L_1(\alpha+L_G\kappa)\|s_k\|} \frac{\alpha(2\|s_{k-1}\|+\|s_k\|)+L_G\kappa\|s_k\|}{L_G} =\frac{\beta\epsilon'^2}{L_1} \label{eq: yerr_1a}
    \end{align}
    where (i) uses eq. \eqref{eq: yerr_t} for $t=k-1$ and the fact that $y^*$ is $\kappa$-Lipschitz mapping (see \cite{lin2019gradient,chen2021proximal} for the proof), (ii) uses $\ln(1-\kappa^{-1})\le -\kappa^{-1}$, $N_k\ge \kappa\ln\Big(\frac{2L_1\alpha\|s_{k-1}\|+L_1(\alpha+L_G\kappa)\|s_k\|}{L_G\beta\epsilon'^2}\Big)$ and $\epsilon'\le \|s_{k-1}\|\vee\|s_k\|\le \|s_{k-1}\|+\|s_k\|$. 
    On the other hand, the right side of eq. \eqref{eq: yerr_t} for $t=k\in [1, T'-1]$ can be lower bounded as follows.
    \begin{align}
        \min\Big(\frac{\alpha(\|s_k\|+\epsilon')}{L_G},\frac{\beta(\|s_k\|^2+\epsilon'^2)}{L_1}\Big)\ge \min\Big(\frac{\alpha\epsilon'}{L_G},\frac{\beta\epsilon'^2}{L_1}\Big) \overset{(i)}{=} \frac{\beta\epsilon'^2}{L_1} \label{eq: yerr_1b}
    \end{align}
    where (i) uses $\epsilon'\le \frac{\alpha L_1}{\beta L_G}$. Combining eqs. \eqref{eq: yerr_1a} \& \eqref{eq: yerr_1b} proves \eqref{eq: yerr_t} for $t=k$. Hence, eq. \eqref{eq: yerr_t} holds for all $t\ge 0$.
\end{proof}

\begin{restatable}{lemma}{lemmaNtKL}\label{lemma_Nt_KL}
Run Algorithm \ref{algo: prox-minimax} with hyperparameters $\epsilon'\le \frac{\alpha L_1}{\beta L_G}$ and sufficiently large number of inner iterations $N_t$ as follows, then the conditions \eqref{eq: grad_goal_KL} \& \eqref{eq: Hess_goal_KL} hold and thus eq. \eqref{eq: Hdec2_KL} holds. 
\begin{align}
    N_t\ge \frac{4\kappa}{3}\ln t+\kappa\ln\Big(\frac{L_1\alpha\|s_{t-1}\|+t^{-4/3}L_1\alpha\epsilon'+L_1L_G\kappa\|s_t\|}{L_G\beta\epsilon'^2}\Big) \label{Nt_KL}
\end{align}
\end{restatable}

\begin{proof}
    The proof of logic is similar to that of Lemma \ref{lemma_Nt_noKL}. We will prove by induction that for any $t\ge 0$,
	\begin{align}
    \|y_{t+1}-y^*(x_t)\|\le& \min\Big(\frac{\alpha(\|s_t\|+\epsilon')}{L_G},\frac{\beta(\|s_t\|^2+\epsilon'^2)}{L_1}\Big). \label{eq: yerr_t}
    \end{align}

    Suppose the error bound \eqref{eq: yerr_t} holds for $t=k-1\ge T'-1$. Then, on one hand, similar to the derivation of eq. \eqref{eq: yerr_1a}, eq. \eqref{eq: 8} implies that
    \begin{align}
        &\|y_{k+1} - y^*(x_{k}) \| \nonumber\\
        &\le (1-\kappa^{-1})^{N_k}\|y_{k} - y^*(x_{k-1})\| + (1-\kappa^{-1})^{N_k}\|y^*(x_{k-1}) - y^*(x_{k})\| \nonumber\\
        &\overset{(i)}{\le} \exp\big(N_k\ln(1-\kappa^{-1})\big) \Big(\min\Big(\frac{\alpha(\|s_{k-1}\|+t^{-2/3}\epsilon')}{L_G},\frac{\beta(\|s_{k-1}\|^2+t^{-4/3}\epsilon'^2)}{L_1}\Big)+\kappa\|s_k\|\Big) \nonumber\\
        &\overset{(ii)}{\le} \exp\Big(-\frac{4}{3}\ln t-\ln\Big(\frac{L_1\alpha\|s_{k-1}\|+t^{-4/3}L_1\alpha\epsilon'+L_1L_G\kappa\|s_k\|}{L_G\beta\epsilon'^2}\Big)\Big)  \frac{\alpha(\|s_{k-1}\|+t^{-2/3}\epsilon')+L_G\kappa\|s_k\|}{L_G} \nonumber\\
        &= \frac{t^{-4/3}L_G\beta\epsilon'^2}{L_1\alpha\|s_{k-1}\|+t^{-4/3}L_1\alpha\epsilon'+L_1L_G\kappa\|s_k\|}  \frac{\alpha(\|s_{k-1}\|+t^{-2/3}\epsilon')+L_G\kappa\|s_k\|}{L_G}\nonumber\\ &\le\frac{\beta\epsilon'^2}{L_1t^{4/3}} \label{eq: yerr_2a}
    \end{align}
    where (i) uses eq. \eqref{eq: yerr_t} for $t=k-1$ and the fact that $y^*$ is $\kappa$-Lipschitz mapping (see \cite{lin2019gradient,chen2021proximal} for the proof), (ii) uses $\ln(1-\kappa^{-1})\le -\kappa^{-1}$, $N_k\ge \frac{4\kappa}{3}\ln k+\kappa\ln\Big(\frac{L_1\alpha\|s_{k-1}\|+k^{-4/3}L_1\alpha\epsilon'+L_1L_G\kappa\|s_k\|}{L_G\beta\epsilon'^2}\Big)$, (iii) uses $4a^3+4b^3\ge (a+b)^3; \forall a,b\ge 0$. 
    
    On the other hand, the right side of eq. \eqref{eq: yerr_t} for $t=k\in [1, T'-1]$ can be lower bounded as follows.
    \begin{align}
        &\min\Big(\frac{\alpha(\|s_k\|+2^{-\max(0,k-T'-1)/3}\epsilon')}{L_G},\frac{\beta(\|s_k\|^2+2^{-2\max(0,k-T'-1)/3}\epsilon'^2)}{L_1}\Big) \nonumber\\
        &\ge \min\Big(\frac{t^{-2/3}\alpha\epsilon'}{L_G},\frac{2^{-2(k-T'-1)/3}\beta\epsilon'^2}{L_1}\Big) \overset{(i)}{=} \frac{2^{-2(k-T'-1)/3}\beta\epsilon'^2}{L_1} \label{eq: yerr_2b}
    \end{align}
    where (i) uses $\epsilon'\le \frac{\alpha L_1}{\beta L_G}$. Combining eqs. \eqref{eq: yerr_1a} \& \eqref{eq: yerr_1b} proves \eqref{eq: yerr_t} for $t=k\ge T'$.
    
    Combining the above 3 cases proves eq. \eqref{eq: yerr_t} for all $t\ge 0$. As a result, eqs. \eqref{eq: grad_goal} \& \eqref{eq: Hess_goal} can be proved as follows.
    \begin{align}
    \|\nabla\Phi(x_t)-\nabla_1 f(x_t, y_{t+1})\|&=\|\nabla_1 f(x_t,y^*(x_t))-\nabla_1 f(x_t, y_{t+1})\|\nonumber\\
    &\le L_1\|y_{t+1}-y^*(x_t)\|\nonumber\\
    &\le\beta(\|s_t\|^2+2^{-2\max(0,t-T'-1)/3}\epsilon'^2),\nonumber
    \end{align}
    \begin{align}
    \|\nabla^2\Phi(x_t)-G(x_t,y_{t+1})\|&=\|G(x_t,y^*(x_t))-G(x_t, y_{t+1})\|\nonumber\\
    &\le L_G\|y_{t+1}-y^*(x_t)\|\nonumber\\
    &\le\alpha(\|s_t\|+2^{-\max(0,t-T'-1)/3}\epsilon').
    \end{align}
\end{proof}
\fi
    
For the stochastic minimax optimization problem (Q) in Section \ref{sec: stoc}, we prove the following supporting lemma on the error of the stochastic estimators.
\lemmaBatch*
\begin{proof}
    Based on Lemmas 6 \& 8 in \cite{kohler2017}, we obtain that with probability at least $1-\delta$, the following bounds hold. (We replaced $\delta$ in \cite{kohler2017} with $\delta/5$ by applying union bound to the following 5 events.)
    \begin{align}
        &\|\widehat{\nabla}_1 f(x,y)-\nabla_1 f(x,y)\|\le 4\sqrt{2}L_0 \sqrt{\frac{\ln(10m/\delta)+1/4}{|B_1|}} \le \epsilon_1,\\ 
        &\|\widehat{\nabla}_{k,\ell}^2 f(x,y)-\nabla_{k,\ell}^2 f(x,y)\|\le 4L_1\sqrt{\frac{\ln\big(10(m\vee n)/\delta\big)}{|B_{k,\ell}|}} \le \epsilon_2; k,\ell\in\{1,2\}.
    \end{align}
    Note that here we only consider the cases that $|B_1|,|B_{k,\ell}|<N$ for all $k,\ell\in\{1,2\}$. Otherwise, $|B_1|=N$ yields $\|\widehat{\nabla}_1 f(x,y)-\nabla_1 f(x,y)\|=0<\epsilon_1$ and $|B_{k,\ell}|=N$ yields $\|\widehat{\nabla}_{k,\ell}^2 f(x,y)-\nabla_{k,\ell}^2 f(x,y)\|=0<\epsilon_2$. Hence, in both cases, the above high probability bounds hold, which further implies eq. \eqref{eq: stoc_err3} following the argument below.
        \begin{align}
        \|\widehat{G}(x,y)-G(x,y)\|&\le \|\widehat{\nabla}_{11} f(x,y)-\nabla_{11} f(x,y)\| + \|(\widehat{\nabla}_{12} f (\widehat{\nabla}_{22} f)^{-1} \widehat{\nabla}_{21} f)(x,y) - (\nabla_{12}f (\nabla_{22}f)^{-1} \nabla_{21} f)(x,y)\| \nonumber\\
        &\le \epsilon_2 +\|(\widehat{\nabla}_{12} f-\nabla_{12}f)\big((\widehat{\nabla}_{22} f)^{-1} \widehat{\nabla}_{21} f\big)(x,y)\| \nonumber\\
        &\quad + \|\nabla_{12}f\big((\widehat{\nabla}_{22} f)^{-1}-(\nabla_{22} f)^{-1}\big)\widehat{\nabla}_{21} f(x,y)\| +\|\nabla_{12}f (\nabla_{22}f)^{-1} (\widehat{\nabla}_{21} f-\nabla_{21}f)(x,y)\| \nonumber\\
        &\overset{(i)}{\le} \epsilon_2 + \epsilon_2 \mu^{-1} L_1 + L_1^2\|\nabla_{22}f(x,y)^{-1}\| \|(\nabla_{22}f-\widehat{\nabla}_{22}f)(x,y)\| \|\widehat{\nabla}_{22}f(x,y)^{-1}\| + L_1\mu^{-1}\epsilon_2 \nonumber\\
        &\overset{(ii)}{\le} \epsilon_2+2\kappa\epsilon_2+L_1^2\mu^{-2}\epsilon_2\le (\kappa+1)^2\epsilon_2.
    \end{align}
    where (i) and (ii) use Lemma \ref{lemma_HessBound}.
\end{proof}

Regarding the high-probability convergence rate of the inner stochastic gradient ascent (SGA) in Algorithm \ref{algo: prox-minimax-stoc}, the following result is a direct application of Theorem 3.1 in \cite{harvey2019simple}.

% This assumption implies that the gradients and stochastic gradients are bounded along the SGA trajectories $x_t,\widetilde{y}_k$, which holds if the trajectories are bounded. The above bound 1 can be obtained by properly scaling the objective function $f$. With this assumption, we obtain the following convergence rate of the SGA steps below.



\section{Proof of \Cref{prop_Phiystar}} \label{sec_prop1proof}
\propphy*
\begin{proof}
%The items \ref{item: ystar_lipschitz} \& \ref{item: Phi_Lsmooth} are proved in \cite{chen2021proximal,lin2019gradient}. 
We first prove the item \ref{item: G_lipschitz}.
Consider any $x, x'\in \mathbb{R}^m$ and $y,y'\in\mathbb{R}^n$. For convenience we denote $z=(x,y)$ and $z'=(x',y')$. Then, by \Cref{assum: f} and using the bounds of \Cref{lemma_HessBound}, we have that
\begin{align}
    &\|G(x',y')-G(x,y)\|\nonumber\\
    &\le \|\nabla_{11} f(x',y')-\nabla_{11} f(x,y)\| + \|\nabla_{12} f(x',y')-\nabla_{12} f(x,y)\| \|[\nabla_{22}f(x',y')]^{-1}\| \|\nabla_{21}f(x',y')\| \nonumber\\
    &\quad +\|\nabla_{12} f(x,y)\| \|[\nabla_{22}f(x',y')]^{-1}-[\nabla_{22}f(x,y)]^{-1}\| \|\nabla_{21}f(x',y')\| \nonumber\\ 
    &\quad +\|\nabla_{12} f(x,y)\| \|[\nabla_{22}f(x,y)^{-1}]\| \|\nabla_{21}f(x',y')-\nabla_{21}f(x,y)\| \nonumber\\
    &\le L_2\|z'-z\| + (L_2\|z'-z\|)\mu^{-1}L_1 \nonumber\\
    &\quad + L_1^2 \|[\nabla_{22}f(x',y')]^{-1}\| \|\nabla_{22}f(x,y)-\nabla_{22}f(x',y')\| \|[\nabla_{22}f(x,y)]^{-1}\| +L_1\mu^{-1}(L_2\|z'-z\|) \nonumber\\
    &\le L_2(1+2\kappa) \|z'-z\| + L_1^2\mu^{-1}(L_2\|z'-z\|)\mu^{-1} \nonumber\\
    &\le L_2(1+\kappa)^2\|z'-z\|. \nonumber
\end{align}

Next, we prove the item \ref{item: ddPhi}. Consider any fixed $x\in\mathbb{R}^m$, we know that $f(x,\cdot)$ achieves its maximum at $y^*(x)$, where the gradient vanishes, i.e., $\nabla_2 f(x,y^*(x))=\zero$. Thus, we further obtain that 
\begin{align}
    &\zero=\nabla_x \nabla_2 f(x,y^*(x))=\nabla_{21} f(x,y^*(x))+\nabla_{22} f(x,y^*(x))\nabla y^*(x), \nonumber
\end{align}
which implies that 
\begin{align}
    \nabla y^*(x)=-[\nabla_{22}f(x,y^*(x))]^{-1}\nabla_{21}f(x,y^*(x)). \label{eq: ystar_grad}
\end{align}

With the above equation, we take derivative of $\nabla \Phi(x)=\nabla_1 f(x,y^*(x))$ and obtain that
\begin{align}
    \nabla^2 \Phi(x) =& \nabla_{11} f(x,y^*(x)) + \nabla_{12} f(x,y^*(x)) \nabla y^*(x)\nonumber\\
    =& \nabla_{11} f(x,y^*(x)) - \nabla_{12} f(x,y^*(x)) [\nabla_{22}f(x,y^*(x))]^{-1}\nabla_{21}f(x,y^*(x))\\\nonumber
    =& G(x, y^*(x)). \nonumber
\end{align}
Moreover, we have that
\begin{align}
    \|\nabla^2 \Phi(x')-\nabla^2 \Phi(x)\|=& \|G(x',y^*(x'))-G(x,y^*(x))\| \nonumber\\
    \le& L_G \big[\|x'-x\|+\|y^*(x')-y^*(x)\|\big] \nonumber\\
    \le& L_G(1+\kappa) \|x'-x\|,
\end{align}
where the last step uses the item \ref{item: ystar_lipschitz} of \Cref{prop_1}. This proves the item \ref{item: ddPhi}. 

%Finally, we will prove the item \ref{item: H_Lsmooth}, i.e., the following partial gradients of function $H(x,x',y)$ is $L_H$-Lipschitz.
%\begin{align}
%    \nabla_1 H(x,x',y)=\nabla \Phi(x) + \frac{2L}{3}\|\|
%\end{align}

\end{proof}


==> 20230217 CubicMinimax_ArXiV_underTMLRreview/proposition2proof.tex <==
\section{Proof of \Cref{prop: lyapunov}} \label{sec_prop2proof}

\proplya*

\begin{proof}
    The required number of inner gradient ascent steps for Output I is shown below. 
    \begin{align}
    \left\{ \begin{gathered}
        N_0\!\ge\! \kappa\ln\Big(\frac{\|y_0-y^*(x_0)\|}{(\alpha\|s_0\|/L_G)\wedge(\beta\|s_0\|^2/L_1)}\Big), \hfill \\
        N_t\!\ge\! \kappa \ln\frac{(\alpha\|s_{k-1}\|/L_G)\wedge (\beta\|s_{k-1}\|^2/L_1)+\kappa\|s_k\|}{(\alpha\|s_k\|/L_G)\wedge(\beta\|s_k\|^2/L_1)}; t\ge 1 \hfill 
    \end{gathered}  \right.. \label{eq: Nt1}
    \end{align}
    
    To prove eq. \eqref{eq: potential} for Output I, we first prove by induction that for any $t\ge 0$,
	\begin{align}
    \|y_{t+1}-y^*(x_t)\|\le& \min\Big(\frac{\alpha\|s_t\|}{L_G},\frac{\beta\|s_t\|^2}{L_1}\Big). \label{eq: yerr_t1}
    \end{align}

    Note that $y_{t+1}$ is obtained by applying $N_t$ gradient ascent steps starting from $y_t$. Hence, by the convergence rate of gradient ascent algorithm under strong concavity, we conclude that with learning rate $\eta_{y}=\frac{2}{L+\mu}$,
    \begin{align}
    	\|y_{t+1} - y^*(x_{t}) \| \le&  (1-\kappa^{-1})^{N_t}\|y_{t} - y^*(x_{t})\|. \label{eq: 8}
    \end{align}

    When $t=0$, eq. \eqref{eq: 8} implies that
    \begin{align}
        \|y_1-y^*(x_0)\|&\le \|y_0-y^*(x_0)\|\exp\big(N_0\ln(1-\kappa^{-1})\big) \nonumber\\
        &\overset{(i)}{\le} \|y_0-y^*(x_0)\|\exp\Big(-\ln\Big(\frac{\|y_0-y^*(x_0)\|}{\min\big(\alpha\|s_0\|/L_G,\beta\|s_0\|^2/L_1\big)}\Big)\Big) \le \min\Big(\frac{\alpha\|s_0\|}{L_G},\frac{\beta\|s_0\|^2}{L_1}\Big) \label{eq: yerr_0}
    \end{align}
    where (i) uses $\ln(1-x)\le -x<0$ for $x=\kappa^{-1}\in(0,1)$ and eq. \eqref{eq: Nt1}. Hence, eq. \eqref{eq: yerr_t1} holds for Output I when $t=0$.
        
    Suppose eq. \eqref{eq: yerr_t1} holds for $t=k-1$. Then, eq. \eqref{eq: 8} implies that
    \begin{align}
        &\|y_{k+1} - y^*(x_{k}) \| \nonumber\\
        &\le (1-\kappa^{-1})^{N_k}\|y_{k} - y^*(x_{k-1})\| + (1-\kappa^{-1})^{N_k}\|y^*(x_{k-1}) - y^*(x_{k})\| \nonumber\\
        &\overset{(i)}{\le} \exp\big(N_k\ln(1-\kappa^{-1})\big) \Big(\min\Big(\frac{\alpha\|s_{k-1}\|}{L_G},\frac{\beta\|s_{k-1}\|^2}{L_1}\Big)+\kappa\|s_k\|\Big) \nonumber\\
        &\overset{(ii)}{\le} \exp\Big(-\ln\frac{(\alpha\|s_{k-1}\|/L_G)\wedge (\beta\|s_{k-1}\|^2/L_1)+\kappa\|s_k\|}{(\alpha\|s_k\|/L_G)\wedge(\beta\|s_k\|^2/L_1)}\Big) \Big(\Big(\frac{\alpha\|s_{k-1}\|}{L_G}\wedge\frac{\beta\|s_{k-1}\|^2}{L_1}\Big)+\kappa\|s_k\|\Big) \nonumber\\
        &=\frac{\alpha\|s_k\|}{L_G} \wedge \frac{\beta\|s_k\|^2}{L_1}\label{eq: yerr_1a}
    \end{align}
    where (i) uses eq. \eqref{eq: yerr_t1} for $t=k-1$ and the fact that $y^*$ is $\kappa$-Lipschitz mapping (see \cite{lin2019gradient,chen2021proximal} for the proof) and (ii) uses $\ln(1-\kappa^{-1})\le -\kappa^{-1}$ and eq. \eqref{eq: Nt1}. Therefore, eq. \eqref{eq: yerr_t1} holds for $t=k$ and thus for all $t\in [0,T-1]$.
    
    Hence, eqs. \eqref{eq: grad_goal_noKL} \& \eqref{eq: Hess_goal_noKL} with $\epsilon'=0$ in Lemma \ref{lemma_ifErrSmall_noKL} can be proved as follows.
    \begin{align}
    \|\nabla\Phi(x_t)-\nabla_1 f(x_t, y_{t+1})\|&=\|\nabla_1 f(x_t,y^*(x_t))-\nabla_1 f(x_t, y_{t+1})\| \le L_1\|y_{t+1}-y^*(x_t)\| \le \beta\|s_t\|^2,\label{eq: dfKL}
    \end{align}
    \begin{align}
    \|\nabla^2\Phi(x_t)-G(x_t,y_{t+1})\|&=\|G(x_t,y^*(x_t))-G(x_t, y_{t+1})\| \le L_G\|y_{t+1}-y^*(x_t)\| \le\alpha\|s_t\|.\label{eq: dGKL}
    \end{align}
    Note that $\epsilon'=0$ implies that $T'=+\infty$, so eq. \eqref{eq: Hdec2_noKL} in Lemma \ref{lemma_ifErrSmall_noKL} holds for all $t\ge 0$. Therefore, eq. \eqref{eq: potential} holds for Output I of Algorithm \ref{algo: prox-minimax}. 
    
    The proof for Output II follows the same logic as that for Output I. The major difference is that the lower bound of $N_t$ changes as follows. 
    \begin{align}
        \left\{ \begin{gathered}
        N_0\ge \kappa\ln\big(L_1\|y_0-y^*(x_0)\|/(2\beta\epsilon'^2)\big)\hfill\\
	    N_t\ge \kappa\ln\Big(\frac{2L_1\alpha\|s_{t-1}\|+L_1(\alpha+L_G\kappa)\|s_t\|}{L_G\beta\epsilon'^2}\Big)=\mathcal{O}\Big(\kappa\ln \frac{L_1\alpha \|s_{t-1}\|+ L_1(\alpha+L_2\kappa)\|s_t\|}{L_G\beta\epsilon'^2}\Big); 1\le t\le T'.\\
	    \end{gathered}  \right., \label{eq: Nt2}
    \end{align}
    which by a similar induction argument yields that
	\begin{align}
    \|y_{t+1}-y^*(x_t)\|\le& \frac{\alpha(\|s_t\|+\epsilon')}{L_G}\wedge\frac{\beta(\|s_t\|^2+\epsilon'^2)}{L_1}; 0\le t\le T'-1. \label{eq: yerr_t2}
    \end{align}
    We briefly sketch the induction here. 
    
    When $t=0$, on one hand, eq. \eqref{eq: 8} implies that
    \begin{align}
        \|y_1-y^*(x_0)\|&\le \|y_0-y^*(x_0)\|\exp\big(N_0\ln(1-\kappa^{-1})\big) \nonumber\\
        &\overset{(i)}{\le} \|y_0-y^*(x_0)\|\exp\Big(-\ln\Big(\frac{L_1\|y_0-y^*(x_0)\|}{2\beta\epsilon'^2}\Big)\Big) \le \frac{2\beta\epsilon'^2}{L_1} \label{eq: yerr_0}
    \end{align}
    where (i) uses $\ln(1-x)\le -x<0$ for $x=\kappa^{-1}\in(0,1)$ and eq. \eqref{eq: Nt2}. On the other hand, the right side of eq. \eqref{eq: yerr_t2} is simplified as follows. 
    \begin{align}
        \frac{\alpha(\|s_0\|+\epsilon')}{L_G}\wedge\frac{\beta(\|s_0\|^2+\epsilon'^2)}{L_1} \overset{(i)}{=}  \frac{2\alpha\epsilon'}{L_G}\wedge\frac{2\beta\epsilon'^2}{L_1}\overset{(ii)}{=} \frac{2\beta\epsilon'^2}{L_1}, \label{eq: yerr_0b}
    \end{align}
    where (i) uses the definition $\|s_0\| = \epsilon'$ and (ii) uses the condition that $\epsilon'\le \frac{\alpha L_1}{\beta L_G}$.
    Hence, eq. \eqref{eq: yerr_t2} holds for Output I when $t=0$.
    
    If eq. \eqref{eq: yerr_t2} holds for $t=k-1\in[0,T'-2]$, then
    \begin{align}
        &\|y_{k+1} - y^*(x_{k}) \| \nonumber\\
        &\le  (1-\kappa^{-1})^{N_k}\|y_{k} - y^*(x_{k-1})\| + (1-\kappa^{-1})^{N_k}\|y^*(x_{k-1}) - y^*(x_{k})\| \nonumber\\
        &\overset{(i)}{\le} \exp\big(N_k\ln(1-\kappa^{-1})\big) \Big(\Big(\frac{\alpha(\|s_{k-1}\|+\epsilon')}{L_G}\wedge\frac{\beta(\|s_{k-1}\|^2+\epsilon'^2)}{L_1}\Big)+\kappa\|s_k\|\Big) \nonumber\\
        &\overset{(ii)}{\le} \exp\Big(-\ln\Big(\frac{2L_1\alpha\|s_{k-1}\|+L_1(\alpha+L_G\kappa)\|s_k\|}{L_G\beta\epsilon'^2}\Big)\Big) \Big(\frac{\alpha(\|s_{k-1}\|+\epsilon')}{L_G} + \kappa\|s_k\|\Big) \nonumber\\
        &\overset{(iii)}{\le}\frac{L_G\beta\epsilon'^2}{2L_1\alpha\|s_{k-1}\|+L_1(\alpha+L_G\kappa)\|s_k\|} \frac{\alpha(2\|s_{k-1}\|+\|s_k\|)+L_G\kappa\|s_k\|}{L_G}\nonumber\\ &=\frac{\beta\epsilon'^2}{L_1}\overset{(iv)}{=}\frac{\alpha\epsilon'}{L_G}\wedge\frac{\beta\epsilon'^2}{L_1}\le \frac{\alpha(\|s_k\|+\epsilon')}{L_G}\wedge\frac{\beta(\|s_k\|^2+\epsilon'^2)}{L_1} \nonumber
    \end{align}
    where (i) uses eq. \eqref{eq: yerr_t2} for $t=k-1$ and the fact that $y^*$ is $\kappa$-Lipschitz mapping (see \cite{lin2019gradient,chen2021proximal} for the proof), (ii) uses $\ln(1-\kappa^{-1})\le -\kappa^{-1}$ and eq. \eqref{eq: Nt2}, (iii) uses $\epsilon'\le \|s_{k-1}\|\vee\|s_k\|\le \|s_{k-1}\|+\|s_k\|$ for $k\le T'-1$, and (iv) uses the condition that $\epsilon'\le \frac{\alpha L_1}{\beta L_G}$. This proves eq. \eqref{eq: yerr_t2} holds for $t=k$ and thus for all $t\in[0,T'-1]$, which further implies eqs. \eqref{eq: grad_goal_noKL} \& \eqref{eq: Hess_goal_noKL}. Hence, by Lemma \ref{lemma_ifErrSmall_noKL}, we prove that eq. \eqref{eq: potential} holds for output II for all $0\le t\le T'-1$. 
\end{proof}



==> 20230217 CubicMinimax_ArXiV_underTMLRreview/remove.tex <==
\section{Two Objective Functions (to remove)}
\begin{align}
    L(s,v):=&\nabla_{\!1}f(x_t,\! y_{t+1})^{\!\top}\!s +  \zeta_{x_t,y_{t+1}}(s,v)+\frac{1}{6\eta_x}\|s\|^3 \label{eq:inexact_CRobj}\\
    L^*(s):=&L(s,v^*(s))=\nabla_{\!1}f(x_t,\! y_{t+1})^{\!\top}\!s + \frac{1}{2} s^{\!\top}G(\!x_t,\! y_{t+1}\!)s+\frac{1}{6\eta_x}\|s\|^3 \label{eq:exact_CRobj}
\end{align}

\section{See GD step in GDA as GD of CR with approximate gradient (to remove)}
Approximate gradient using $v_h\approx v^*(s)$ obtained by $h$ gradient ascent steps:
\begin{align}
    g_h=\nabla_{\!1}f(x_t,\!y_{t+1}) + \nabla_{11}f(x_t,\!y_{t+1}) s + \nabla_{12}f(x_t,\!y_{t+1}) v_h +\frac{1}{2\eta_x}\|s\|s
\end{align}

True gradient (when $v=v^*(s)$ above): 
\begin{align}
	g=\nabla_{\!1}f(x_t,\!y_{t+1}) + G(x_t,\!y_{t+1})s +\frac{1}{2\eta_x}\|s\|s. 
\end{align}

Gradient error bound:
\begin{align}
    \|g_h-g\|&=\|\nabla_{12}f(x_t,\!y_{t+1}) (v_h-v^*(s))\|\nonumber\\
    &\le L(1-\kappa^{-1})^h\|v_0-v^*(s)\|\nonumber\\
    &\overset{(i)}{\le} L\kappa(1-\kappa^{-1})^h\|s\|,\nonumber
\end{align} 
where (i) uses $v_0=0$ and $\|v^*(s)\|=\|\nabla_{22}^{-1}f(x,y) \nabla_{21}f(x,y)s\|\le \kappa\|s\|$. 

The gradient pertrubation is reflected in eq. (8) and the beginning of Lemma A.2 proof in \cite{carmon2019gradient}

Question: 
Axact GD: $O(d^2$) to obtain exact $v^*$
Gradient Descent Efficiently Finds the Cubic-Regularized Non-Convex Newton Step.pdf 
From function value gap to (via eq. (5) with $\rho||s^*||>=\gamma$)

Approximate GD (GDA): $O(\ln(1-1/\kappa))$ to obtain approximate $v^*$. 

keep both? Also GD analysis is the basis of GDA analysis. 

\section{Exact GD (to remove)}
Convergence rate with $K$ GD iterations  (Theorems 3.1 and 3.2 of \cite{carmon2019gradient}):
\begin{align}
    L^*(s_K)-L^*(s^*)\le \widetilde{\mathcal{O}}(1/K). \nonumber
\end{align}
Then if $\frac{\|s^*\|}{2\eta_x}\ge \frac{\epsilon'}{2\eta_x}\ge -2\lambda_{\min}[G(x_t,y_{t+1})]\approx -2\mu$ (as $y_{t+1}\approx y^*(x_t)$), we have
\begin{align}
    L^*(s_K)-L^*(s^*)&=\frac{1}{2}(s_K-s^*)^{\top}\Big(G(x_t,y_{t+1})+\frac{\|s^*\|}{2\eta_x}I\Big)(s_K-s^*) + \frac{1}{12\eta_x}(\|s^*\|-\|s_K\|)^2(\|s^*\|+2\|s_K\|) \nonumber\\
    &\ge -\frac{1}{2}\lambda_{\min}[G(x_t,y_{t+1})]\|s_K-s^*\|^2 \nonumber
\end{align}
Then use $\|s_K-s^*\|\le \widetilde{\mathcal{O}}(K^{-1/2})$ to obtain 3 approximate optimality conditions for $s_K$.

Challenge: What if $\|s^*\|<\epsilon'$ for some outer iteration $t$? 

\section{Stationary point of CR minimax (to remove)}
\begin{align}
&\nabla_{\!1}f(x_t,\!y_{t+1}) + \nabla_{11}f(x_t,\!y_{t+1}) s + \nabla_{12}f(x_t,\!y_{t+1}) v +\frac{1}{2\eta_x}\|s\|s=0 \label{stat1}\\
&\nabla_{21}f(x_t,\!y_{t+1})s + \nabla_{22}f(x_t,\!y_{t+1}) v =0 \label{stat2}
\end{align}
Eq. \eqref{stat2} implies that $v=-\nabla_{22}f(x_t,\!y_{t+1})^{-1}\nabla_{21}f(x_t,\!y_{t+1})s$. Substitute that into eq. \eqref{stat1} yields that
\begin{align}
	\nabla_{\!1}f(x_t,\!y_{t+1}) + \nabla_{11}f(x_t,\!y_{t+1}) s - \nabla_{12}f(x_t,\!y_{t+1})\nabla_{22}f(x_t,\!y_{t+1})^{-1}\nabla_{21}f(x_t,\!y_{t+1})s +\frac{1}{2\eta_x}\|s\|s=0, \nonumber
\end{align}
i.e.,
\begin{align}
	\nabla_{\!1}f(x_t,\!y_{t+1}) + G(x_t,\!y_{t+1})s +\frac{1}{2\eta_x}\|s\|s=0, \nonumber
\end{align}
which is exactly the same as the stationary condition of the CR problem. 

\section{Inexact GD convergence analysis for cubic-regularization subproblem}
% \begin{assum}\label{assum: f}
% 	The minimax problem $\mathrm{(P)}$ satisfies:
% 	\begin{enumerate}[leftmargin=*,topsep=0mm,itemsep=1mm]
% 		\item Function $f(\cdot,\cdot)$ is $L_1$-smooth and function $f(x,\cdot)$ is $\mu$-strongly concave for any fixed $x$;
% 		\item The Jacobian mappings $\nabla_{11} f$, $\nabla_{12} f$, $\nabla_{21} f$, $\nabla_{22} f$ are $L_2$-Lipschitz continuous;
% 		\item Function $\Phi(x):=\max_{y\in \mathbb{R}^n} f(x,y)$ is bounded below and has compact sub-level sets.
% 	\end{enumerate}
% \end{assum} 

Denote 
\begin{align}
    R:=\sqrt{L_1^2L_2^2(1+\kappa)^2+4L_2\|g\|}-L_1L_2(1+\kappa)
\end{align}
\begin{align}
    \|G(x,y)\|\le 2L_1\kappa (=\beta in \cite{carmon2019gradient})
\end{align}

$2\rho$ in \cite{carmon2019gradient} corresponds to our $1/\eta_x$. 

$\text{gap}=\lambda_{\max}(A)-\lambda_{\min}(A)$ in \cite{carmon2019gradient} corresponds to our $\text{gap}\le 4L_1\kappa$. 

$\gamma=-\lambda_{\min}(A)$ in \cite{carmon2019gradient} corresponds to our $|\gamma|\in 2L_1\kappa$. 



\section{Try directly see the perturbation error of the final result (To remove later)}
\begin{align}
    f(s)=b^{\top}s+\frac{1}{2}s^{\top}As+\frac{\rho}{3}\|s\|^3\nonumber
\end{align}
Let $s_0=\widetilde{s}_0$ and stepsize $\eta=\frac{1}{4(\|A\|+\rho R)}$.
\begin{align}
	s_{t+1}=s_t-\eta \nabla f(s_t), \quad \widetilde{s}_{t+1}=\widetilde{s}_t-\eta \big(\nabla f(\widetilde{s}_t)+d_t\big).\nonumber
\end{align}

% \subsection{Find $s_{\max}$ such that $\|\widetilde{s}_t\|\le s_{\max}$}
% Let $0\le s_{\text{in}}\le s_{\max}$ be such that
% \begin{align}
%     &s_{\text{in}}+\eta (\|b\|+\|A\|s_{\text{in}}+\rho s_{\text{in}}^2) \le s_{\max} \nonumber\\
%     &d 
% \end{align}

% \subsection{Proof of convergence rate}
Suppose the $t$-th CR-GD iteration takes $h_t$ maximum steps, then 
\begin{align}
\|d_t\|\le L\kappa(1-\kappa^{-1})^{h_t} s_{\max}. \nonumber
\end{align}

Therefore,
\begin{align}
	&\|\widetilde{s}_1-s_1\|=\eta\|d_0\|.\nonumber	
\end{align}
\begin{align}
	\|\widetilde{s}_{t+1}-s_{t+1}\|&\le \|\widetilde{s}_t-s_t\|+\eta\|\nabla f(s_t)-\nabla f(\widetilde{s}_t)\|+\eta\|-d_t\| \nonumber\\
	&\le (1+\eta L_{CR})\|\widetilde{s}_t-s_t\|+\eta\|d_t\| \nonumber
\end{align}
where $f(s)$ is $L_{CR}:=\|A\|+2\rho s_{\max}$-smooth when $\|s\|\le s_{\max}$. 
\begin{align}
	\|\widetilde{s}_t-s_t\|&\le \eta \sum_{t'=0}^{t-1} (1+\eta L_{CR})^{t-1-t'}\|d_{t'}\|\nonumber\\
	&\le L\kappa\eta s_{\max}\sum_{t'=0}^{t-1} (1+\eta L_{CR})^{t-1-t'}(1-\kappa^{-1})^{h_{t'}}\label{ds_general}
\end{align}
The CR-GD paper proved that
\begin{align}
	f(s_t)-f(s^*)\le \frac{\epsilon}{2} \label{CRGD_eps}
\end{align}
if 
\begin{align}
    t\ge \frac{120\|s^*\|^2}{\eta\epsilon} \ln\Big(\frac{2\|s^*\|^2(\|A\|+2\rho\|s^*\|)}{\epsilon}\Big(1+\frac{\lambda_1^2}{4\rho|b^{\top}q_1|}\Big)\Big):=C\epsilon^{-1}\ln(\epsilon^{-1})\nonumber
\end{align}
where $Aq_j=\lambda_jq_j$ with $\lambda_1\le\ldots\le\lambda_d$ and $\|q_j\|=1$. ($|b^{\top}q_1|\ge \epsilon$ with high probability after uniform perturbation.) 

Based on eq. \eqref{CRGD_eps}, to ensure that $f(\widetilde{s}_t)-f(s^*)\le\epsilon$, we simply need $\|\widetilde{s}_t-s_t\|\le \frac{\epsilon}{2\ell_{CR}}$ where $f(s)$ is $\ell_{CR}:=\|b\|+\|A\|s_{\max}+\rho s_{\max}^2$-Lipschitz when $\|s\|\le s_{\max}$. This combined with eq. \eqref{ds_general} yields the condition that
\begin{align}
    \sum_{t'=0}^{t-1} (1+\eta L_{CR})^{t-1-t'}(1-\kappa^{-1})^{h_{t'}} \le \frac{\epsilon}{2\ell_{CR}L\kappa\eta s_{\max}}. \nonumber
\end{align}
The following choice of $h_t$ satisfies the above.
\begin{align}
    h_{t'}=\Big\lceil \frac{\kappa}{2}\big(\ln(2\ell_{CR}L\kappa\eta s_{\max}\epsilon^{-1})+(t-1-t')\ln(1+\eta L_{CR})\big)\Big\rceil
\end{align}





==> 20230217 CubicMinimax_ArXiV_underTMLRreview/stochastic.tex <==
\section{Sub-Sampled Stochastic Cubic-GDA }\label{sec: stoc}

In this section, we apply stochastic sub-sampling to further improve the performance and complexity of Cubic-GDA in large-scale nonconvex minimax optimization with big data. Specifically, we consider the following stochastic finite-sum minimax optimization problem (Q). 
\begin{align}
	\min_{x\in \mathbb{R}^m}\max_{y\in \mathbb{R}^n}~ f(x,y):= \frac{1}{N}\sum_{i=1}^N f_i(x,y), \tag{Q}
\end{align} 
where $N$ denotes the total number of training samples and $f_i$ corresponds to the loss function on the $i$-th sample. We adopt the following assumptions. 

\begin{assum}\label{assum: fi}
	The stochastic minimax optimization problem $\mathrm{(Q)}$ satisfies:
	\begin{enumerate}[leftmargin=*,topsep=0mm,itemsep=1mm]
		\item For any sample $i$, function $f_i(\cdot,\cdot)$ is $L_1$-smooth, function $f_i(\cdot,y)$ is $L_0$-Lipschitz for any fixed $y$, and function $f_i(x,\cdot)$ is $\mu$-strongly concave for any fixed $x$;
		\item For any sample $i$, the Jacobian mappings $\nabla_{11} f_i$, $\nabla_{12} f_i$, $\nabla_{21} f_i$, $\nabla_{22} f_i$ are $L_2$-Lipschitz continuous;
		\item Function $\Phi(x):=\max_{y\in \mathbb{R}^n} f(x,y)$ is bounded below and has compact sub-level sets.
	\end{enumerate}
\end{assum} 

Applying Cubic-GDA to solve the above problem (Q) would require querying full partial gradients and full Jacobian matrices that involve all the training samples. Instead, it is more efficient to approximate these quantities via stochastic sub-sampling. Therefore, we propose a \textbf{stochastic Cubic-GDA} algorithm, which replaces the exact quantities $\nabla_1 f$ and $G$ involved in the cubic update by their corresponding stochastic approximations. 

Specifically, to approximate the partial gradient $\nabla_1 f$, we sub-sample a mini-batch of samples $B_1$ with replacement from the training set and construct the following sample average approximation. 
\begin{align}
    \widehat{\nabla}_1 f(x,y) &= \frac{1}{|B_1|} \sum_{i \in B_1} \nabla_1 f_i(x,y). \label{eq: stoc_f1}
\end{align}
On the other hand, to approximate the matrix $G$, we sub-sample mini-batches of samples $B_{11}, B_{12}, B_{21}, B_{22}$ with replacement and construct approximated Jacobian matrices $\widehat{\nabla}_{11} f, \widehat{\nabla}_{12} f, \widehat{\nabla}_{21} f, \widehat{\nabla}_{22} f$ in the same way as above. Then, we construct the following approximation of $G$.
\begin{align}
    \widehat{G}(x,y) = \big[\widehat{\nabla}_{11} f - \widehat{\nabla}_{12} f (\widehat{\nabla}_{22}f)^{-1} \widehat{\nabla}_{21} f\big](x,y). \label{eq: stocG}
\end{align}
We summarize the update rule of stochastic Cubic-GDA in \Cref{algo: prox-minimax-stoc} below.
In particular, we run stochastic gradient ascent in the inner iterations to obtain the approximated maximizer $y_{t+1}$, and its high-probability convergence rate has been established in the stochastic optimization literature \citep{harvey2019simple}. 

\begin{algorithm}
	\caption{Stochastic Cubic-GDA}\label{algo: prox-minimax-stoc}
	{\bf Input:} Initialize $x_0,y_0$, learning rates $\eta_{x}$, threshold $\epsilon'$ \\
	{Define $\|s_0\|=\epsilon'$} \\
	\For{ $t=0,1, 2,\ldots, T-1$}{
	    Initialize $\widetilde{y}_0 = y_t$
	    
        \For{$k=0,1, 2,\ldots, N_t-1$}{
            Query a sample $\xi$ to compute $\nabla_2 f_{\xi}(x_t, \widetilde{y}_k)$\\
            $\widetilde{y}_{k+1} = \widetilde{y}_k + \frac{2}{\mu(k+1)} \nabla_2 f_{\xi}(x_t, \widetilde{y}_k)$
        }
        
        Set $y_{t+1} = \sum_{k=0}^{N_t-1}\frac{2k}{N_t(N_t-1)}\widetilde{y}_{k}$
        
        Sample minibatch $B_1(t),B_{11}(t),B_{12}(t),B_{21}(t),B_{22}(t)$ to compute \cref{eq: stoc_f1} and \cref{eq: stocG}. Then, solve the following cubic problem for $s_{t+1}$:
        
        $\mathop{\arg\!\min}_s \!\widehat{\nabla}_{\!1}f(x_t,\! y_{t+1})^{\!\top}\!s + \frac{1}{2} s^{\!\top}\widehat{G}(x_t,\! y_{t+1}\!)s+\frac{1}{6\eta_x}\|s\|^3$
        
        Update $x_{t+1}=x_t+s_{t+1}$
	}
	\textbf{Output:}  $x_{T'},y_{T'}$ with 
	$T'=\min\{t: \|s_{t-1}\|\vee\|s_t\|\le\epsilon'\}$
\end{algorithm}

The following lemma characterizes the sample complexities of all the stochastic approximators for achieving a certain approximation accuracy.


\begin{restatable}{lemma}{lemmaBatch}\label{lemma: batch}
    Fix any $0<\epsilon_1 \le 2L_0$, $0<\epsilon_2{\le 4L_1}$ and choose the following batch sizes
    \begin{align}
    |B_1| &\ge \mathcal{O}\Big(\frac{L_0^2}{\epsilon_1^{2}}\ln\frac{m}{\delta} \Big), \label{eq: b1}\\  
    |B_{11}|,|B_{12}|,|B_{21}|,|B_{22}|&\ge \mathcal{O}\Big(\frac{L_1^2}{\epsilon_2^{2}} \ln\frac{m+n}{\delta}\Big). \label{eq: b2}
    \end{align}
    Then, the stochastic approximators satisfy the following error bounds with probability at least $1-\delta$.
    \begin{align}
        &\|\widehat{\nabla}_1 f(x,y)-\nabla_1 f(x,y)\|\le \epsilon_1,\label{eq: stoc_err1}\\ 
        &\|\widehat{\nabla}_{k\ell}^2 f(x,y) \!-\! \nabla_{k\ell}^2 f(x,y)\|\le \epsilon_2, ~ \forall k,\ell \in \{1,2\},\label{eq: stoc_err2}\\ 
        &\|\widehat{G}(x,y)-G(x,y)\|\le (\kappa+1)^2\epsilon_2.\label{eq: stoc_err3}
    \end{align}
\end{restatable}

Therefore, by choosing proper batch sizes, the inexactness of the stochastic gradient, Jacobian and Hessian estimators can be controlled within a desired range. From this perspective, stochastic Cubic-GDA can be viewed as an inexact version of the Cubic-GDA algorithm. 

To characterize the convergence and sample complexity of stochastic Cubic-GDA, we adopt an adaptive inexactness criterion for the sub-sampling scheme. Specifically, we choose time-varying batch sizes in a way such that the gradient and Jacobian inexactness in iteration $t$ are proportional to the previous increment, i.e., $\epsilon_1(t)\propto \|s_t\|^2, \epsilon_2(t)\propto \|s_t\|$. Such an
adaptive inexact criterion is justified in the cubic regularization literature \citep{wang2018note,wang2019stochastic} with the following advantages: 1) it is adapted to the optimization increment and hence leads to reduced batch sizes when the increment is large in the early iterations; 2) it makes the batch size scheduling scheme in \Cref{lemma: batch} practical, as the batch sizes in iteration $t$ now depend on the increment $\|s_t\|$ obtained in the previous iteration $t-1$. We also note that since the sub-sampling scheme is adapted to the previous increment, the output rule of \Cref{algo: prox-minimax-stoc} is designed to control the value of both the current and the previous increments. This termination rule is critical to bound the adapted gradient and Jacobian inexactness in the analysis. 


We obtain the following global convergence and sample complexity result of stochastic Cubic-GDA.

\begin{restatable}[Convergence and sample complexity]{thm}{thmstoc}\label{thm: 5}
    Let Assumption \ref{assum: fi} and \Cref{lemma: SGA} hold. For $0<\epsilon\le \frac{L_1\sqrt{33L_{\Phi}}}{L_G}$, choose $\epsilon'=\frac{\epsilon}{\sqrt{33L_{\Phi}}}$, $\eta_x\le \frac{1}{55L_{\Phi}}$, $T\ge \frac{\Phi(x_0)-\Phi^*+8L_{\Phi}\epsilon'^2}{3L_{\Phi}\epsilon'^3}$ and $N_t\ge\mathcal{O}\big(\frac{L_0\ln(1/\delta)+L_0^2}{\kappa^{-2}(L_{\Phi}^2\|s_t\|^4+\epsilon^4)\wedge L_1^2(\|s_t\|^2+\epsilon^2/L_{\Phi})}\big)$. Moreover, in iteration $t$, choose the batch sizes according to \cref{eq: b1,eq: b2} with the inexactness given by
    \begin{align}
        \epsilon_1(t)=&\frac{L_{\Phi}}{2}\Big(\|s_t\|^2+\frac{\epsilon^2}{33L_{\Phi}}\Big)\wedge 2L_0, \nonumber\\
        \epsilon_2(t)=&\frac{L_{\Phi}}{2(\kappa+1)^2}\Big(\|s_t\|+\frac{\epsilon}{\sqrt{33L_{\Phi}}}\Big)\wedge 4L_1. \nonumber
\end{align}
    Then, the output of {Stochastic Cubic-GDA} satisfies
    \begin{align}
       \mu(x_{T'}) \le \epsilon. \label{eq: gH_rate2}
    \end{align}
    Consequently, the total number of cubic iterations satisfies $T'\le \mathcal{O}(\sqrt{L_2}\kappa^{1.5}\epsilon^{-3})$, the total number of queried gradient samples satisfies $\sum_{t'=0}^{T'}\big(N_t+|B_1(t)|\big)\le\mathcal{O}\Big(\frac{L_0^2\kappa^{3.5}\sqrt{L_2}}{\epsilon^7}\ln\frac{m}{\delta}\Big)$, and the total number of queried Jacobian samples satisfies  $\sum_{t=0}^{T'-1}\sum_{k=1}^2\sum_{\ell=1}^2|B_{k,\ell}(t)|\le \mathcal{O}\big( \frac{L_1^2\kappa^{2.5}}{\sqrt{L_2}\epsilon^5}\ln\frac{m+n}{\delta}\big)$. 
\end{restatable}
Therefore, under adaptive sub-sampling, the induced gradient and Jacobian inexactness $\epsilon_1(t), \epsilon_2(t)$ are properly controlled so that the iteration complexity $T'$ of stochastic Cubic-GDA remains in the same level as that of Cubic-GDA. Moreover, as opposed to the sample complexity of Cubic-GDA that scales linearly with regard to the data size $N$, the sample complexity of stochastic Cubic-GDA is independent of $N$. For example, by comparing the 
more expensive Jacobian sample complexity between Cubic-GDA and stochastic Cubic-GDA, we conclude that stochastic sub-sampling helps reduce the sample complexity so long as the data size is large enough, i.e., $N\ge \widetilde{\mathcal{O}}\Big(\frac{L_1^2\kappa}{L_2\epsilon^2}\Big)$.

%We compare the above complexity result of stochastic Cubic-GDA with that of Cubic-GDA on the finite-sum minimax optimization problem (Q). Note that Cubic-GDA computes full gradients and Hessians, each of which requires to compute $N$ samples. Therefore, based on Theorem \ref{thm: 1b}, to achieve $\mu(x_{T'}) \le \epsilon$, the total numbers of required gradient and Hessian computations for Cubic-GDA are respectively $N+N\sum_{t=0}^{T'} N_t\le \mathcal{O}(N\sqrt{L_2}\kappa^{2.5}\epsilon^{-3})$ and $4NT'\le \mathcal{O}(N\sqrt{L_2}\kappa^{1.5}\epsilon^{-3})$, which are respectively larger than those required by stochastic Cubic-GDA when the number of training samples is sufficiently large, i.e., $N\ge \widetilde{\mathcal{O}}\Big(\frac{L_0^2\kappa}{\epsilon^4}\vee \frac{L_1^2\kappa}{L_2\epsilon^2}\Big)$. 




==> 20230217 CubicMinimax_ArXiV_underTMLRreview/thm1bproof.tex <==
\section{Proof of Theorem \ref{thm: 1b}}\label{sec: thm2}
\thmglobalrate*

% [to remove] Let \Cref{assum: f} hold. For any $\alpha, \beta>0$, choose $\epsilon'\le \frac{\alpha L_1}{\beta L_G}$, $\eta_x\le (9L_{\Phi}+18\alpha+28\beta)^{-1}$ and $\eta_y\le \frac{2}{L+\mu}$. Then, Outputs I $\&$ II of \Cref{algo: prox-minimax} satisfy the following potential decrease property respectively in the cases listed below.
% \begin{align}
%     H_{t+1}-H_t \le -(L_{\Phi}+\alpha+\beta)(\|s_{t+1}\|^3+\|s_t\|^3). 
% \end{align}
% \begin{itemize}[leftmargin=*,topsep=0mm,itemsep=1mm]
%     \item Output I: choose $N_t \ge \mathcal{O} \big( \kappa\ln \frac{t\alpha\|s_{t-1}\|+t^{1/4}\alpha\epsilon'+ t\kappa\|s_t\|}{\beta\epsilon'^2} \big)$, \red{$T\ge \frac{\Phi(x_0)-\Phi^*+8L_{\Phi}\epsilon'^2}{\epsilon'^3(L_{\Phi}+\alpha+\beta)}$}. Then, for all $0\le t~\le T-1$, \cref{eq: potential}
%     holds with $H_t=\Phi(x_t)+(L_{\Phi}+2\alpha+3\beta)\|s_t\|^2+a_t\epsilon'^3\big(\frac{\alpha}{2}+\beta\big)$, where $a_t = 6\pi^{-2} - \sum_{k=1}^{t-1}k^{-2} \downarrow 0$;
%     \item Output II: choose $N_t\ge \mathcal{O}\big(\kappa\ln \frac{\alpha \|s_{t-1}\|+ (\alpha+\kappa)\|s_t\|}{\beta\epsilon'^2}\big)$. Then, for all $0\le t\le T'-1$, \cref{eq: potential}
%     holds with $H_t:=\Phi(x_t)+(L_{\Phi}+2\alpha+3\beta)\|s_t\|^2$.
% \end{itemize}

\begin{proof}%[Proof of Theorem \ref{thm: 1b}]
Substituting $\alpha=\beta=L_{\Phi}=L_2(1+\kappa)^3$ and $\epsilon'=\frac{\epsilon}{\sqrt{33L_{\Phi}}}$ into Lemma \ref{lemma_general_rate} yields that when $T\ge \sqrt{33L_{\Phi}}\frac{33(\Phi(x_0)-\Phi^*)+8\epsilon^2}{3\epsilon^3}$ and $\eta_x=(55L_{\Phi})^{-1}$, we have $T'\le \sqrt{33L_{\Phi}}\frac{33(\Phi(x_0)-\Phi^*)+8\epsilon^2}{3\epsilon^3}=\mathcal{O}\big(\sqrt{L_2}\kappa^{1.5}\epsilon^{-3}\big)\le T$, and moreover,
\begin{align}
    &\|\nabla \Phi(x_{T'})\| \le \Big(\frac{1}{2\eta_x}+L_{\Phi}+2\alpha+2\beta\Big) \epsilon'^2 \le \epsilon^2, \nonumber\\
    &\lambda_{\min}\big(\nabla^2 \Phi(x_{T'})\big) \ge -\Big(\frac{1}{2\eta_x}+L_{\Phi}+2\alpha\Big)\epsilon' \ge -\sqrt{33L_{\Phi}}\epsilon. \nonumber
\end{align}
This proves eq. \eqref{eq: gH_rate1}. 

Note that the number of gradient ascent iterations $N_t$ should satisfy eq. \eqref{eq: Nt2}. Substituting $\alpha=\beta=L_{\Phi}=L_2(1+\kappa)^3$ and $\epsilon'=\frac{\epsilon}{\sqrt{33L_{\Phi}}}$ into eq. \eqref{eq: Nt2} yields that
\begin{align}
    \left\{ \begin{gathered}
    N_0\ge \kappa\ln\big(L_1\|y_0-y^*(x_0)\|/(2\beta\epsilon'^2)\big) = \kappa\ln\big(33L_1\|y_0-y^*(x_0)\|/(2\epsilon^2)\big) \hfill\\
    N_t\ge \kappa\ln\Big(\frac{2L_1\alpha\|s_{t-1}\|+L_1(\alpha+L_G\kappa)\|s_t\|}{L_G\beta\epsilon'^2}\Big)\overset{(i)}{=}\kappa\ln\Big(\frac{66L_1(1+\kappa)\|s_{t-1}\|+33L_1(2+\kappa)\|s_t\|}{\epsilon^2}\Big); 1\le t\le T'\\
    \end{gathered}  \right., \nonumber
\end{align}
where (i) uses $L_G=L_2(1+\kappa)^2$ and $L_{\Phi}=L_2(1+\kappa)^3$ in \Cref{prop_Phiystar}. 

When we select $N_t$ such that the above holds with equality, then the total number of gradient ascent iterations is upper bounded as follows
\begin{align}
    \sum_{t=0}^{T'-1} N_t&= \kappa\ln\big(33L_1\|y_0-y^*(x_0)\|/(2\epsilon^2)\big) + \kappa\sum_{t=0}^{T'-1} \ln\Big(\frac{66L_1(1+\kappa)\|s_{t-1}\|+33L_1(2+\kappa)\|s_t\|}{\epsilon^2}\Big) \nonumber\\
    &\le \kappa\ln\big(33L_1\|y_0-y^*(x_0)\|/(2\epsilon^2)\big) + \kappa \sum_{t=0}^{T'-1} \ln\big(\|s_{t-1}\|+\|s_t\|\big)  +\kappa T'\ln \big(66L_1\epsilon^{-2}(1+\kappa)\big) \nonumber\\
    &\overset{(i)}{\le} \kappa\ln\big(33L_1\|y_0-y^*(x_0)\|/(2\epsilon^2)\big) + \frac{\kappa T'}{3} \frac{1}{T'}\sum_{t=0}^{T'-1} \ln\big(4\|s_{t-1}\|^3+4\|s_t\|^3\big) +\kappa T'\ln \big(66L_1\epsilon^{-2}(1+\kappa)\big) \nonumber\\
    &\overset{(ii)}{\le} \kappa\ln\big(33L_1\|y_0-y^*(x_0)\|/(2\epsilon^2)\big) + \frac{\kappa T'}{3} \ln\Big(\frac{4}{T'}\sum_{t=0}^{T'-1} \big(\|s_{t-1}\|^3+\|s_t\|^3\big)\Big) +\kappa T'\ln \big(66L_1\epsilon^{-2}(1+\kappa)\big) \nonumber\\
    &\overset{(iii)}{\le} \kappa\ln\big(33L_1\|y_0-y^*(x_0)\|/(2\epsilon^2)\big) + \frac{\kappa T'}{3} \ln\Big(\frac{4(H_0-H^*)}{3L_{\Phi}T'}\Big) +\kappa T'\ln \big(66L_1\epsilon^{-2}(1+\kappa)\big)  \nonumber\\
    &=\widetilde{\mathcal{O}}(\kappa T') \le \widetilde{\mathcal{O}} \big(\sqrt{L_2}\kappa^{2.5}\epsilon^{-3}\big)
\end{align}
where (i) uses $(a+b)^3\le 4(a^3+b^3)$ for any $a,b\ge 0$, (ii) applies Jensen's inequality to the concave function $\ln(\cdot)$, and (iii) telescopes eq. \eqref{eq: potential} over $t=0,1,\ldots,T'-1$.
\end{proof}


==> 20230217 CubicMinimax_ArXiV_underTMLRreview/thm1proof.tex <==
\section{Proof of \Cref{thm: 1}} \label{sec_thm1proof}
\thmconv*

\begin{proof}
    We first prove item \ref{item: Phi_lim}. We have shown in \Cref{prop: lyapunov} that $\{H_t\}_t$ is monotonically decreasing. 
    {Also, \Cref{assum: f} implies that  $H_t=\Phi(x_t)+(L_{\Phi}+2\alpha+3\beta)\|s_t\|^3\ge \Phi^*>-\infty$ for Output I of Algorithm \ref{algo: prox-minimax}. Therefore, we conclude that $\{H_t\}_t$ converges to a finite limit $H^*>-\infty$.}
    
    Telescoping eq. \eqref{prop: lyapunov} over $t=0,1,\ldots,T-1$ yields that 
    \begin{align}
        \sum_{t=0}^{T-1}(\|s_{t+1}\|^3+\|s_t\|^3)\le& \frac{H_0-H_T}{L_{\Phi}+\alpha+\beta} \le \frac{H_0-H^*}{L_{\Phi}+\alpha+\beta} < +\infty, \label{eq: sum_s_cubic}
    \end{align}
    which by letting $T\to +\infty$ yields that $\sum_{t=0}^{\infty}(\|s_{t+1}\|^3+\|s_t\|^3)\le \frac{H_0-H^*}{L_{\Phi}+\alpha+\beta}<+\infty$ and thus $\|s_t\|\to 0$. Therefore
    \begin{align}
        \Phi(x_t)=H_t-(L_{\Phi}+2\alpha+3\beta)\|s_t\|^3 \to H^*.\nonumber
    \end{align}
    This proves item \ref{item: Phi_lim}.
    
    Next, we prove item \ref{item: compact}. Note that $\Phi$ has compact sub-level sets. Moreover, for all $t$, we have
    \begin{align}
        \Phi(x_t)\le H_t\le H_0<+\infty.
    \end{align}
    Hence, the sequence $\{x_t\}_t$ is bounded and thus has a compact set of limit points. Since $y^*$ is Lipschitz continuous by Proposition \ref{prop_Phiystar}, $\{\|y^*(x_t)\|\}_t$ is also bounded. Note that the proof of \Cref{prop: lyapunov} for Output I of Algorithm \ref{algo: prox-minimax} proves eq. \eqref{eq: yerr_t1}, which by $\|s_t\|\to 0$ implies that $\|y_{t+1} - y^*(x_t)\| \to 0$. Therefore, $\|y_{t+1}\|\le \|y^*(x_t)\|+\|y_{t+1} - y^*(x_t)\|$ is also bounded and thus also has a compact set of limit points. This proves item \ref{item: compact}.
    
    Finally, we will prove item \ref{item: 2ndCritical}. Suppose that $x_{t_k}\stackrel{k}{\to} x^*$ along a certain sub-sequence $\{x_{t_k}\}_k$. We have that $y_{t_k+1}\stackrel{k}{\to} y^*(x^*)$ based on \Cref{prop: lyapunov} and the continuity of $y^*$. In addition, \Cref{prop_Phiystar} implies that $\Phi$, $\nabla \Phi$, $\nabla^2 \Phi$ and $G$ are continuous. Therefore, for every limit point $x^*$,
    \begin{align}
        \Phi(x^*) =& \lim_{t_k\to\infty} \Phi(x_{t_k}) = H^* . \nonumber\\
        \|\nabla \Phi(x^*)\| =& \lim_{t_k\to\infty} \|\nabla \Phi(x_{t_k}) \| = \lim_{t_k\to\infty} \|\nabla f(x_{t_k},y^*(x_{t_k})) \|= \lim_{t_k\to\infty} \|\nabla f(x_{t_k},y_{t_k+1}) \| \nonumber\\
        \stackrel{(i)}{=}& \lim_{t_k\to\infty}\Big\|G(x_{t_k}, y_{t_k+1})(s_{t_k+1}) + \frac{1}{2\eta_x}\|s_{t_k+1}\| (s_{t_k+1})\Big\|=0 \nonumber\\
        \lambda_{\min} \big[\nabla^2 \Phi(x^*)\big]=& \lim_{t_k\to\infty} \lambda_{\min} \big[\nabla^2 \Phi(x_{t_k}) \big] = \lim_{t_k\to\infty} \lambda_{\min} \big[G(x_{t_k},y^*(x_{t_k})) \big] \nonumber\\
        =& \lim_{t_k\to\infty} \lambda_{\min} \big[G(x_{t_k},y_{t_k+1})\big] \stackrel{(ii)}{\ge} -\frac{1}{2\eta_x}\lim_{t_k\to\infty}\|s_{t_k+1}\| = 0 \nonumber
    \end{align}
    where (i) uses eq. \eqref{eq: CRcond1}, and (ii) uses eq. \eqref{eq: CRcond2}. Therefore, $x^*$ is a second-order stationary point of $\Phi$. Consequently, $(x^*, y^*(x^*))$ is a local minimax point due to \Cref{coro: 1}. 
    This proves item \ref{item: 2ndCritical}. 
\end{proof}



==> 20230217 CubicMinimax_ArXiV_underTMLRreview/thm2proof.tex <==
\section{Proof of \Cref{thm: 2}} \label{sec_thm2proof}

%\thmvarconv*

\begin{proof}
    For the potential function $H(x,x')=\Phi(x)+(L_{\Phi}+2\alpha+3\beta)\|x'-x\|^2$, we first derive a bound on its gradient $\|\nabla H(x,x')\|=\sqrt{\|\nabla_1 H(x,x')\|^2+\|\nabla_2 H(x,x')\|^2}$ as follows. 
    \begin{align}
        &\|\nabla H(x_t,x_{t-1})\|\nonumber\\
        &\le \|\nabla_1 H(x_t,x_{t-1})\|+\|\nabla_2 H(x_t,x_{t-1})\| \nonumber\\
        &= \Big\|\nabla \Phi(x_t)+2(L_{\Phi}+2\alpha+3\beta)(x_t-x_{t-1}) \Big\| + \Big\|2(L_{\Phi}+2\alpha+3\beta)(x_t-x_{t-1})\Big\|\nonumber\\
        &\le \|\nabla\Phi(x_t)\|+4(L_{\Phi}+2\alpha+3\beta)\|s_t\| \label{eq: 12}
    \end{align}
%    $\nabla_1 f(x_t, y_{t+1})+G(x_t, y_{t+1})(x_{t+1}-x_t) + \frac{\eta_x}{2}\|x_{t+1}-x_t\| (x_{t+1}-x_t) =0$
    where (i) uses eq. (2.2) of \cite{Nesterov2006}, the fact that $\nabla^2\Phi$ is $L_{\Phi}$-Lipschitz, and eq. \eqref{eq: ystar_grad}, (ii) uses Lemma \ref{lemma_HessBound} and $\nabla^2 \Phi(x)=G(x,y^*(x))$ from item 4 of Proposition \ref{prop_Phiystar}, (iii) uses eq. \eqref{eq: stationary}, $\nabla\Phi(x)=\nabla_1 f(x,y^*(x))$ from item 2 of Proposition \ref{prop_Phiystar} and the inequality that $1+\kappa\le 2\kappa$, (iv) and (v) use eq. \eqref{eq: 8b}, \red{and (v) uses $L_G=L_2(1+\kappa)^2\le 4L_2\kappa^2$, $L_{\Phi}=L_2(1+\kappa)^3\le 8L_2\kappa^3$.} 
    %$\nabla_1 f(x_t, y_{t+1})+G(x_t, y_{t+1})(x_{t+1}-x_t) + \frac{\eta_x}{2}\|x_{t+1}-x_t\| (x_{t+1}-x_t) =0$

%\begin{align}
%	\|y_{t+1} - y^*(x_{t}) \| \le&  (1-\kappa^{-1})^{N_t/2}\|y_{t} - y^*(x_{t})\|\\ %\label{eq: 8} \\
%	\le& \|x_t-x_{t-1}\|^2 %\label{eq: 8b}
%\end{align}

    Next, we prove the convergence of the sequence $\{x_t\}_t$ under the assumption that $H(x,x',y)$ satisfies the {\L}ojasiewicz gradient geometry. 
    Recall that we have shown in the proof of \Cref{thm: 1} that: 1) $\{H_t\}_t$ decreases monotonically to the finite limit $H^*$; 2) for any limit point $x^*, y^*$ of $\{x_t\}_t, \{y_t\}_t$, $\Phi(x^*)=H^*$. Hence, the {\L}ojasiewicz gradient inequality (see \Cref{def: KL}) holds after sufficiently large number of iterations, i.e., there exists $t_1\in \mathbb{N}^+$ such that for all $t\ge t_1$, $H(x_t,x_{t-1},y_{t+1})-H^*\le c\|\nabla H(x_t,x_{t-1},y_{t+1})\|^{\theta}$. Equivalently,
    \begin{align}
    	\varphi'(H_t -H^*) \|\nabla H(x_t,x_{t-1},y_{t+1})\|\ge 1. \nonumber
    \end{align}
    where we define the concave function that $\varphi(s):=\frac{c^{1/\theta}}{1-1/\theta}s^{1-1/\theta} (\theta>1, s>0)$. 
    
    In addition, since $\|x_t-x_{t-1}\|\stackrel{t}{\to} 0$ (Proposition \ref{prop: lyapunov}), there exists $t_2\in\mathbb{N}^{+}$ such that for all $t\ge t_2$, $\|x_t-x_{t-1}\|\le 1$. Hence, rearranging the above inequality and utilizing \cref{eq: 12}, we obtain that for all $t\ge t_0:=\max(t_1,t_2)$, 
    \begin{align}
    	&\varphi'(H_t -H^*) \nonumber\\
    	&\ge \|\nabla H(x_t,x_{t-1},y_{t+1})\|^{-1} \nonumber\\
    	&\ge \Big[\Big(\red{\frac{4L_2^2\kappa^2}{L_1}+L_2}\Big)\|x_{t-1}-x_{t-2}\|^2 + \Big(\red{10L_2\kappa^3 + \frac{24 L_2^3\kappa}{L_1^2}}+\frac{1}{2\eta_x}\Big) \|x_t-x_{t-1}\|^2 \Big]^{-1}\label{eq: 13}
    \end{align}
    
    By concavity of the function $\varphi(s):=\frac{c^{1/\theta}}{1-1/\theta}s^{1-1/\theta} (\theta>1, s>0)$, we know that 
    \begin{align}
    	&\varphi(H_t -H^*) - \varphi(H_{t+1} -H^*) \nonumber\\
    	&\ge \varphi'(H_t -H^*) (H_t - H_{t+1}) \nonumber\\
    	&\stackrel{(i)}{\ge} \frac{\red{L_2\kappa^3} \|x_{t+1}-x_t\|^3}{\Big(\red{\frac{4L_2^2\kappa^2}{L_1}+L_2}\Big)\|x_{t-1}-x_{t-2}\|^2 + \Big(\red{10L_2\kappa^3 + \frac{24 L_2^3\kappa}{L_1^2}}+\frac{1}{2\eta_x}\Big) \|x_t-x_{t-1}\|^2} \label{eq: phidiff}\\
    	&\stackrel{(ii)}{\ge} \frac{\red{L_2\kappa^3} \|x_{t+1}-x_t\|^3}{\Big(\sqrt{\red{\frac{4L_2^2\kappa^2}{L_1}+L_2}}\|x_{t-1}-x_{t-2}\| + \sqrt{\red{10L_2\kappa^3 + \frac{24 L_2^3\kappa}{L_1^2}}+\frac{1}{2\eta_x}} \|x_t-x_{t-1}\|\Big)^2}, \nonumber
    \end{align}
    where (i) uses \Cref{prop: lyapunov} and \cref{eq: 13}, (ii) uses the inequality that $a^2+b^2\le (a+b)^2$ for any $a,b\ge 0$. 
    
    Rearranging the above inequality yields that
    \begin{align}
        &\red{L_2\kappa^3} \|x_{t+1}-x_t\|^3  \nonumber\\
        &\le [\varphi(H_t -H^*) - \varphi(H_{t+1} -H^*)]\nonumber\\ 
        &\quad \Bigg(\sqrt{\red{\frac{4L_2^2\kappa^2}{L_1}+L_2}}\|x_{t-1}-x_{t-2}\| + \sqrt{\red{10L_2\kappa^3 + \frac{24 L_2^3\kappa}{L_1^2}}+\frac{1}{2\eta_x}} \|x_t-x_{t-1}\|\Bigg)^2 \nonumber\\
        &\le \frac{1}{27}\Bigg(C^2[\varphi(H_t -H^*) - \varphi(H_{t+1} -H^*)]+\frac{2}{C}\sqrt{\red{\frac{4L_2^2\kappa^2}{L_1}+L_2}}\|x_{t-1}-x_{t-2}\|  \nonumber\\
        &\quad +\frac{2}{C}\sqrt{\red{10L_2\kappa^3 + \frac{24 L_2^3\kappa}{L_1^2}}+\frac{1}{2\eta_x}} \|x_t-x_{t-1}\|\Bigg)^3
    \end{align}
    where the final step uses the AM-GM inequality that $ab^2=\big[\sqrt[3]{(C^2a)(b/C)(b/C)}\big]^3\le \frac{1}{27}(C^2a+\frac{2b}{C})^3$ for any $a,b\ge 0$ and $C>0$ (the value of $C$ will be assigned later). Taking cubic root of both sides of the above inequality and telescoping it over {$t=t_0,\ldots,T-1$}, we obtain that
    \begin{align}
    	&\red{\kappa\sqrt[3]{L_2}}\sum_{t=t_0}^{T-1}\|x_{t+1}-x_t\|\nonumber\\
    	&\le \frac{C^2}{3}[\varphi(H_{t_0} -H^*) - \varphi(H_T -H^*)]+\frac{2}{3C}\sqrt{\red{\frac{4L_2^2\kappa^2}{L_1}+L_2}}\sum_{t=t_0}^{T-1}\|x_{t-1}-x_{t-2}\| \nonumber\\
        &\quad + \frac{2}{3C}\sqrt{\red{10L_2\kappa^3 + \frac{24 L_2^3\kappa}{L_1^2}}+\frac{1}{2\eta_x}} \sum_{t=t_0}^{T-1}\|x_t-x_{t-1}\|\nonumber\\
    	&\le \frac{C^2}{3}\varphi(H_{t_0} -H^*) + \frac{2}{3C}\sqrt{\red{\frac{4L_2^2\kappa^2}{L_1}+L_2}}\sum_{t=t_0}^{T-1}\|x_{t-1}-x_{t-2}\| \nonumber\\
        &\quad + \frac{2}{3C}\sqrt{\red{10L_2\kappa^3 + \frac{24 L_2^3\kappa}{L_1^2}}+\frac{1}{2\eta_x}} \sum_{t=t_0}^{T-1}\|x_t-x_{t-1}\|\nonumber
    \end{align}
    where the final step uses the facts that $H_t-H^*\ge 0$ and that $\varphi(s)$ is monotonically increasing. Since the value of $C>0$ is arbitrary, we can select large enough $C$ such that $\frac{2}{3C}\sqrt{\red{\frac{4L_2^2\kappa^2}{L_1}+L_2}}, \frac{2}{3C}\sqrt{\red{10L_2\kappa^3 + \frac{24 L_2^3\kappa}{L_1^2}}+\frac{1}{2\eta_x}}<\frac{\red{\kappa\sqrt[3]{L_2}}}{3}$. Hence, the inequality above further implies that
    \begin{align}
        \frac{\red{\kappa\sqrt[3]{L_2}}}{3}\sum_{t=t_0}^{T-1}\|x_{t+1}-x_t\| \le& \frac{C^2}{3}\varphi(H_{t_0} -H^*) \nonumber\\
        & +\frac{\red{\kappa\sqrt[3]{L_2}}}{3} \big[\|x_{t_0-1}-x_{t_0-2}\|+2\|x_{t_0}-x_{t_0-1}\|\big] < +\infty. \label{eq: sum_dx_upperbound}
    \end{align}
    Letting $T\to\infty$ concludes that
    $$\sum_{t=1}^{\infty}\|x_{t+1} - x_t\| {<} +\infty.$$ 
    Moreover, this implies that $\{x_t\}_t$ is a Cauchy sequence and therefore converges to a certain limit, i.e., $x_t \overset{t}{\to} x^*$. We have shown in \Cref{thm: 1} that any such limit point must be a second-order critical point of $\Phi$. Hence, we conclude that $\{x_t\}_t$ converges to a certain second-order critical point $x^*$ of $\Phi(x)$. Also, note that $\|y^*(x_{t})-y_{t}\| \overset{t}{\to} 0$, $x_t\overset{t}{\to} x^*$ and $y^*$ is a Lipschitz mapping, so we conclude that $\{y_t\}_t$ converges to $y^*(x^*)$.  Finally, the item \ref{item: 2ndCritical} of \Cref{thm: 1} implies that $x^*$ is a second-order critical point of $\Phi(x)$. 
\end{proof}


==> 20230217 CubicMinimax_ArXiV_underTMLRreview/thm3proof.tex <==
\section{Proof of \Cref{thm: 3}} \label{sec_thm3proof}

\thmconvrate*

\begin{proof}
    We redefine the potential function $H(x,x')=\Phi(x)+(L_{\Phi}+2\alpha+3\beta)\|x-x'\|^3$ to make the dependence on $x,x'$ explicit. Then, the potential function in \Cref{prop: lyapunov} can be rewritten as $H_t=H(x_t, x_{t-1})$. 
    Recall that we have shown in the proof of \Cref{thm: 1} that: 1) $\{H_t\}_t$ decreases monotonically to the finite limit $H^*$; 2) for any limit point $x^*, y^*$ of $\{x_t\}_t, \{y_t\}_t$, $\Phi(x^*)=H^*$. Hence, the {\L}ojasiewicz gradient inequality (see \Cref{def: KL}) holds after sufficiently large number of iterations, i.e., there exists $t_0\in \mathbb{N}^+$ such that for all $t\ge t_0$, $H(x_t,x_{t-1})-H^*\le c\|\nabla H(x_t,x_{t-1})\|^{\theta}$. By denoting $d_t=H(x_t,x_{t-1})-H^*=H_t-H^*$, this inequality implies that
    \begin{align}
    &c^{-1/\theta}d_t^{1/\theta} \nonumber\\
    &\le \|\nabla H(x_t,x_{t-1})\| \nonumber\\
    &\le \|\nabla_1 H(x_t,x_{t-1})\| + \|\nabla_2 H(x_t,x_{t-1})\| \nonumber\\
    &\le \Big\|\nabla \Phi(x_t)+3(L_{\Phi}+2\alpha+3\beta)\|x_t-x_{t-1}\|(x_t-x_{t-1})\Big\| + \big\|3(L_{\Phi}+2\alpha+3\beta)\|x_t-x_{t-1}\|(x_t-x_{t-1})\big\| \nonumber\\
    &\le \|\nabla \Phi(x_t)\| +6(L_{\Phi}+2\alpha+3\beta)\|s_t\|^2 \nonumber\\
    &\overset{(i)}{=}\Big\|\nabla \Phi(x_{t})-\nabla f(x_{t-1},y_{t}) -G(x_{t-1},y_{t}) s_{t} -\frac{1}{2\eta_x}\|s_{t}\|s_{t}\Big\| + 6(L_{\Phi}+2\alpha+3\beta)\|s_t\|^2 \nonumber\\
    &\le \|\nabla \Phi(x_{t})-\nabla \Phi(x_{t-1})-\nabla^2 \Phi(x_{t-1})s_{t}\| + \|\nabla \Phi(x_{t-1})-\nabla f(x_{t-1},y_{t})\|\nonumber\\
    &\quad + \|\nabla^2 \Phi(x_{t-1})s_{t}-G(x_{t-1},y_{t}) s_{t}\| + \frac{1}{2\eta_x}\|s_{t}\|^2 +6(L_{\Phi}+2\alpha+3\beta)\|s_t\|^2 \nonumber\\
    &\overset{(ii)}{\le} \Big(7L_{\Phi}+12\alpha+18\beta+\frac{1}{2\eta_x}\Big)\|s_{t}\|^2  +\beta\|s_{t-1}\|^2 +\alpha\|s_{t-1}\|\|s_{t}\| \nonumber\\
    &\overset{(iii)}{\le} \Big(7L_{\Phi}+13\alpha+18\beta+\frac{1}{2\eta_x}\Big)\|s_{t}\|^2  +(\alpha+\beta)\|s_{t-1}\|^2\nonumber\\
    &\le \Big(7L_{\Phi}+13\alpha+18\beta+\frac{1}{2\eta_x}\Big)\big(\|s_{t}\|^2+\|s_{t-1}\|^2\big)\nonumber\\
    &\overset{(iv)}{\le} (14L_{\Phi}+26\alpha+36\beta+\frac{1}{\eta_x}\Big) (\|s_{t}\|^3+\|s_{t-1}\|^3)^{2/3} \nonumber\\
    &\overset{(v)}{\le} \frac{14L_{\Phi}+26\alpha+36\beta+1/\eta_x}{(L_{\Phi}+\alpha+\beta)^{2/3}} (H_{t-1}-H_t)^{2/3}.\nonumber\\
    &=\frac{14L_{\Phi}+26\alpha+36\beta+1/\eta_x}{(L_{\Phi}+\alpha+\beta)^{2/3}} (d_{t-1}-d_t)^{2/3}. \nonumber
    \end{align}
    where (i) uses eq. \eqref{eq: CRcond1}, (ii) uses eqs. \eqref{eq: dfKL} \& \eqref{eq: dGKL} and the item \ref{item: ddPhi} of \Cref{prop_Phiystar} that $\nabla^2\Phi$ is $L_{\Phi}$-Lipschitz, (iii) uses $ab\le (a^2+b^2)/2$ for all $a,b\ge 0$, (iv) uses $a^2+b^2 \le 2(a^3+b^3)^{2/3}$ for all $a,b\ge 0$, (v) uses Proposition \ref{prop: lyapunov}. The above inequality can be rearranged as follows.
    \begin{align}
        d_{t-1}\ge d_t+Cd_t^{\frac{3}{2\theta}} \label{eq: 16} 
    \end{align}
    where $C=\frac{L_{\Phi}+\alpha+\beta}{c^{\frac{3}{2\theta}}(14L_{\Phi}+26\alpha+36\beta+1/\eta_x)^{3/2}}$. 
    
    Next, we prove the convergence rates case by case.
    
    (Case 1) If $\theta\in (\frac{3}{2}, +\infty)$, since $d_t \ge 0$, eq. \eqref{eq: 16} implies that for $t\ge t_0$,
    \begin{align}
        d_{t-1}\ge Cd_t^{\frac{3}{2\theta}},\nonumber
    \end{align}
    which is equivalent to that
    \begin{align}
    	C^{-\frac{2\theta}{2\theta-3}}d_t\le \big(C^{-\frac{2\theta}{2\theta-3}}d_{t-1}\big)^{2\theta/3} \label{eq: HdecSuper}
    \end{align}
    
    Since $d_t\downarrow 0$, $C^{-\frac{3\theta}{2\theta-3}}d_{t_0} \le e^{-1}$ for sufficiently large $t_0\in \mathbb{N}^+$. Hence, eq. \eqref{eq: HdecSuper} implies that for any $k\in\mathbb{N}^+$
    \begin{align}
    	C^{-\frac{3\theta}{2\theta-3}}d_{t}\le& \big[C^{-\frac{3\theta}{2\theta-3}}d_{t_0}\big]^{[(2\theta/3)^{t-t_0}]} \le \exp\Big[-\Big(\frac{2\theta}{3}\Big)^{t-t_0}\Big].\nonumber
    \end{align}
    Note that $\theta\in (\frac{3}{2}, +\infty)$ implies that $\frac{2\theta}{3}>1$, and thus the above inequality implies that $d_t\downarrow 0$ (i.e., $H(z_t) \downarrow H^*$) at the super-linear rate given by eq. \eqref{eq: HsuperConverge}. 

    (Case 2) If $\theta=\frac{3}{2}$, eq. \eqref{eq: 16} implies that for $t\ge t_0$,
    \begin{align}
        d_{t-1}\ge (1+C)d_t.\label{eq: HdecLinear}
    \end{align}
    Note that $d_{t_0}\le 1$ for sufficiently large $t_0$. Therefore, $d_t\downarrow 0$ (i.e., $H(z_t) \downarrow H^*$) at the linear rate given by eq. \eqref{eq: HlinearConverge}. 

    (Case 3) If $\theta\in (1, \frac{3}{2})$, consider the following two subcases.
    
    If $d_{t-1}\le 2d_t$, denote $\psi(s)=\frac{2\theta}{3-2\theta}s^{1-\frac{3}{2\theta}}$, then for any $t\ge t_0$,
    \begin{align}
    	\psi(d_t)-\psi(d_{t-1})=&\int_{d_{t}}^{d_{t-1}} -\psi'(s)ds = \int_{d_{t}}^{d_{t-1}} s^{-\frac{3}{2\theta}}ds \stackrel{(i)}{\ge} d_{t-1}^{-\frac{3}{2\theta}} (d_{t-1}-d_t) \nonumber\\
    	\stackrel{(ii)}{\ge}& C \Big(\frac{d_t}{d_{t-1}}\Big)^{\frac{3}{2\theta}} \stackrel{(iii)}{\ge} 2^{-\frac{3}{2}}C \ge \frac{C}{4} \label{eq: subcase1}
    \end{align}
    where (i) uses $d_t\le d_{t-1}$ and $-\frac{3}{2}\theta<0$, (ii) uses eq. \eqref{eq: 16}, and (iii) uses $\frac{d_t}{d_{t-1}} \ge \frac{1}{2}$ and $\frac{3}{2\theta}\in \big(1,\frac{3}{2}\big)$. 
    
    If $d_{t-1}>2d_t$, then for any $t\ge t_0$,
    \begin{align}
    	\psi(d_t)-\psi(d_{t-1})=&\frac{2\theta}{3-2\theta}(d_t^{1-\frac{3}{2\theta}}-d_{t-1}^{1-\frac{3}{2\theta}}) \stackrel{(i)}{\ge} \frac{2\theta}{3-2\theta}\big[d_t^{1-\frac{3}{2\theta}}-(2d_t)^{1-\frac{3}{2\theta}}\big] \nonumber\\
    	\ge& \frac{2\theta\big(1-2^{1-\frac{3}{2\theta}}\big)}{3-2\theta} d_t^{1-\frac{3}{2\theta}} \stackrel{(ii)}{\ge} \frac{C}{4}. \label{eq: subcase2}
    \end{align}
    where (i) uses $d_{t-1}>2d_t$ and $1-\frac{3}{2\theta}\in \big(-\frac{1}{2},0\big)$, $\frac{2\theta}{3-2\theta}>0$, and (ii) uses $1-\frac{3}{2\theta}\in \big(-\frac{1}{2},0\big)$ and $d_t\le d_{t_0} \le \Big(\frac{8\theta\big(1-2^{1-\frac{3}{2\theta}}\big)}{C(3-2\theta)}\Big)^{\frac{2\theta}{3-2\theta}}$ for sufficiently large $t_0\in\mathbb{N}^+$. 

Since at least one of eqs. \eqref{eq: subcase1} \& \eqref{eq: subcase2} holds, we have $\psi(d_t) \ge \psi(d_{t_0})+C(t-t_0)/4 \ge C(t-t_0)/4$. By substituting the definition of $\psi$, this inequality implies that $d_t\downarrow 0$ (i.e., $H(z_t) \downarrow H^*$) in a sub-linear rate given by eq. \eqref{eq: HsubConverge}. 
\end{proof}


==> 20230217 CubicMinimax_ArXiV_underTMLRreview/thm4proof.tex <==
\section{Convergence Rate of SGA} \label{sec_thm4proof}
The following high-probability convergence rate of SGA is a direct application of the Theorem 3.1 of \cite{harvey2019simple}.

\begin{restatable}{thm}{lemmaSGA}\label{lemma: SGA}
    Let Assumption \ref{assum: fi} hold. For all $t,k$, assume that $\|\nabla_2 f(x_t,\widetilde{y}_k)\|\le L_0$ and $\|\widehat{\nabla}_2 f(x_t,\widetilde{y}_k)-\nabla_2 f(x_t,\widetilde{y}_k)\|\le 1$ almost surely.
    The inner stochastic gradient ascent steps in \Cref{algo: prox-minimax-stoc} converges at the following rate with probability at least $1-\delta$.
    \begin{align}
        \|y_{t+1}-y^*(x_t)\|\le \mathcal{O}\Big(\sqrt\frac{L_0\ln(1/\delta)+L_0^2}{\mu^2 N_t}\Big).\nonumber
    \end{align}
\end{restatable}

\begin{proof}
    Based on Theorem 3.1 of \cite{harvey2019simple}, the inner SGA steps in Algorithm \ref{algo: prox-minimax-stoc} has the following convergence rate with probability at least $1-\delta$.
    \begin{align}
        f(x_t,y^*(x_t))-f(x_t,y_{t+1})\le \mathcal{O}\Big(\frac{L_0\ln(1/\delta)+L_0^2}{\mu N_t}\Big),
    \end{align}
    which by $\mu$-strong concavity of $f(x_t,\cdot)$ proves the following convergence rate.
    \begin{align}
        \|y_{t+1}-y^*(x_t)\|\le \sqrt{2\big(f(x_t,y^*(x_t))-f(x_t,y_{t+1})\big)/\mu} \le \mathcal{O}\Big(\sqrt\frac{L_0\ln(1/\delta)+L_0^2}{\mu^2 N_t}\Big).\nonumber
    \end{align}
\end{proof}

==> 20230217 CubicMinimax_ArXiV_underTMLRreview/thm5proof.tex <==
\section{Proof of \Cref{thm: 5}} \label{sec_thm5proof}
\thmstoc*

\begin{proof}
    In Lemma \ref{lemma: batch}, replace $x, y$ with $x_t, y_t$, $B_1$ with $B_1(t)$, and $B_{k,\ell}$ with $B_{k,\ell}(t)$ for any $k,\ell\in\{1,2\}$, and substitute the following hyperparameters.
    \begin{align}
        \epsilon_1(t)=&\frac{L_{\Phi}}{2}\Big(\|s_t\|^2+\frac{\epsilon^2}{33L_{\Phi}}\Big)\wedge 2L_0=\mathcal{O}(L_{\Phi}\|s_t\|^2+\epsilon^2), \nonumber\\
        \epsilon_2(t)=&\frac{L_{\Phi}}{2(\kappa+1)^2}\Big(\|s_t\|+\frac{\epsilon}{\sqrt{33L_{\Phi}}}\Big)\wedge 4L_1=\mathcal{O}\big(\kappa^{-2}(L_{\Phi}\|s_t\|+\sqrt{L_{\Phi}}\epsilon)\big). \nonumber
    \end{align}
    Then, we obtain that using the following batchsizes 
    \begin{align}
        \left\{ \begin{gathered}
           |B_1(t)|\ge \mathcal{O}\Big(\frac{L_0^2}{(L_{\Phi}^2\|s_t\|^4 + \epsilon^4)}\ln\frac{m}{\delta}\Big) \hfill \\
           |B_{k,\ell}(t)|\ge \mathcal{O}\Big(\frac{L_1^2\kappa^4}{L_{\Phi}(L_{\Phi}\|s_t\|^2 + \epsilon^2)}\ln\frac{m+n}{\delta}\Big) \hfill 
        \end{gathered}  \right.,\label{eq: batchsizes}
    \end{align}
    the stochastic approximators satisfy the following error bounds with probability at least $1-\delta$.
    \begin{align}
        \|\widehat{\nabla}_1 f(x_t,y_t)-\nabla_1 f(x_t,y_t)\|&\le \epsilon_1(t) \le\frac{L_{\Phi}}{2}\Big(\|s_t\|^2+\frac{\epsilon^2}{33L_{\Phi}}\Big),\label{eq: stoc_err1_detail}\\ 
        \|\widehat{G}(x_t,y_t)-G(x_t,y_t)\|&\le  \epsilon_2(t)\le \frac{L_{\Phi}}{2}\Big(\|s_t\|+\frac{\epsilon}{\sqrt{33L_{\Phi}}}\Big).\label{eq: stoc_err3_detail}
    \end{align}
    Based on Theorem \ref{lemma: SGA}, using the following number of stochastic gradient ascent steps
    \begin{align}
        N_t&\ge \mathcal{O}\Big(\frac{L_0\ln(1/\delta)+L_0^2}{\mu^2L_{\Phi}^2\big(([\|s_t\|^2+\epsilon^2/(33L_{\Phi})]/L_1) \wedge ([\|s_t\|+\epsilon/\sqrt{33L_{\Phi}}]/L_G)\big)^2}\Big)\nonumber\\
        &\overset{(i)}{=}\mathcal{O}\Big(\frac{L_0\ln(1/\delta)+L_0^2}{\big(([L_{\Phi}\|s_t\|^2+\epsilon^2]/\kappa)\wedge L_1(\|s_t\|+\epsilon/\sqrt{L_{\Phi}})\big)^2}\Big)\nonumber\\
        &=\mathcal{O}\Big(\frac{L_0\ln(1/\delta)+L_0^2}{\kappa^{-2}(L_{\Phi}^2\|s_t\|^4+\epsilon^4)\wedge L_1^2(\|s_t\|^2+\epsilon^2/L_{\Phi})}\Big), \label{eq: Ntstoc}
    \end{align} 
    where (i) uses $\kappa=L_1/\mu$ and $L_{\Phi}=L_G(1+\kappa)$ (\Cref{prop_Phiystar}). 
    we have
    \begin{align}
        \|y_{t+1}-y^*(x_t)\|\le \mathcal{O}\Big(\sqrt\frac{L_0\ln(1/\delta)+L_0^2}{\mu^2 N_t}\Big)\le \frac{L_{\Phi}}{2}\min\Big(\frac{1}{L_1}\Big(\|s_t\|^2+\frac{\epsilon^2}{33L_{\Phi}}\Big), \frac{1}{L_G}\Big(\|s_t\|+\frac{\epsilon}{\sqrt{33L_{\Phi}}}\Big)\Big). \label{eq: yerr_stoc}
    \end{align}
    Therefore, 
    \begin{align}
        &\|\nabla\Phi(x_t)-\widehat{\nabla}_1 f(x_t, y_{t+1})\|\nonumber\\
        &\overset{(i)}{\le}\|\nabla_1 f(x_t,y^*(x_t))-\nabla_1 f(x_t, y_{t+1})\|+\|\widehat{\nabla}_1 f(x_t, y_{t+1})-\nabla_1 f(x_t, y_{t+1})\|\nonumber\\
        &\overset{(ii)}{\le} L_1\|y_{t+1}-y^*(x_t)\| + \frac{L_{\Phi}}{2}\Big(\|s_t\|^2+\frac{\epsilon^2}{33L_{\Phi}}\Big) \nonumber\\
        &\overset{(iii)}{\le} L_{\Phi}\Big(\|s_t\|^2+\frac{\epsilon^2}{33L_{\Phi}}\Big),\label{eq: dfstoc}
    \end{align}
    where (i) uses $\nabla\Phi(x)=\nabla_1 f(x,y^*(x))$ in \Cref{prop_1}, (ii) uses eq. \eqref{eq: stoc_err1_detail} and \Cref{assum: f}, and (iii) uses eq. \eqref{eq: yerr_stoc}. 
    \begin{align}
        &\|\nabla^2\Phi(x_t)-\widehat{G}(x_t,y_{t+1})\|\nonumber\\
        &\overset{(i)}{\le}\|G(x_t,y^*(x_t))-G(x_t,y_{t+1})\|+\|\widehat{G}(x_t,y_{t+1})-G(x_t,y_{t+1})\|\nonumber\\
        &\overset{(ii)}{\le} L_G\|y_{t+1}-y^*(x_t)\| + \frac{L_{\Phi}}{2}\Big(\|s_t\|+\frac{\epsilon}{\sqrt{33L_{\Phi}}}\Big) \nonumber\\
        &\overset{(iii)}{\le} L_{\Phi}\Big(\|s_t\|+\frac{\epsilon}{\sqrt{33L_{\Phi}}}\Big),\label{eq: dGstoc}
    \end{align}
    where (i) uses $\nabla^2\Phi(x)=G(x,y^*(x))$ in \Cref{prop_Phiystar}, (ii) uses eq. \eqref{eq: stoc_err3_detail} and the item \ref{item: G_lipschitz} of \Cref{prop_Phiystar}, and (iii) uses eq. \eqref{eq: yerr_stoc}. Eqs. \eqref{eq: dfstoc} \& \eqref{eq: dGstoc} imply that the conditions \eqref{eq: grad_goal_noKL} \& \eqref{eq: Hess_goal_noKL} hold with $\alpha=\beta=L_{\Phi}=L_2(1+\kappa)^3$ and $\epsilon'=\frac{\epsilon}{\sqrt{33L_{\Phi}}}$. In Lemma \ref{lemma_general_rate}, by substituting these values of $\alpha$, $\beta$, $\epsilon'$ and $\eta_x=(55L_{\Phi})^{-1}$, we obtain that when $T\ge \frac{\Phi(x_0)-\Phi^*+8L_{\Phi}\epsilon'^2}{3L_{\Phi}\epsilon'^3}$,  we have $T'\le \sqrt{33L_{\Phi}}\frac{33(\Phi(x_0)-\Phi^*)+8\epsilon^2}{3\epsilon^3}=\mathcal{O}\big(\sqrt{L_2}\kappa^{1.5}\epsilon^{-3}\big)\le T$, and moreover,
    \begin{align}
        &\|\nabla \Phi(x_{T'})\| \le \Big(\frac{1}{2\eta_x}+L_{\Phi}+2\alpha+2\beta\Big) \epsilon'^2 \le \epsilon^2, \nonumber\\
        &\lambda_{\min}\big(\nabla^2 \Phi(x_{T'})\big) \ge -\Big(\frac{1}{2\eta_x}+L_{\Phi}+2\alpha\Big)\epsilon' \overset{(i)}{\ge} -\sqrt{33L_{\Phi}}\epsilon, \nonumber
    \end{align}
    This proves that eq. \eqref{eq: gH_rate2} holds with probability at least $1-\delta$. 
    
    Choosing both $N_t$ in eq. \eqref{eq: Ntstoc} and the batchsizes in eq. \eqref{eq: batchsizes} with equality, the number of gradient computations has the following upper bound. 
    \begin{align}
        &\sum_{t=0}^{T'-1} \big(N_t+|B_1(t)|\big)\nonumber\\
        &=\sum_{t=0}^{T'-1}\mathcal{O} \Big( \frac{L_0\ln(1/\delta)+L_0^2}{\kappa^{-2}(L_{\Phi}^2\|s_t\|^4+\epsilon^4)\wedge L_1^2(\|s_t\|^2+\epsilon^2/L_{\Phi})} + \frac{L_0^2}{L_{\Phi}^2\|s_t\|^4 + \epsilon^4}\ln\frac{m}{\delta}\Big) \nonumber\\
        &\le \sum_{t=0}^{T'-1}\mathcal{O} \Big( \frac{L_0\ln(1/\delta)+L_0^2}{\epsilon^4\kappa^{-2}\wedge L_1^2\epsilon^2/L_{\Phi}} + \frac{L_0^2}{\epsilon^4}\ln\frac{m}{\delta}\Big) \nonumber\\
        &\overset{(i)}{\le} 
        T'\mathcal{O}\Big(\frac{L_0\kappa^2}{\epsilon^4}\big(\ln(1/\delta)+L_0\big) + \frac{L_0^2}{\epsilon^4}\ln\frac{m}{\delta}\Big) \nonumber\\
        &\overset{(ii)}{\le} \mathcal{O}\big(\sqrt{L_2}\kappa^{1.5}\epsilon^{-3}\big) \mathcal{O}\Big(\frac{L_0^2\kappa^2}{\epsilon^4}\ln\frac{m}{\delta}\Big) \nonumber\\
        &\le \mathcal{O}\Big(\frac{L_0^2\kappa^{3.5}\sqrt{L_2}}{\epsilon^7}\ln\frac{m}{\delta}\Big)
    \end{align}
    where (i) uses $\epsilon'=\frac{\epsilon}{\sqrt{33L_{\Phi}}}\le \frac{L_1}{L_G}=\frac{L_1(1+\kappa)}{L_{\Phi}}$ which implies that $\epsilon^4\kappa^{-2} \le \mathcal{O}(L_1^2\epsilon^2/L_{\Phi})$, (ii) uses $T'\le\mathcal{O}\big(\sqrt{L_2}\kappa^{1.5}\epsilon^{-3}\big)$ we proved above. The number of Hessian computations has the following upper bound.
    \begin{align}
        &\sum_{t=0}^{T'-1} \sum_{k=1}^2\sum_{\ell=1}^2|B_{k,\ell}(t)|\nonumber\\
        &=\sum_{t=0}^{T'-1}\mathcal{O} \Big(\frac{L_1^2\kappa^4}{L_{\Phi}(L_{\Phi}\|s_t\|^2 + \epsilon^2)}\ln\frac{m+n}{\delta}\Big) \nonumber\\
        &\le \sum_{t=0}^{T'-1}\mathcal{O} \Big(\frac{L_1^2\kappa^4}{L_{\Phi}\epsilon^2}\ln\frac{m+n}{\delta}\Big) \nonumber\\
        &\overset{(i)}{\le} 
        T'\mathcal{O}\Big( \frac{L_1^2\kappa}{L_2\epsilon^2}\ln\frac{m+n}{\delta}\Big) \nonumber\\
        &\overset{(ii)}{\le} \mathcal{O}\Big( \frac{L_1^2\kappa^{2.5}}{\sqrt{L_2}\epsilon^5}\ln\frac{m+n}{\delta}\Big)
    \end{align}
    where (i) uses $L_{\Phi}=L_2(1+\kappa)^3=\mathcal{O}(L_2\kappa^3)$, (ii) uses $T'\le \sqrt{33L_{\Phi}}\frac{33(\Phi(x_0)-\Phi^*)+8\epsilon^2}{3\epsilon^3}=\mathcal{O}\big(\sqrt{L_2}\kappa^{1.5}\epsilon^{-3}\big)$ we proved above. 
\end{proof}



==> assumption1.tex <==
\section{Proof of the relationship among the statements in Assumption 1}\label{sec_assum1}

We will prove that in \Cref{assum: f}, the item 2 and the statement that $g$ is lower semi-continuous can be derived from the rest of \Cref{assum: f}. 
\begin{proof}
	\noindent Since the sub-level set $\{x: (\Phi+g)(x)\le\alpha\}$ is closed, $\Phi+g$ is lower semi-continuous. Without item 2 and any assumption on $g$, Lemma \Cref{prop_Phiystar} holds which implies continuity of $\Phi$, so $g$ is lower semi-continuous.  
	
	%\noindent If the sub-level set $A=\{x: (\Phi+g)(x)\le0 \}$ is empty, then 0 is a lower bound of $\Phi+g$. Hence, we focus on the case where $A$ is non-empty convex set.\\
	
	\noindent Suppose $\Phi+g$ is not bounded below, then there is a sequence $\{x_t\}_t$ such that $(\Phi+g)(x_t)\le -t$. Since $x_t\in A$ and $A$ is compact, $\{x_n\}$ has at one convergent subsequence $x_{n(t)}\overset{t}{\to} x^*$. Since $\Phi+g$ is lower semi-continuous, $\Phi(x^*)+g(x^*)\le \mathop{\lim\inf}_{n\to\infty} \Phi(x_{n(t)})+g(x_{n(t)})=-\infty$. However, since $\Phi$ is continuous and $g$ is proper, $\Phi(x^*), g(x^*)>-\infty$, is a contradiction. Hence, $\Phi+g$ is not bounded below, that is, the item 2 of \Cref{assum: f} holds
\end{proof}

==> coro1proof.tex <==



==> experiments.tex <==
In this section, we do empirical studies contrasting our algorithm with the classical GDA algorithm on both synthetic problem and real-world application.

\subsection{Synthetic Minimax Problem}

We construct the following nonconvex-strongly-concave minimax problem:
\[
f_i(\textbf{x,y}) = w(x_3) - \frac{y_1^2}{40} + A_i x_1 y_1 - \frac{5y_2^2}{2} + B_i x_2 y_2
\]

where $A_i$ and $B_i$ are independent random variables from uniform distribution range from 0.5 to 1.5, $N=1000$ is the number of total sample,
$w(.)$ is W-shaped scalar functions whose exact form is shown in Appendix.
Then we consider the minimax problem with such expression below:
\begin{equation}
    \min\limits_{\textbf{x} \in \mathcal{R}^3} \max\limits_{\textbf{y} \in \mathcal{R}^2} f(\textbf{x,y}) =  \min\limits_{\textbf{x} \in \mathcal{R}^3} \max\limits_{\textbf{y} \in \mathcal{R}^2} \frac{1}{N}\sum^N_{i=1} f_i(\textbf{x,y})
\end{equation}

We first set initial point at $\textbf{x}=[0,0,1]^T$ and $\textbf{y}=[1,1]^T$, compare the different performance on batchsize 20,100,500.  

\begin{figure}[htbp]

\centering
\includegraphics[width=0.95\linewidth]{emsnewsletter-template/pictures/batchsize-contrast.png}

\caption{stochastic cubic GDA on different batchsize}\label{result1}
	
\end{figure}

Trough Figure 1 we can obviously see that stochastic cubic GDA can have a good performance on a small mini batch, which means we could do descent on a small mini-step and have a faster converge speed and lower total sample size.

Second we contrast stochastic cubic gda with stochastic gda under same initial point $\textbf{x}=[0,0,1]^T$ and $\textbf{y}=[1,1]^T$, with same batch-size = 100 and same learning rate $lr = 0.01$ at descent step.

\begin{figure}[htbp]

\centering
\includegraphics[width=0.95\linewidth]{emsnewsletter-template/pictures/cubic vs gda.png}

\caption{comparison $\Phi(x)$ of cubic GDA and classical GDA }\label{result1}
	
\end{figure}

Figure 2 shows stochastic cubic GDA has a obvious faster speed of convergence over classical GDA. It needs shorter time and less sample size to reach the minimax point, which illustrates cubic method really works. 

\subsection{Neural network simulation}

This section we compare the stochastic cubic GDA with the classical GDA using the example of a convolutional neural network. All these algorithms have a single-loop structure.

We decide to solve problem below using the MINST dataset.

\begin{equation}
    \min\limits_{\theta} \max\limits_{ \{ \xi_i \}_{i=1}^n} \frac{1}{n} \sum_{i=1}^n 
    \left[ \ell (h_{\theta} (\xi_i, y_i) ) - \lambda \Vert \xi_i - x_i \Vert^2 \right]
\end{equation}

where $n = 60k$ is the number of training samples, $\theta$ is the parameter of the neural network
and $(x_i, y_i)$ corresponds to the i-th image and label, respectively, $\xi_i$ refers to the adversarial sample corresponding to $x_i$, we choose cross-entropy loss function as $\ell$.

We set $\lambda$ = 2.0 that suffices to make the maximization part be strongly-concave. The network model we use is a convolution network that consists of two convolution blocks followed by two fully connected layers. Specifically, each convolution block contains a convolution layer, a max-pooling layer with stride step 2, and a ReLU activation layer. The convolution layers in the two blocks have 1, 10 input channels and 10, 20 output channels, respectively, and both of them have kernel size 5, stride step 1 and no padding. The two fully connected layers have input dimensions 320, 50 and output dimensions 50, 10, respectively.

In both algorithm, we randomly select a mini-batch with 512 size to do optimization. In validation step we randomly select 2000 images and labels as the test set. The learning rate of the ascent step in both algorithm is 0.1 and both do 20 steps of gradient ascend before do descend in each epoch. The descend learning rate in both algorithms is 0.01, while in stochastic cubic GDA we only do one step of cubic descend, in classical GDA we do 10 steps of gradient descend in each epoch. We use efficiency algorithm in this paper to estimate the cubic function, and the learning rate in solving the cubic problem is 0.1 and 0.001, respectively. Since it may be hard to evaluate the exact value of $\Phi(x)$, we run 100 gradient ascent steps to make $\xi$ close to the maximum and compute the loss as estimated $\Phi(x)$.

\begin{figure}[htbp]

\centering
\includegraphics[width=1\linewidth]{emsnewsletter-template/pictures/cubic vs gda2.png}

\caption{Left: comparison $\Phi(x)$ of three algorithms Right: comparison of robust test accuracy of three algorithms}\label{result2}
	
\end{figure}

Figure 3 (Left) compares the estimated objective function value achieved by both algorithms. It can be seen that cubic algorithm has a manifest superiority on the convergence over the other algorithm and is significantly faster. Figure 3 (Right) further demonstrates the advantage of stochastic cubic in robust test accuracy. It can be seen that the robust model trained by cubic method achieves a better robustness.

==> intro.tex <==
\section{Introduction}
Minimax optimization (a.k.a.\! two-player sequential zero-sum games) is a popular modeling framework that has broad applications in modern machine learning, including game theory \citep{ferreira2012minimax}, generative adversarial networks \citep{goodfellow2014generative}, adversarial training \citep{Sinha2017CertifyingSD}, reinforcement learning \citep{qiu2020single,ho2016generative,MultiAgent_Jiaming}, etc. A standard minimax optimization problem is shown below, where $f$ is a smooth bivariate function.
\begin{align}
	\min_{x\in \mathbb{R}^m}\max_{y\in \mathbb{R}^n}~ f(x,y). \tag{P}
\end{align} 
In the existing literature, many optimization algorithms have been developed to solve different types of minimax problems. Among them, a simple and popular algorithm is the gradient descent-ascent (GDA), which alternates between a gradient descent update on $x$ and a gradient ascent update on $y$ in each iteration. Specifically, the global convergence of GDA has been established for minimax problems under various types of global geometries, such as convex-concave-type geometry ($f$ is convex in $x$ and concave in $y$) \citep{nedic2009subgradient,du2019linear,mokhtari2020unified,zhang2020suboptimality}, bi-linear geometry \citep{neumann1928theorie,robinson1951iterative} and Polyak-{\L}ojasiewicz geometry \citep{nouiehed2019solving,yang2020global}, yet these geometries are not satisfied by general nonconvex minimax problems in modern machine learning applications.  
Recently, many studies proved the convergence of GDA in nonconvex minimax optimization for both nonconvex-concave problems \citep{lin2019gradient,nouiehed2019solving,xu2020unified} and nonconvex-strongly-concave problems \citep{lin2019gradient,xu2020unified,chen2021proximal}.
{In these studies, it has been shown that GDA converges sublinearly to a stationary point where the gradient of an envelope-type function $\Phi(x):=\max_y f(x,y)$ vanishes.}

Although GDA can find stationary points in nonconvex minimax optimization, the stationary points may include candidate solutions that are far more sub-optimal than global minimax points. However, finding global minimax points is in general NP-hard \citep{jin2019local}. Recently, \cite{jin2019local} proposes a notion of local minimax point that is computationally tractable and is close to global minimax point. Specifically, a local minimax point $(x, y)$ is a stationary point that satisfies the following second-order non-degeneracy conditions (see  \Cref{def: local} for the formal definition). 
\begin{align*}
    \nabla_{\!22} f(x, \!y) \prec \zero, ~\big[\nabla_{\!11} f - \nabla_{\!12} f (\nabla_{\!22} f)^{-1} \nabla_{\!21} f\big](x,\!y) \succeq \zero.
\end{align*}

In the existing literature, several studies have proposed Newton-type GDA algorithms for finding such local minimax points. Specifically, \cite{Wang2020follow} proposed a Follow-the-Ridge (FR) algorithm, which is a variant of GDA that applies a second-order correction term to the gradient ascent update. In particular, the authors showed that any strictly stable fixed point of
FR is a local minimax point, and vice versa.  In another work \citep{zhang2021newtontype}, the authors proposed two Newton-type GDA algorithms that are proven to locally converge to a local minimax point at a linear and super-linear convergence rate, respectively. However, these second-order-type GDA algorithms only have asymptotic convergence guarantees that require initializing sufficiently close to a local minimax point, and they do not have any global convergence guarantees. 
Therefore, we are motivated to ask the following fundamental questions.
 \begin{itemize}[leftmargin=*,topsep=0pt]
 	\item {\bf Q:} {\em Can we develop globally convergent {GDA-type} algorithms that can efficiently find local minimax points in nonconvex minimax optimization? What are their convergence rates and complexities?}
 \end{itemize}

%Developing and analyzing such an algorithm is nontrivial due to the following reasons: 1) we need to have a good understanding and characterization of both the first-order and second-order information of nonconvex minimax problems; 2) we need to develop a computationally feasible and efficient GDA algorithm that can leverage the local curvature of the function to escape saddle points; 3) we aim to develop a unified analysis framework that can characterize the convergence rate of this algorithm under different types of nonconvex geometry of the minimax problem. 


In this work, we provide comprehensive answers to these questions. We develop deterministic and stochastic {Newton-type GDA} algorithms that globally converge to local minimax points in nonconvex-strongly-concave minimax optimization, and study their convergence rates and sample complexities under standard assumptions. We summarize our contributions as follows.

%\vspace{1mm}
\subsection{Our Contributions}
%\vspace{1mm}
We consider the standard minimax optimization problem (P), where $f$ is twice-differentiable with Lipschitz continuous gradient and Hessian, and is nonconvex-strongly-concave. In this setting, we first show that local minimax points of $f$ are equivalent to second-order stationary points of the
envelope function $\Phi(x):=\max_{y\in \mathbb{R}^n} f(x,y)$. Then, inspired by the classic cubic regularization algorithm, we propose a {cubic-regularized GDA} (named Cubic-GDA) algorithm to find local minimax points. The algorithm uses gradient ascent to update $y$, which is then used to estimate the gradient and Hessian involved in the cubic regularization update for $x$ (see \Cref{algo: prox-minimax} for more details).

%Specifically, we propose Cubic-GDA -- a \red{Newton-type GDA} algorithm that leverages the classical cubic regularization technique to escape saddle points. Different from the standard cubic regularization algorithm that uses the Hessian information of the function, the Hessian of $\Phi(x)$ is not directly available in nonconvex minimax optimization, and hence we develop a rigorous and computationally feasible scheme in Cubic-GDA to estimate the Hessian. 

\textbf{Global convergence.} We show that Cubic-GDA admits an intrinsic potential function $H_t$ (see \Cref{prop: lyapunov}) that monotonically decreases over the iterations. Based on this property, we prove that every limit point of $\{x_t\}_t$ generated by Cubic-GDA is a local minimax point. Moreover, to achieve an $\epsilon$-accurate local minimax point, Cubic-GDA requires $\mathcal{O}\big(\kappa^{1.5}\epsilon^{-3}\big)$ number of cubic updates and $\mathcal{O}\big(\kappa^{2.5}\epsilon^{-3}\big)$ number of gradient ascent updates, where $\kappa>1$ denotes the problem condition number. 

\textbf{Asymptotic convergence.} By leveraging the potential function, we also characterize the asymptotic convergence rates of Cubic-GDA under a class of {\L}ojasiewicz-type local gradient geometry. Specifically, depending on the sharpness parameter of the local geometry, the asymptotic convergence rate of Cubic-GDA ranges from sub-linear convergence to super-linear convergence. These asymptotic convergence rates are orderwise faster than those of the standard GDA established in \citep{chen2021proximal} under the same type of local geometry. 
%\footnote{Note that the geometry parameter $\theta$ in this paper corresponds to $\frac{1}{1-\theta}$ in \citep{chen2021proximal}.}. 

\textbf{Sample complexity.} We further develop a stochastic variant of Cubic-GDA that applies sub-sampling to improve the sample complexity in large-scale minimax optimization. In particular, we adopt time-varying batch sizes in a way such that the induced gradient inexactness and Hessian inexactness are adapted to the optimization increment $\|x_t - x_{t-1}\|$ in the previous iteration. Consequently, to achieve an $\epsilon$-accurate local minimax point, we show that stochastic Cubic-GDA requires querying $\widetilde{\mathcal{O}}\big(\kappa^{3.5}\epsilon^{-7}\big)$ number of gradient samples and $\widetilde{\mathcal{O}}\big(\kappa^{2.5}\epsilon^{-5}\big)$ number of Jacobian samples.

%\vspace{-2mm}
% \begin{table}[ht]
% 	\caption{\red{Move to KL section.} Comparison of potential function value gap $H(z) - H^*$ convergence rates of Cubic-GDA and GDA under different parameterizations of {\L}ojasiewicz gradient geometry.}\label{table: 1}
% 	\center
% 	\vspace{0mm}
% 	\begin{tabular}{ccc}
% 		\toprule
% 		{Geometry parameter} & {GDA \citep{chen2021proximal}} & {\bf Cubic-GDA (This paper)} \\ \midrule
% 		$\theta\in(2,+\infty)$   &\makecell{ Super-linear convergence} & \makecell{Super-linear convergence}   \\
% 		\midrule
% 		$\theta=2$  & \makecell{Linear convergence} & \makecell{ Super-linear convergence}  \\
% 		\midrule
% 		$\theta \in (\frac{3}{2}, 2)$  & \makecell{Sub-linear convergence} & \makecell{Super-linear convergence}  \\
% 		\midrule
% 		$\theta = \frac{3}{2}$  & \makecell{Sub-linear convergence}& \makecell{Linear convergence} \\
% 		\midrule
% 		$\theta \in (1,\frac{3}{2})$  & \makecell{Sub-linear convergence}& \makecell{Sub-linear convergence} \\
% 		\bottomrule
% 	\end{tabular}
% \vspace{-2mm}
% \end{table}

\subsection{Other Related Work}\label{sec: related_work}
%\vspace{-2mm}
\textbf{Deterministic GDA algorithms:}
% \red{Many studies characterized the convergence of GDA in nonconvex minimax optimization. Specifically,
%  \cite{lin2019gradient,nouiehed2019solving,xu2020unified} studied the convergence of GDA in the nonconvex-concave setting whereas \cite{lin2019gradient,xu2020unified} focused on the nonconvex-strongly-concave setting. 
%  In these general nonconvex settings, it is shown that GDA converges to a certain stationary point at a sublinear rate. Recently, \cite{chen2021proximal}
%  proved the parameter convergence of proximal-GDA in regularized nonconvex-strongly-concave optimization under the Kurdyka-{\L}ojasiewicz geometry. The convergence rates obtained there are orderwise slower than that of Cubic-GDA.}
\cite{yang2020global} studied an alternating gradient descent-ascent (AGDA) algorithm in which the gradient ascent step uses the current variable $x_{t+1}$ instead of $x_t$. \cite{xu2020unified} studied an alternating gradient projection algorithm which applies $\ell_2$ regularizer to the local objective function of GDA followed by projection onto the constraint sets. \cite{daskalakis2018limit,mokhtari2020unified,zhang2020suboptimality} analyzed optimistic gradient descent-ascent (OGDA) which applies negative momentum to accelerate GDA. \cite{mokhtari2020unified} also studied an extra-gradient algorithm which applies two-step GDA in each iteration. \cite{nouiehed2019solving} studied multi-step GDA where multiple gradient ascent steps are performed, and they also studied the momentum-accelerated version.  \cite{cherukuri2017saddle,daskalakis2018limit,jin2019local} studied GDA in continuous time dynamics using differential equations. \cite{adolphs2019local} analyzed a second-order variant of the GDA algorithm. 
In a concurrent work \citep{luo2021finding}, the authors proposed a Minimax Cubic-Newton algorithm that is similar to our Cubic-GDA but adopts a different output rule. {Specifically, in iteration $t$, they terminate the algorithm based on the current increment $\|s_{t+1}\|$. As a comparison, our Output II terminates the algorithm based on $\|s_t\|\vee \|s_{t+1}\|$. This output rule is critical to develop the practical and adaptive sub-sampling scheme for our stochastic Cubic-GDA. 
In addition, we also analyze the last-iterate convergence of Cubic-GDA with Output I. Moreover, we develop a stochastic version of Cubic-GDA and analyze its sample complexity.}

%They characterize the computation complexity under a special type of inexactness that approximates the inverse Jacobian using matrix Chebyshev polynomials. As a comparison, this study focuses on analyzing the global and local convergence properties of Cubic-GDA.

% 1.  We also study last-iterate convergence; output II is different, helps develop practical stochastic sampling scheme later

% 2. Analysis is based on potential function, 

% 3. We also study stochastic version


\textbf{Stochastic GDA algorithms: } \cite{lin2019gradient,yang2020global} analyzed stochastic GDA and stochastic AGDA, which are direct extension of GDA and AGDA to the stochastic setting. Variance reduction techniques have been applied to stochastic minimax optimization, including SVRG-based \citep{du2019linear,yang2020global}, SPIDER-based \citep{xu2020gradient}, SREDA \citep{xu2020enhanced}, STORM \citep{qiu2020single} and its gradient free version \citep{huang2020accelerated}. \cite{xielower} studied the complexity lower bound of first-order stochastic algorithms for finite-sum minimax problem.



\textbf{Cubic regularization (CR):} {The CR algorithm dates back to \citep{Griewank}, where global convergence is established.} In \cite{Nesterov2006}, the author analyzed the convergence rate of CR to second-order stationary points in nonconvex optimization. In \citep{Nesterov2008}, the authors established the sub-linear convergence of CR for solving convex smooth problems, and they further proposed an accelerated version of CR with improved sub-linear convergence. \cite{Yue2018} studied the asymptotic convergence properties of CR under the error bound condition, and established the quadratic convergence of the iterates. 
%{Recently, \cite{Hallak2020} proposed a framework of two directional method for finding second-order stationary points in general smooth nonconvex optimization. The main idea is to search for a feasible direction toward the solution and is not based on cubic regularization.}
Several other works proposed different methods to solve the cubic subproblem of CR, e.g., \citep{Agarwal2017,Carmon2016,Cartis2011a}.
Another line of work aimed at improving the computation efficiency of CR by solving the cubic subproblem with inexact gradient and Hessian information. In particular, \cite{Saeed2017} proposed an inexact CR for solving convex problem. Also, \cite{Cartis2011b} proposed an adaptive inexact CR for nonconvex optimization, whereas \cite{Jiang2017} further studied the accelerated version for convex optimization. Several studies explored subsampling schemes to implement inexact CR algorithms, e.g., \citep{kohler2017,Xu2017,Zhou2018,Wang2018}. 




==> introduction_unused.tex <==
\section{Introduction}
A majority of machine learning applications are naturally formulated as nonconvex optimization due to the complex mechanism of the underlying model. Typical examples include training neural networks in deep learning \cite{Goodfellow2016}, low-rank matrix factorization \cite{RongGe2016,Bhojanapalli2016}, phase retrieval \cite{Candes2015,Zhang2017}, etc. In particular, these machine learning problems take the generic form
\begin{align*}
\min_{\xb\in \RR^d}~~f(\xb), \tag{P}
\end{align*}
where the objective function $f: \RR^d \to \RR$ is a differentiable and nonconvex function, and usually corresponds to the total loss over a set of data samples. 
Traditional first-order algorithms such as gradient descent can produce a solution $\bar{\xb}$ that satisfies the first-order stationary condition, i.e., $\nabla f (\bar{\xb}) = \zero$. However, such first-order stationary condition does not exclude the possibility of approaching a saddle point, which can be a highly suboptimal solution and therefore deteriorate the performance. 

Recently in the machine learning community, there has been an emerging interest in designing algorithms to scape saddle points in nonconvex optimization, and one popular algorithm is the cubic-regularized Newton's algorithm \cite{Nesterov2006,Agarwal2017,Yue2018}, which is also referred to as cubic regularization (CR) for simplicity. Such a second-order method exploits the Hessian information and produces a solution $\bar{\xb}$ for problem (P) that satisfies the second-order stationary condition, i.e., 
$$(\text{second-order stationary}):\quad \nabla f (\bar{\xb}) = \zero, ~\nabla^2 f(\bar{\xb}) \succeq \zero.$$
The second-order stationary condition ensures CR to escape saddle points wherever the corresponding Hessian matrix has a negative eigenvalue (i.e., strict saddle points \cite{Sun2015}). In particular, many nonconvex machine learning problems have been shown to exclude spurious local minima and have only strict saddle points other than global minima \cite{Baldi1989,Sun2017,RongGe2016,zhou2018}. In such a desirable case, CR is guaranteed to find the global minimum for these nonconvex problems. 
To be specific, given a proper parameter $M>0$, CR generates a variable sequence $\{ \xb_{k}\}_k$ via the following update rule
\begin{align}
	\text{(CR)}~ \xb_{k+1} \in \argmin_{\yb \in \RR^d} ~\inner{\yb - \xb_{k}}{\nabla f (\xb_{k})} + \frac{1}{2} (\yb - \xb_{k})^\ttop \nabla^2 f(\xb_{k})  (\yb - \xb_{k}) + \frac{M}{6} \|\yb - \xb_{k}\|^3. \label{eq: CR}
\end{align}
Intuitively, CR updates the variable by minimizing an approximation of the objective function at the current iterate. This approximation is essentially the third-order Taylor's expansion of the objective function. We note that computationally efficient solver has been proposed for solving the above cubic subproblem \cite{Agarwal2017}, and it was shown that the resulting computation complexity of CR to achieve a second-order stationary point serves as the state-of-the-art among existing algorithms that achieve the second-order stationary condition.
%is lower than that of gradient descent to achieve a first-order stationary point.

Several studies have explored the convergence of CR for nonconvex optimization. Specifically, the pioneering work \cite{Nesterov2006} first proposed the CR algorithm and showed that the variable sequence $\{\xb_{k} \}_k$ generated by CR has second-order stationary limit points and converges sub-linearly. Furthermore, the gradient norm along the iterates was shown to converge quadratically (i.e., super-linearly) given an initialization with positive definite Hessian. Moreover, the function value along the iterates was shown to converge super-linearly under a certain gradient dominance condition of the objective function. Recently, \cite{Yue2018} studied the asymptotic convergence rate of CR under the local error bound condition, and established the quadratic convergence of the distance between the variable and the solution set. 
Clearly, these results demonstrate that special geometrical properties (such as the gradient dominance condition and the local error bound) enable much faster convergence rate of CR towards a second-order stationary point. However, these special conditions may fail to hold for generic complex objectives involved in practical applications. Thus, it is desired to further understand the convergence behaviors of CR for optimizing nonconvex functions over a broader spectrum of geometrical conditions.

The Kurdyka-{\L}ojasiewicz (K{\L}) property (see \Cref{sec: pre} for details) \cite{Bolte2007,Bolte2014} serves as such a candidate. As described in \Cref{sec: pre}, the \KL property captures a broad spectrum of the local geometries that a nonconvex function can have and is parameterized by a parameter $\theta$ that changes over its allowable range.  In fact, the \KL property has been shown to hold ubiquitously for most practical functions (see \Cref{sec: pre} for a list of examples). 
The \KL property has been exploited extensively to analyze the convergence rate of various {\em first-order} algorithms for nonconvex optimization, e.g., gradient method \cite{Attouch2009,Li2017}, alternating minimization \cite{Bolte2014} and distributed gradient methods \cite{Zhou2016}.
But it has not been exploited to establish the {\em convergence rate} of second-order algorithms towards second-order stationary points.  
In this paper, we exploit the \KL property of the objective function to provide a comprehensive study of the convergence rate of CR for nonconvex optimization. We anticipate our study to substantially advance the existing understanding of the convergence of CR to a much broader range of nonconvex functions. We summarize our contributions as follows.
\vspace{-5pt}
\subsection{Our Contributions}
\vspace{-5pt}
We characterize the convergence rate of CR locally towards second-stationary points for nonconvex optimization under the \KL property of the objective function. Our results also compare and contrast the different order-level of guarantees that \KL yields between the first and second-order algorithms.
Also, our analysis characterizes the convergence property for a range of \KL parameter $\theta$,  which requires the development of different recursive inequalities for various cases.

\textbf{Gradient norm \& least eigenvalue of Hessian:}
We characterize the asymptotic convergence rates of the sequence of gradient norm $\{\|\nabla f(\xb_{k})\| \}_k$ and the sequence of the least eigenvalue of Hessian $\{\lambda_{\min} (\nabla^2 f(\xb_{k}))\}_k$ generated by CR. We show that CR meets the second-order stationary condition at a (super)-linear rate in the parameter range $\theta \in [\frac{1}{3}, 1]$ for the \KL property, while the convergence rates become sub-linearly in the parameter range $\theta \in (0, \frac{1}{3})$ for the \KL property.

\textbf{Function value gap \& variable distance:} 
We characterize the asymptotic convergence rates of the function value sequence $\{f(\xb_{k})\}_k$ and the variable sequence $\{\xb_{k}\}_k$ to the function value and the variable of a second-order stationary point, respectively. The obtained convergence rates range from sub-linearly to super-linearly depending on the parameter $\theta$ associated with the \KL property. Our convergence results generalize the existing ones established in \cite{Nesterov2006} corresponding to special cases of $\theta$ to the full range of $\theta$. Furthermore, these types of convergence rates for CR are orderwise faster than the corresponding convergence rates of the first-order gradient descent algorithm in various regimes of the \KL parameter $\theta$ (see \Cref{table: 1} and \Cref{table: 2}  for the comparisons). 

Based on the \KL property, we establish a generalized local error bound condition (referred to as the \KL error bound). The \KL error bound further leads to characterization of the convergence rate of distance between the variable and the solution set, which ranges from sub-linearly to super-linearly depending on the parameter $\theta$ associated with the \KL property.
This result generalizes the existing one established in \cite{Yue2018} corresponding to a special case of $\theta$ to the full range of $\theta$. 


\vspace{-5pt}
\subsection{Related Work}
\vspace{-5pt}
\textbf{Cubic regularization:} CR algorithm was first proposed in \cite{Nesterov2006}, in which the authors analyzed the convergence of CR to second-order stationary points for nonconvex optimization. In \cite{Nesterov2008}, the authors established the sub-linear convergence of CR for solving convex smooth problems, and they further proposed an accelerated version of CR with improved sub-linear convergence. Recently, \cite{Yue2018} studied the asymptotic convergence properties of CR under the error bound condition, and established the quadratic convergence of the iterates. Several other works proposed different methods to solve the cubic subproblem of CR, e.g., \cite{Agarwal2017,Carmon2016,Cartis2011a}.


\textbf{Inexact-cubic regularization:} 
Another line of work aimed at improving the computation efficiency of CR by solving the cubic subproblem with inexact gradient and Hessian information. In particular, \cite{Saeed2017,Jin2017} proposed an inexact CR for solving convex problem and nonconvex problems, respectively. Also, \cite{Cartis2011b} proposed an adaptive inexact CR for nonconvex optimization, whereas \cite{Jiang2017} further studied the accelerated version for convex optimization. Several studies explored subsampling schemes to implement inexact CR algorithms, e.g., \cite{kohler2017,Xu2017,Zhou2018,Wang2018}. 


\textbf{\KL property:} The \KL property was first established in \cite{Bolte2007}, and was then widely applied to characterize the asymptotic convergence behavior for various first-order algorithms for nonconvex optimization \cite{Attouch2009,Li2017,Bolte2014,Zhou2016,Zhou_2017a}. The \KL property was also exploited to study the convergence of second-order algorithms such as generalized Newton's method \cite{Frankel2015} and the trust region method \cite{Noll2013}. However, these studies did not characterize the convergence rate and the studied methods cannot guarantee to converge to second-order stationary points, whereas this paper provides this type of results.

\textbf{First-order algorithms that escape saddle points:} Many first-order algorithms are proved to achieve second-order stationary points for nonconvex optimization. For example, online stochastic gradient descent \cite{Ge2015}, perturbed gradient descent \cite{Jin2017}, gradient descent with negative curvature \cite{Carmon2016,Liu2017} and other stochastic algorithms \cite{Zhu2017}.



==> jacobian.tex <==
\section{Compute Jacobian-Vector Product}\label{app: jacob}

In \Cref{algo: prox-minimax} (and similarly for \Cref{algo: prox-minimax-stoc}), the key step is the cubic regularization update, which requires solving the following generic cubic sub-problem.
\begin{align*}
    \mathop{\arg\!\min}_s \nabla_{1}f(x, y)^{\top}s + \frac{1}{2} s^{\!\top}G(x, y)s+\frac{1}{6\eta_x}\|s\|^3, ~~\text{where}~~G(x, y) = \big[\nabla_{11} f - \nabla_{12} f (\nabla_{22} f)^{-1} \nabla_{21} f\big](x,y).
\end{align*}
In the literature, many gradient-based cubic-solvers have been developed to efficiently solve cubic sub-problems, and their convergence guarantee and computation complexity are well established \citep{Carmon2016,Tripuraneni18}. In particular, when implementing these cubic-solvers to solve the above cubic sub-problem, one needs to query the Hessian-vector product $G(x,y)\cdot u$ for a general vector $u$. This quantity can be efficiently computed as we elaborate below. 

First, note that for any vector $v$, the Jacobian-vector products $\nabla_{k\ell} f(x,y)\cdot v$ for all $k,\ell\in\{1,2\}$ can be computed via standard auto-differentiation as follows
\begin{align*}
    \nabla_{k\ell} f(x,y)\cdot v = \nabla_\ell\big(\nabla_k f(x,y)^\top v\big), \quad \forall k,\ell\in\{1,2\}.
\end{align*}
Therefore, we can query the above Jacobian-vector product oracle to compute 
\begin{align*}
    z_{1} := \nabla_{11} f(x,y)\cdot u, \quad z_{2} := \nabla_{21} f(x,y)\cdot u.
\end{align*}
Then, we have  $G(x,y)\cdot u = z_{1} - \big[\nabla_{12} f (\nabla_{22} f)^{-1}\big](x,y)\cdot z_{2}$. Note that the quantity $z_{3} := (\nabla_{22} f(x,y))^{-1}\cdot z_{2}$ can be computed by solving the linear system 
\begin{align*}
    \nabla_{22} f(x,y)\cdot z_{3} = z_{2}
\end{align*}
using standard conjugate gradient solvers. Lastly, we query another Jacobian-vector product oracle to compute 
\begin{align*}
    z_{4}:=\nabla_{12} f(x,y)\cdot z_{3}.
\end{align*}
Finally, the Hessian-vector product can be computed as $G(x,y)\cdot u = z_{1} - z_{4}$.

==> preliminary.tex <==
{\bf Notation:} For a bivariate function $f(x,y)$, we denote $\nabla_1 f, \nabla_2 f$ as the partial gradients with respect to the first and the second input arguments of $f$, respectively. We also denote the Jacobian blocks with regard to the two input arguments as $\nabla_{11} f, \nabla_{22} f, \nabla_{12} f, \nabla_{21} f$. We denote the $\max$ and $\min$ operators as $\vee$ and $\wedge$, respectively.

\section{Problem Formulation and Preliminaries}\label{sec: pre}

We consider the following standard minimax optimization problem (P), where $f$ is a nonconvex-strongly-concave bivariate function and is twice-differentiable. Throughout the paper, we define the envelope function $\Phi(x):=\max_{y\in \mathbb{R}^n} f(x,y)$.
\begin{align}
	\min_{x\in \mathbb{R}^m}\max_{y\in \mathbb{R}^n}~ f(x,y). \tag{P}
\end{align} 
Our goal is to develop algorithms that globally converge to local minimax points of (P), which are defined to satisfy the following set of conditions \citep{jin2019local}. 
\begin{definition}[Local minimax point]\label{def: local}
A point $(x, y)$ is a local minimax point of (P) if it satisfies 
\begin{enumerate}[leftmargin=*,topsep=0mm,itemsep=1mm]
    \item Stationary: $\nabla_1 f(x,y)=\zero,~ \nabla_2 f(x,y)=\zero$;
    \item Non-degeneracy: $\nabla_{22} f(x, y) \prec \zero$, and \\ $\big[\nabla_{11} f - \nabla_{12} f (\nabla_{22} f)^{-1} \nabla_{21} f\big](x,y) \succeq \zero$.
\end{enumerate}
\end{definition}
Local minimax points are different from global minimax points, which require $x$ and $y$ to be the global minimizer and global maximizer of the functions $\Phi(x)$ and $f(x, \cdot)$, respectively. 
In general minimax optimization, global minimax points can be neither local minimax points nor even stationary points \citep{jin2019local}.  
However, it has been shown that global minimax necessarily implies local minimax in nonconvex-strongly-concave optimization \citep{jin2019local}. Moreover, under mild conditions, many machine learning problems have been shown to possess local minimax points, e.g., generative adversarial networks (GANs) \citep{Nagarajan17,zhang2021newtontype}, distributional robust machine learning \citep{sinha2017certifiable}, etc. 



Throughout the paper, we adopt the following standard assumptions on the minimax optimization problem (P) \citep{lin2019gradient,jin2019local,zhang2021newtontype}.
\begin{assum}\label{assum: f}
	The minimax problem $\mathrm{(P)}$ satisfies:
	\begin{enumerate}[leftmargin=*,topsep=0mm,itemsep=1mm]
		\item Function $f(\cdot,\cdot)$ is $L_1$-smooth and function $f(x,\cdot)$ is $\mu$-strongly concave for any fixed $x$;
		\item The Jacobian mappings $\nabla_{11} f$, $\nabla_{12} f$, $\nabla_{21} f$, $\nabla_{22} f$ are $L_2$-Lipschitz continuous;
		\item Function $\Phi(x):=\max_{y\in \mathbb{R}^n} f(x,y)$ is bounded below and has compact sub-level sets.
	\end{enumerate}
\end{assum} 

To elaborate, {item 1 considers the class of nonconvex-strongly-concave functions $f$ that has been widely studied in the minimax optimization literature \citep{lin2019gradient,jin2019local,xu2020unified,lu2020hybrid}}, and it is also satisfied by many machine learning applications. 
Item 2 assumes that the block Jacobian matrices of $f$ are Lipschitz continuous, which is a standard assumption for analyzing second-order optimization algorithms \citep{Nesterov2006,Agarwal2017}. Moreover, item 3 {guarantees that the minimax problem has at least one solution.} 

Under \Cref{assum: f}, the following properties regarding the gradient of the minimax problem (P) have been proved in the literature. Throughout, we denote $\kappa=L_1/\mu$ as the condition number. 
\begin{restatable}{proposition}{prop1}{\citep{lin2019gradient}}\label{prop_1}
	Let \Cref{assum: f} hold. Then, the mapping $y^*(x):=\arg\max _{y\in \mathbb{R}^n}f(x,y)$ is unique for every fixed $x$. 
	Moreover, it holds that
	\begin{enumerate}[leftmargin=*,topsep=0mm,itemsep=1mm]
		\item Mapping $y^*(x)$ is $\kappa$-Lipschitz continuous; \label{item: ystar_lipschitz}
		\item Function $\Phi(x)$ is $L_1(1+\kappa)$-smooth and $\nabla\Phi(x)=\nabla_1 f(x,y^*(x))$. \label{item: Phi_Lsmooth}
	\end{enumerate}
\end{restatable}



% \begin{definition}(Subdifferential and critical point, \cite{rockafellar2009variational})\label{def:sub}
% 	The Frech\'et subdifferential $\widehat\partial h$ of function $h$ at $x\in \dom h$ is the set of $u\in \mathbb{R}^d$ defined as
% 	\begin{align*}
% 	\widehat\partial h(x) := \Big\{u: \liminf_{z\neq x, z\to x} \frac{h(z) - h(x) - u^\intercal(z-x)}{\|z-x\|} \ge 0 \Big\},
% 	\end{align*}
% 	and the limiting subdifferential $\partial h$ at $x\in\dom h$ is the graphical closure of $\widehat\partial h$ defined as:
% 	\begin{align*}
% 	\partial h(x) := \{ u: \exists x_k \to x, h(x_k) \to h(x), \red{u_k \in \widehat{\partial} h(x_k), u_k \to u} \}.
% 	\end{align*}
% 	The set of \textbf{critical points} of $h$ is defined as $\mathbf{\crit}\!~h := \{ x: \zero\in\partial h(x) \}$. 
% \end{definition}
% Throughout, we refer to the limiting subdifferential as subdifferential. We note that  subdifferential is a generalization of gradient (when $h$ is differentiable) and subgradient (when $h$ is convex) to the nonconvex setting. In particular, any local maximizer of $h$ must be a critical point.
 
%so the critical point defined in \Cref{def:sub} also generalizes its usual definition for smooth or convex functions. 




















==> proposition1proof.tex <==
%In this supplementary material, we present the proof of all the results claimed in the paper. 

\section{Supporting Lemmas}
We first prove the following auxiliary lemma that bounds the spectral norm of the Jacobian matrices. 
\begin{lemma}\label{lemma_HessBound}
    Let \Cref{assum: f} hold. Then, for any $x\in \mathbb{R}^m$ and $y\in \mathbb{R}^n$, the Jacobian matrices of $f(x,y)$ {and $G(x,y)=\big[\nabla_{11} f - \nabla_{12} f (\nabla_{22} f)^{-1} \nabla_{21} f\big](x,y)$} satisfy the following bounds.
    \begin{align}
        &\|[\nabla_{22} f(x,y)]^{-1}\|\le \mu^{-1}, \label{HessInv_up}\\
        &\|\nabla_{12} f(x,y)\|=\|\nabla_{21} f(x,y)\|\le L_1, \label{Hess_below}\\
        &{\|\nabla_{11} f(x,y)\|\le L_1,} \label{Hess_below2}\\
        &{\|G(x,y)\|\le L_1(1+\kappa).}\label{G_up}
    \end{align}
    The same bounds also hold for $\widehat{\nabla}_{11} f$, $\widehat{\nabla}_{12} f$, $\widehat{\nabla}_{21} f$, $\widehat{\nabla}_{22} f$  and $\widehat{G}$ defined in Section \ref{sec: stoc} under \Cref{assum: fi}.
\end{lemma}
\begin{proof}
    We first prove \cref{HessInv_up}. Consider any $x\in \mathbb{R}^m$ and $y\in \mathbb{R}^n$. By \Cref{assum: f} we know that $f(x,\cdot)$ is $\mu$-strongy concave, which implies that $-\nabla_{22} f(x,y)\succeq \mu I$. Thus, we further conclude that 
    $$\|[\nabla_{22} f(x,y)]^{-1}\|=\lambda_{\max}\big([-\nabla_{22} f(x,y)]^{-1}\big)=\Big(\lambda_{\min}\big(-\nabla_{22} f(x,y)\big)\Big)^{-1}\le \mu^{-1}.$$
    
    %Define the Frobenius norm of a matrix $A=[a_{ij}]$ as $\|A\|_F:=\sqrt{\sum_{ij}a_{ij}^2}$. Then, and $u\in \mathbb{R}^d$ ($d$ is the dimensionality of $\mathbb{R}^n$)
    Next, we prove eq. \eqref{Hess_below}. Consider any $x, u\in \mathbb{R}^m$ and $y\in \mathbb{R}^n$, we have
    \begin{align}
        \|\nabla_{21} f(x,y)u\|=&\Big\|\frac{\partial}{\partial t}\nabla_2 f(x+tu,y)\Big|_{t=0}\Big\|\nonumber\\
        =&\Big\|\lim_{t\to 0} \frac{1}{t}\big[\nabla_2 f(x+tu,y)-\nabla_2 f(x,y)\big]\Big\|\nonumber\\
        =& \lim_{t\to 0} \frac{1}{|t|}\big\|\nabla_2 f(x+tu,y)-\nabla_2 f(x,y)\big\| \nonumber\\
        \le& \lim_{t\to 0} \frac{L_1}{|t|}\big\|tu\big\|=L_1\|u\|,
    \end{align}
    which implies that $\|\nabla_{21} f(x,y)\|\le L_1$. Since $f$ is twice differentiable and has continuous second-order derivative, we have $\nabla_{12} f(x,y)^{\top}=\nabla_{21} f(x,y)$, and hence eq. \eqref{Hess_below} follows. {The proof of eq. \eqref{Hess_below2} is similar.
    
    Finally, eq. \eqref{G_up} can be proved as follows using eqs. \eqref{HessInv_up}\&\eqref{Hess_below}.
    \begin{align}
        \|G(x,y)\|\le \|\nabla_{11} f(x,y)\| + \|\nabla_{12} f(x,y)\| \|\nabla_{22} f^{-1}(x,y)\| \|\nabla_{21} f(x,y)\| \le L_1 + L_1\mu^{-1} L_1 =L_1(1+\kappa). \nonumber
    \end{align}
    The proof is similar for the stochastic minimax optimization problem (Q) in Section \ref{sec: stoc} under \Cref{assum: fi}.
    }
\end{proof}

The following lemma restates Lemma 3 of \cite{wang2018note}. 
\begin{lemma}\label{lemma_CRsol}
    The solution $s_{k+1}$ of the cubic regularization problem in Algorithm \ref{algo: prox-minimax} satisfies the following conditions, 
    \begin{align}
        \nabla f(x_t,y_{t+1})+G(x_t,y_{t+1})s_{t+1}+\frac{1}{2\eta_x}\|s_{t+1}\|s_{t+1}=&~ \zero, \label{eq: CRcond1}\\
        G(x_t,y_{t+1})+\frac{1}{2\eta_x}\|s_{t+1}\|I\succeq& ~\mathbf{O}, \label{eq: CRcond2}\\
        \nabla f(x_t,y_{t+1})^{\top}s_{t+1}+\frac{1}{2}s_{t+1}^{\top}G(x_t,y_{t+1})s_{t+1} \le& -\frac{1}{4\eta_x}\|s_{t+1}\|^3. \label{eq: CRcond3}
    \end{align}
\end{lemma}

\begin{restatable}{lemma}{lemmaIfErrSmallNoKL}\label{lemma_ifErrSmall_noKL}
    Suppose the gradient $\nabla_1 f(x_t, y_{t+1})$ and Hessian $G(x_t,y_{t+1})$ involved in the cubic-regularization step in Algorithm \ref{algo: prox-minimax} satisfy the following bounds for all $t\le T'-1$ with $T'=\min\{t\ge 0: \|s_{t-1}\|\vee \|s_t\|\le\epsilon'\}$:
    \begin{align}
        &\|\nabla\Phi(x_t)-\nabla_1 f(x_t, y_{t+1})\| \le \beta(\|s_t\|^2+\epsilon'^2),\label{eq: grad_goal_noKL}\\ 
        &\|\nabla^2\Phi(x_t)-G(x_t,y_{t+1})\| \le \alpha(\|s_t\|+\epsilon'). \label{eq: Hess_goal_noKL}
    \end{align}
    
    Then, choosing $\eta_x\le (9L_{\Phi}+18\alpha+28\beta)^{-1}$, the sequence $\{x_t\}_t$ generated by Algorithm \ref{algo: prox-minimax} satisfies that for all $t\le T'-2$,
    \begin{align}
        &H_{t+1}-H_t \le -(L_{\Phi}+\alpha+\beta)(\|s_{t+1}\|^3+\|s_t\|^3), \label{eq: Hdec2_noKL}
    \end{align}
    where $H_t=\Phi(x_t)+(L_{\Phi}+2\alpha+3\beta)\|x_t-x_{t-1}\|^3$. The same conclusion holds for Algorithm \ref{algo: prox-minimax-stoc} by replacing $\nabla_1 f(x_t,y_{t+1})$, $G(x_t,y_{t+1})$ with their stochastic estimators $\widehat{\nabla}_1 f(x_t,y_{t+1})$, $\widehat{G}(x_t,y_{t+1})$ respectively. 
\end{restatable}

\begin{proof}
The proof logic follows that of the proof of Theorem 1 in \cite{wang2019stochastic}.
By the Lipschitz continuity of the Hessian of $\Phi$, we obtain that
\begin{align}
    &\Phi(x_{t+1})-\Phi(x_t) \nonumber\\
    &\le \nabla \Phi(x_t)^{\top} (x_{t+1}-x_t) + \frac{1}{2}(x_{t+1}-x_t)^{\top} \nabla^2 \Phi(x_t)  (x_{t+1}-x_t) + \frac{L_{\Phi}}{6} \|x_{t+1}-x_t\|^3 \nonumber\\
    &= \nabla_1 f(x_t, y_{t+1})^{\top} s_{t+1}  + \frac{1}{2}s_{t+1}^{\top} G(x_t,y_{t+1}) s_{t+1} + \frac{L_{\Phi}}{6} \|s_{t+1}\|^3 \nonumber\\
    &\quad +\big(\nabla \Phi(x_t)-\nabla_1 f(x_t, y_{t+1})\big)^{\top} s_{t+1} + \frac{1}{2}s_{t+1}^{\top} \big(\nabla^2 \Phi(x_t)-G(x_t,y_{t+1})\big) s_{t+1}\nonumber\\
    &\stackrel{(i)}{\le}  \Big(\frac{L_{\Phi}}{6}-\frac{1}{4\eta_x}\Big)\|s_{t+1}\|^3 +
    \beta \|s_{t+1}\|(\|s_t\|^2+\epsilon'^2) + \frac{\alpha}{2}\|s_{t+1}\|^2(\|s_t\|+\epsilon') \nonumber\\
    &\stackrel{(ii)}{\le} \Big(\frac{L_{\Phi}}{6}-\frac{1}{4\eta_x}\Big)\|s_{t+1}\|^3 + \Big(\frac{\alpha}{2}+\beta\Big)(2\|s_{t+1}\|^3+\|s_t\|^3+\epsilon'^3) \nonumber\\
    &\stackrel{(iii)}{\le} \Big(\frac{L_{\Phi}}{6}-\frac{1}{4\eta_x}\Big)\|s_{t+1}\|^3 + \Big(\frac{\alpha}{2}+\beta\Big)(3\|s_{t+1}\|^3+2\|s_t\|^3) \nonumber\\
    &\le -\Big(\frac{1}{4\eta_x}-\frac{L_{\Phi}}{6}-\frac{3\alpha}{2}-3\beta\Big)\|s_{t+1}\|^3 + (\alpha+2\beta)\|s_t\|^3, \nonumber\\
    &\stackrel{(iv)}{\le} -(2L_{\Phi}+3\alpha+4\beta)\|s_{t+1}\|^3 + (\alpha+2\beta)\|s_t\|^3\nonumber
\end{align}
where (i) uses eqs. \eqref{eq: CRcond3}, \eqref{eq: grad_goal_noKL}\& \eqref{eq: Hess_goal_noKL}, (ii) uses the inequality that $ab^2\le a^3\vee b^3\le a^3+b^3, \forall a,b\ge 0$, (iii) uses $\epsilon'^3\le \|s_t\|^3\vee\|s_{t+1}\|^3\le \|s_t\|^3+\|s_{t+1}\|^3, \forall 0\le t\le T'-2$ based on the termination criterion of $T'$, and (iv) uses $\eta_x\le (9L_{\Phi}+18\alpha+28\beta)^{-1}$. Eq. \eqref{eq: Hdec2_noKL} follows from the above inequality by defining $H_t=\Phi(x_t)+(L_{\Phi}+2\alpha+3\beta)\|x_t-x_{t-1}\|^2$. 

Note that the cubic-regularization step in Algorithm \ref{algo: prox-minimax-stoc} 
simply replaces $\nabla_1 f(x_t,y_{t+1})$, $G(x_t,y_{t+1})$ in Algorithm \ref{algo: prox-minimax} with their stochastic estimators $\widehat{\nabla}_1 f(x_t,y_{t+1})$, $\widehat{G}(x_t,y_{t+1})$ respectively. Hence, eq. \eqref{eq: Hdec2_noKL} holds for Algorithm \ref{algo: prox-minimax-stoc} after such replacement in eqs. \eqref{eq: grad_goal_noKL} \& \eqref{eq: Hess_goal_noKL}.
\end{proof}

\begin{lemma}\label{lemma_general_rate}
    Suppose all the conditions of Lemma \ref{lemma_ifErrSmall_noKL} hold. If $T\ge \frac{\Phi(x_0)-\Phi^*+(L_{\Phi}+3\alpha+4\beta)\epsilon'^2}{(L_{\Phi}+\alpha+\beta)\epsilon'^3}$ in Algorithm \ref{algo: prox-minimax}, then $T'=\min\{t\ge 1: \|s_{t-1}\|\vee \|s_t\|\le\epsilon'\}\le \frac{\Phi(x_0)-\Phi^*+(L_{\Phi}+3\alpha+4\beta)\epsilon'^2}{(L_{\Phi}+\alpha+\beta)\epsilon'^3}\le T$. Consequently, the Output II of Algorithm \ref{algo: prox-minimax} has the following convergence rate
    \begin{align}
        &\|\nabla \Phi(x_{T'})\| \le \Big(\frac{1}{2\eta_x}+L_{\Phi}+2\alpha+2\beta\Big) \epsilon'^2, \label{eq: grad_rate_early}\\
        &\nabla^2 \Phi(x_{T'}) \succeq -\Big(\frac{1}{2\eta_x}+L_{\Phi}+2\alpha\Big)\epsilon'I. \label{eq: Hess_rate_early}
    \end{align}
    The same conclusion holds for Algorithm \ref{algo: prox-minimax-stoc} by replacing $\nabla_1 f(x_t,y_{t+1})$, $G(x_t,y_{t+1})$ in the conditions \eqref{eq: grad_goal_noKL} \& \eqref{eq: Hess_goal_noKL} with their stochastic estimators $\widehat{\nabla}_1 f(x_t,y_{t+1})$, $\widehat{G}(x_t,y_{t+1})$ respectively. 
\end{lemma}
\begin{proof}
The proof logic follows that of the proof of Theorem 1 in \cite{wang2019stochastic}.
%The proof logic is similar to the end of the proof of Theorem 1 in \cite{wang2019stochastic}. 

Suppose $T'\le T$ does not hold, i.e., $\|s_{t-1}\|\vee \|s_t\|>\epsilon', \forall 1\le t\le T$, which implies that eq. \eqref{eq: Hdec2_noKL} holds for all $0\le t\le T-1$ based on Lemma \ref{lemma_ifErrSmall_noKL}.

On one hand, telescoping eq. \eqref{eq: Hdec2_noKL} over $t=0,1,\ldots,T-1$ yield that
\begin{align}
    H_0-H_T&\ge
    (L_{\Phi}+\alpha+\beta)\sum_{t=0}^{T-1}(\|s_{t+1}\|^3+\|s_t\|^3) \nonumber\\
    &\ge (L_{\Phi}+\alpha+\beta)\sum_{t=0}^{T-1}(\|s_t\|\vee\|s_{t+1}\|)^3 \nonumber\\
    &> T(L_{\Phi}+\alpha+\beta)\epsilon'^3\nonumber\\
    &\ge \Phi(x_0)-\Phi^*+(L_{\Phi}+3\alpha+4\beta)\epsilon'^2.  \label{eq: Hdiff_low}
\end{align}
On the other hand, recalling the definition of $H_t$ in Lemma \ref{lemma_ifErrSmall_noKL}, we have
\begin{align}
    H_0-H_T&=\Phi(x_0)-\Phi(x_T)+(L_{\Phi}+2\alpha+3\beta)(\|s_0\|^2-\|s_T\|^2) \nonumber\\
    &\stackrel{(i)}{\le} \Phi(x_0)-\Phi^*+(L_{\Phi}+3\alpha+4\beta)\epsilon'^2, \label{eq: Hdiff_up}
\end{align}
where (i) uses $\|s_0\|=\epsilon'$ and $\Phi(x_T)\ge \Phi^*=\min_{x\in\mathbb{R}^m}\Phi(x)$. Note that eqs. \eqref{eq: Hdiff_low} \& \eqref{eq: Hdiff_up} contradict. Therefore, we must have $1\le T'\le T$ for any $T\ge \frac{\Phi(x_0)-\Phi^*+(L_{\Phi}+3\alpha+4\beta)\epsilon'^2}{(L_{\Phi}+\alpha+\beta)\epsilon'^3}$, which implies that $T'\le \frac{\Phi(x_0)-\Phi^*+(L_{\Phi}+3\alpha+4\beta)\epsilon'^2}{(L_{\Phi}+\alpha+\beta)\epsilon'^3}\le T$.  

Finally, we conclude that 
\begin{align}
&\|\nabla \Phi(x_{T'})\|\nonumber\\
&\overset{(i)}{=}\Big\|\nabla \Phi(x_{T'})-\nabla f(x_{T'-1},y_{T'}) -G(x_{T'-1},y_{T'}) s_{T'} -\frac{1}{2\eta_x}\|s_{T'}\|s_{T'}\Big\| \nonumber\\
&\le \|\nabla \Phi(x_{T'})-\nabla \Phi(x_{T'-1})-\nabla^2 \Phi(x_{T'-1})s_{T'}\| + \|\nabla \Phi(x_{T'-1})-\nabla f(x_{T'-1},y_{T'})\|\nonumber\\
&\quad + \|\nabla^2 \Phi(x_{T'-1})s_{T'}-G(x_{T'-1},y_{T'}) s_{T'}\| + \frac{1}{2\eta_x}\|s_{T'}\|^2 \nonumber\\
&\overset{(ii)}{\le} \Big(L_{\Phi}+\frac{1}{2\eta_x}\Big)\|s_{T'}\|^2  +\beta(\|s_{T'-1}\|^2+\epsilon'^2) +\alpha(\|s_{T'-1}\|+\epsilon')\|s_{T'}\|\nonumber\\
&\overset{(iii)}{\le} \Big(\frac{1}{2\eta_x}+L_{\Phi}+2\alpha+2\beta\Big) \epsilon'^2, \label{eq: grad_bound_general}
\end{align}
where (i) uses eq. \eqref{eq: CRcond1}, (ii) uses eqs. \eqref{eq: grad_goal_noKL} \& \eqref{eq: Hess_goal_noKL} and the item \ref{item: ddPhi} of \Cref{prop_Phiystar} that $\nabla^2\Phi$ is $L_{\Phi}$-Lipschitz, and (iii) uses $\|s_{T'-1}\|\vee \|s_{T'}\|\le\epsilon'$. Also,
\begin{align}
\nabla^2 \Phi(x_{T'}) &\overset{(i)}{\succeq}  G(x_{T'-1},y_{T'})-\|G(x_{T'-1},y_{T'})-\nabla^2 \Phi(x_{T'})\|I \nonumber\\
&\overset{(ii)}{\succeq} -\frac{1}{2\eta_x}\|s_{T'}\|I -\|G(x_{T'-1},y_{T'})-\nabla^2 \Phi(x_{T'-1})\|I -\|\nabla^2 \Phi(x_{T'})-\nabla^2 \Phi(x_{T'-1})\|I \nonumber\\
&\overset{(iii)}{\succeq} -\Big(\frac{1}{2\eta_x}+L_{\Phi}\Big)\|s_{T'}\|I-\alpha(\|s_{T'-1}\|+\epsilon')I \nonumber\\
&\overset{(iv)}{\succeq} -\Big(\frac{1}{2\eta_x}+L_{\Phi}+2\alpha\Big)\epsilon' I, \label{eq: Hess_bound_general}
\end{align}
where (i) uses Weyl's inequality, (ii) uses eq. \eqref{eq: CRcond2}, (iii) uses eq. \eqref{eq: Hess_goal_noKL} and the item \ref{item: ddPhi} of \Cref{prop_Phiystar} that $\nabla^2\Phi$ is $L_{\Phi}$-Lipschitz, and (iv) uses $\|s_{T'-1}\|\vee \|s_{T'}\|\le\epsilon'$. 
\end{proof}

\iffalse
\begin{restatable}{lemma}{lemmaNtnoKL}\label{lemma_Nt_noKL}
Run Algorithm \ref{algo: prox-minimax} with hyperparameter choices $\epsilon'\le \frac{\alpha L_1}{\beta L_G}$ and $\eta_{y}=\frac{2}{L+\mu}$ and sufficiently large number of inner iterations $N_t$ as follows, then the conditions \eqref{eq: grad_goal_noKL} \& \eqref{eq: Hess_goal_noKL} hold and thus eq. \eqref{eq: Hdec2_noKL} holds. 
\begin{align}
    \left\{ \begin{gathered}
    N_0\ge 2\kappa\ln\big(L_1\|y_0-y^*(x_0)\|/(2\beta\epsilon'^2)\big)\hfill\\
    N_t\ge \kappa\ln\Big(\frac{2L_1\alpha\|s_{t-1}\|+L_1(\alpha+L_G\kappa)\|s_t\|}{L_G\beta\epsilon'^2}\Big); t\ge 1.\\
    \end{gathered}  \right. \label{Nt_noKL}
\end{align}
\end{restatable}
\begin{proof}
    We first bound the term $\|y_{t+1}-y^*(x_t)\|$, which corresponds to the optimality gap of the maximization problem. Note that $y^*(x_t)\in \mathbb{R}^n$ is the unique maximizer of the strongly concave function $f(x_t,y)$. 
    Note that $y_{t+1}$ is obtained by applying $N_t$ gradient ascent steps starting from $y_t$. Hence, by the convergence rate of gradient ascent algorithm under strong concavity, we conclude that with learning rate $\eta_{y}=\frac{2}{L+\mu}$,
    \begin{align}
    	\|y_{t+1} - y^*(x_{t}) \| \le&  (1-\kappa^{-1})^{N_t}\|y_{t} - y^*(x_{t})\| \label{eq: 8}
    \end{align}
    
    We will prove by induction that for any $t\ge 0$,
	\begin{align}
    \|y_{t+1}-y^*(x_t)\|\le& \min\Big(\frac{\alpha(\|s_t\|+\epsilon')}{L_G},\frac{\beta(\|s_t\|^2+\epsilon'^2)}{L_1}\Big). \label{eq: yerr_t}
    \end{align}

    %We consider the following three cases.
    
    %(Case 1) 
    When $t=0$, on one hand, eq. \eqref{eq: 8} implies that
    \begin{align}
        \|y_1-y^*(x_t)\|&\le \|y_0-y^*(x_0)\|\exp\big(N_0\ln(1-\kappa^{-1})\big) \nonumber\\
        &\overset{(i)}{\le} \|y_0-y^*(x_0)\|\exp\Big(-\ln\Big(\frac{L_1\|y_0-y^*(x_0)\|}{2\beta\epsilon'^2}\Big)\Big) \le \frac{2\beta\epsilon'^2}{L_1} \label{eq: yerr_0a}
    \end{align}
    where (i) uses $\ln(1-x)\le -x<0$ for $x=\kappa^{-1}\in(0,1)$ and $N_0\ge 2\kappa\ln\big(L_1\|y_0-y^*(x_0)\|/(2\beta\epsilon'^2)\big)$. 
    
    On the other hand, the right side of eq. \eqref{eq: yerr_t} is simplified as follows. 
    \begin{align}
        \min\Big(\frac{\alpha(\|s_0\|+\epsilon')}{L_G},\frac{\beta(\|s_0\|^2+\epsilon'^2)}{L_1}\Big) \overset{(i)}{=}  \min\Big(\frac{2\alpha\epsilon'}{L_G},\frac{2\beta\epsilon'^2}{L_1}\Big)\overset{(ii)}{=} \frac{2\beta\epsilon'^2}{L_1} \label{eq: yerr_0b}
    \end{align}
    where (i) uses $\|s_0\|=\epsilon'$ and (ii) uses $\epsilon'\le \frac{\alpha L_1}{\beta L_G}$. Hence, eqs. \eqref{eq: yerr_0a}\&\eqref{eq: yerr_0b} imply that the error bound \eqref{eq: yerr_t} holds for $t=0$.
    
    %(Case 2) 
    Suppose the error bound \eqref{eq: yerr_t} holds for $t=k-1$. Then, on one hand, eq. \eqref{eq: 8} implies that
    \begin{align}
        &\|y_{k+1} - y^*(x_{k}) \| \nonumber\\
        &\le  (1-\kappa^{-1})^{N_k}\|y_{k} - y^*(x_{k})\| \nonumber\\
        &\le  (1-\kappa^{-1})^{N_k}\|y_{k} - y^*(x_{k-1})\| + (1-\kappa^{-1})^{N_k}\|y^*(x_{k-1}) - y^*(x_{k})\| \nonumber\\
        &\overset{(i)}{\le} \exp\big(N_k\ln(1-\kappa^{-1})\big) \Big(\min\Big(\frac{\alpha(\|s_{k-1}\|+\epsilon')}{L_G},\frac{\beta(\|s_{k-1}\|^2+\epsilon'^2)}{L_1}\Big)+\kappa\|s_k\|\Big) \nonumber\\
        &\overset{(ii)}{\le} \exp\Big(-\ln\Big(\frac{2L_1\alpha\|s_{k-1}\|+L_1(\alpha+L_G\kappa)\|s_k\|}{L_G\beta\epsilon'^2}\Big)\Big) \Big(\frac{\alpha(\|s_{k-1}\|+\epsilon')}{L_G} + \kappa\|s_k\|\Big) \nonumber\\
        &= \frac{L_G\beta\epsilon'^2}{2L_1\alpha\|s_{k-1}\|+L_1(\alpha+L_G\kappa)\|s_k\|} \frac{\alpha(2\|s_{k-1}\|+\|s_k\|)+L_G\kappa\|s_k\|}{L_G} =\frac{\beta\epsilon'^2}{L_1} \label{eq: yerr_1a}
    \end{align}
    where (i) uses eq. \eqref{eq: yerr_t} for $t=k-1$ and the fact that $y^*$ is $\kappa$-Lipschitz mapping (see \cite{lin2019gradient,chen2021proximal} for the proof), (ii) uses $\ln(1-\kappa^{-1})\le -\kappa^{-1}$, $N_k\ge \kappa\ln\Big(\frac{2L_1\alpha\|s_{k-1}\|+L_1(\alpha+L_G\kappa)\|s_k\|}{L_G\beta\epsilon'^2}\Big)$ and $\epsilon'\le \|s_{k-1}\|\vee\|s_k\|\le \|s_{k-1}\|+\|s_k\|$. 
    On the other hand, the right side of eq. \eqref{eq: yerr_t} for $t=k\in [1, T'-1]$ can be lower bounded as follows.
    \begin{align}
        \min\Big(\frac{\alpha(\|s_k\|+\epsilon')}{L_G},\frac{\beta(\|s_k\|^2+\epsilon'^2)}{L_1}\Big)\ge \min\Big(\frac{\alpha\epsilon'}{L_G},\frac{\beta\epsilon'^2}{L_1}\Big) \overset{(i)}{=} \frac{\beta\epsilon'^2}{L_1} \label{eq: yerr_1b}
    \end{align}
    where (i) uses $\epsilon'\le \frac{\alpha L_1}{\beta L_G}$. Combining eqs. \eqref{eq: yerr_1a} \& \eqref{eq: yerr_1b} proves \eqref{eq: yerr_t} for $t=k$. Hence, eq. \eqref{eq: yerr_t} holds for all $t\ge 0$.
\end{proof}

\begin{restatable}{lemma}{lemmaNtKL}\label{lemma_Nt_KL}
Run Algorithm \ref{algo: prox-minimax} with hyperparameters $\epsilon'\le \frac{\alpha L_1}{\beta L_G}$ and sufficiently large number of inner iterations $N_t$ as follows, then the conditions \eqref{eq: grad_goal_KL} \& \eqref{eq: Hess_goal_KL} hold and thus eq. \eqref{eq: Hdec2_KL} holds. 
\begin{align}
    N_t\ge \frac{4\kappa}{3}\ln t+\kappa\ln\Big(\frac{L_1\alpha\|s_{t-1}\|+t^{-4/3}L_1\alpha\epsilon'+L_1L_G\kappa\|s_t\|}{L_G\beta\epsilon'^2}\Big) \label{Nt_KL}
\end{align}
\end{restatable}

\begin{proof}
    The proof of logic is similar to that of Lemma \ref{lemma_Nt_noKL}. We will prove by induction that for any $t\ge 0$,
	\begin{align}
    \|y_{t+1}-y^*(x_t)\|\le& \min\Big(\frac{\alpha(\|s_t\|+\epsilon')}{L_G},\frac{\beta(\|s_t\|^2+\epsilon'^2)}{L_1}\Big). \label{eq: yerr_t}
    \end{align}

    Suppose the error bound \eqref{eq: yerr_t} holds for $t=k-1\ge T'-1$. Then, on one hand, similar to the derivation of eq. \eqref{eq: yerr_1a}, eq. \eqref{eq: 8} implies that
    \begin{align}
        &\|y_{k+1} - y^*(x_{k}) \| \nonumber\\
        &\le (1-\kappa^{-1})^{N_k}\|y_{k} - y^*(x_{k-1})\| + (1-\kappa^{-1})^{N_k}\|y^*(x_{k-1}) - y^*(x_{k})\| \nonumber\\
        &\overset{(i)}{\le} \exp\big(N_k\ln(1-\kappa^{-1})\big) \Big(\min\Big(\frac{\alpha(\|s_{k-1}\|+t^{-2/3}\epsilon')}{L_G},\frac{\beta(\|s_{k-1}\|^2+t^{-4/3}\epsilon'^2)}{L_1}\Big)+\kappa\|s_k\|\Big) \nonumber\\
        &\overset{(ii)}{\le} \exp\Big(-\frac{4}{3}\ln t-\ln\Big(\frac{L_1\alpha\|s_{k-1}\|+t^{-4/3}L_1\alpha\epsilon'+L_1L_G\kappa\|s_k\|}{L_G\beta\epsilon'^2}\Big)\Big)  \frac{\alpha(\|s_{k-1}\|+t^{-2/3}\epsilon')+L_G\kappa\|s_k\|}{L_G} \nonumber\\
        &= \frac{t^{-4/3}L_G\beta\epsilon'^2}{L_1\alpha\|s_{k-1}\|+t^{-4/3}L_1\alpha\epsilon'+L_1L_G\kappa\|s_k\|}  \frac{\alpha(\|s_{k-1}\|+t^{-2/3}\epsilon')+L_G\kappa\|s_k\|}{L_G}\nonumber\\ &\le\frac{\beta\epsilon'^2}{L_1t^{4/3}} \label{eq: yerr_2a}
    \end{align}
    where (i) uses eq. \eqref{eq: yerr_t} for $t=k-1$ and the fact that $y^*$ is $\kappa$-Lipschitz mapping (see \cite{lin2019gradient,chen2021proximal} for the proof), (ii) uses $\ln(1-\kappa^{-1})\le -\kappa^{-1}$, $N_k\ge \frac{4\kappa}{3}\ln k+\kappa\ln\Big(\frac{L_1\alpha\|s_{k-1}\|+k^{-4/3}L_1\alpha\epsilon'+L_1L_G\kappa\|s_k\|}{L_G\beta\epsilon'^2}\Big)$, (iii) uses $4a^3+4b^3\ge (a+b)^3; \forall a,b\ge 0$. 
    
    On the other hand, the right side of eq. \eqref{eq: yerr_t} for $t=k\in [1, T'-1]$ can be lower bounded as follows.
    \begin{align}
        &\min\Big(\frac{\alpha(\|s_k\|+2^{-\max(0,k-T'-1)/3}\epsilon')}{L_G},\frac{\beta(\|s_k\|^2+2^{-2\max(0,k-T'-1)/3}\epsilon'^2)}{L_1}\Big) \nonumber\\
        &\ge \min\Big(\frac{t^{-2/3}\alpha\epsilon'}{L_G},\frac{2^{-2(k-T'-1)/3}\beta\epsilon'^2}{L_1}\Big) \overset{(i)}{=} \frac{2^{-2(k-T'-1)/3}\beta\epsilon'^2}{L_1} \label{eq: yerr_2b}
    \end{align}
    where (i) uses $\epsilon'\le \frac{\alpha L_1}{\beta L_G}$. Combining eqs. \eqref{eq: yerr_1a} \& \eqref{eq: yerr_1b} proves \eqref{eq: yerr_t} for $t=k\ge T'$.
    
    Combining the above 3 cases proves eq. \eqref{eq: yerr_t} for all $t\ge 0$. As a result, eqs. \eqref{eq: grad_goal} \& \eqref{eq: Hess_goal} can be proved as follows.
    \begin{align}
    \|\nabla\Phi(x_t)-\nabla_1 f(x_t, y_{t+1})\|&=\|\nabla_1 f(x_t,y^*(x_t))-\nabla_1 f(x_t, y_{t+1})\|\nonumber\\
    &\le L_1\|y_{t+1}-y^*(x_t)\|\nonumber\\
    &\le\beta(\|s_t\|^2+2^{-2\max(0,t-T'-1)/3}\epsilon'^2),\nonumber
    \end{align}
    \begin{align}
    \|\nabla^2\Phi(x_t)-G(x_t,y_{t+1})\|&=\|G(x_t,y^*(x_t))-G(x_t, y_{t+1})\|\nonumber\\
    &\le L_G\|y_{t+1}-y^*(x_t)\|\nonumber\\
    &\le\alpha(\|s_t\|+2^{-\max(0,t-T'-1)/3}\epsilon').
    \end{align}
\end{proof}
\fi
    
For the stochastic minimax optimization problem (Q) in Section \ref{sec: stoc}, we prove the following supporting lemma on the error of the stochastic estimators.
\lemmaBatch*
\begin{proof}
    Based on Lemmas 6 \& 8 in \cite{kohler2017}, we obtain that with probability at least $1-\delta$, the following bounds hold. (We replaced $\delta$ in \cite{kohler2017} with $\delta/5$ by applying union bound to the following 5 events.)
    \begin{align}
        &\|\widehat{\nabla}_1 f(x,y)-\nabla_1 f(x,y)\|\le 4\sqrt{2}L_0 \sqrt{\frac{\ln(10m/\delta)+1/4}{|B_1|}} \le \epsilon_1,\\ 
        &\|\widehat{\nabla}_{k,\ell}^2 f(x,y)-\nabla_{k,\ell}^2 f(x,y)\|\le 4L_1\sqrt{\frac{\ln\big(10(m\vee n)/\delta\big)}{|B_{k,\ell}|}} \le \epsilon_2; k,\ell\in\{1,2\}.
    \end{align}
    Note that here we only consider the cases that $|B_1|,|B_{k,\ell}|<N$ for all $k,\ell\in\{1,2\}$. Otherwise, $|B_1|=N$ yields $\|\widehat{\nabla}_1 f(x,y)-\nabla_1 f(x,y)\|=0<\epsilon_1$ and $|B_{k,\ell}|=N$ yields $\|\widehat{\nabla}_{k,\ell}^2 f(x,y)-\nabla_{k,\ell}^2 f(x,y)\|=0<\epsilon_2$. Hence, in both cases, the above high probability bounds hold, which further implies eq. \eqref{eq: stoc_err3} following the argument below.
        \begin{align}
        \|\widehat{G}(x,y)-G(x,y)\|&\le \|\widehat{\nabla}_{11} f(x,y)-\nabla_{11} f(x,y)\| + \|(\widehat{\nabla}_{12} f (\widehat{\nabla}_{22} f)^{-1} \widehat{\nabla}_{21} f)(x,y) - (\nabla_{12}f (\nabla_{22}f)^{-1} \nabla_{21} f)(x,y)\| \nonumber\\
        &\le \epsilon_2 +\|(\widehat{\nabla}_{12} f-\nabla_{12}f)\big((\widehat{\nabla}_{22} f)^{-1} \widehat{\nabla}_{21} f\big)(x,y)\| \nonumber\\
        &\quad + \|\nabla_{12}f\big((\widehat{\nabla}_{22} f)^{-1}-(\nabla_{22} f)^{-1}\big)\widehat{\nabla}_{21} f(x,y)\| +\|\nabla_{12}f (\nabla_{22}f)^{-1} (\widehat{\nabla}_{21} f-\nabla_{21}f)(x,y)\| \nonumber\\
        &\overset{(i)}{\le} \epsilon_2 + \epsilon_2 \mu^{-1} L_1 + L_1^2\|\nabla_{22}f(x,y)^{-1}\| \|(\nabla_{22}f-\widehat{\nabla}_{22}f)(x,y)\| \|\widehat{\nabla}_{22}f(x,y)^{-1}\| + L_1\mu^{-1}\epsilon_2 \nonumber\\
        &\overset{(ii)}{\le} \epsilon_2+2\kappa\epsilon_2+L_1^2\mu^{-2}\epsilon_2\le (\kappa+1)^2\epsilon_2.
    \end{align}
    where (i) and (ii) use Lemma \ref{lemma_HessBound}.
\end{proof}

Regarding the high-probability convergence rate of the inner stochastic gradient ascent (SGA) in Algorithm \ref{algo: prox-minimax-stoc}, the following result is a direct application of Theorem 3.1 in \cite{harvey2019simple}.

% This assumption implies that the gradients and stochastic gradients are bounded along the SGA trajectories $x_t,\widetilde{y}_k$, which holds if the trajectories are bounded. The above bound 1 can be obtained by properly scaling the objective function $f$. With this assumption, we obtain the following convergence rate of the SGA steps below.



\section{Proof of \Cref{prop_Phiystar}} \label{sec_prop1proof}
\propphy*
\begin{proof}
%The items \ref{item: ystar_lipschitz} \& \ref{item: Phi_Lsmooth} are proved in \cite{chen2021proximal,lin2019gradient}. 
We first prove the item \ref{item: G_lipschitz}.
Consider any $x, x'\in \mathbb{R}^m$ and $y,y'\in\mathbb{R}^n$. For convenience we denote $z=(x,y)$ and $z'=(x',y')$. Then, by \Cref{assum: f} and using the bounds of \Cref{lemma_HessBound}, we have that
\begin{align}
    &\|G(x',y')-G(x,y)\|\nonumber\\
    &\le \|\nabla_{11} f(x',y')-\nabla_{11} f(x,y)\| + \|\nabla_{12} f(x',y')-\nabla_{12} f(x,y)\| \|[\nabla_{22}f(x',y')]^{-1}\| \|\nabla_{21}f(x',y')\| \nonumber\\
    &\quad +\|\nabla_{12} f(x,y)\| \|[\nabla_{22}f(x',y')]^{-1}-[\nabla_{22}f(x,y)]^{-1}\| \|\nabla_{21}f(x',y')\| \nonumber\\ 
    &\quad +\|\nabla_{12} f(x,y)\| \|[\nabla_{22}f(x,y)^{-1}]\| \|\nabla_{21}f(x',y')-\nabla_{21}f(x,y)\| \nonumber\\
    &\le L_2\|z'-z\| + (L_2\|z'-z\|)\mu^{-1}L_1 \nonumber\\
    &\quad + L_1^2 \|[\nabla_{22}f(x',y')]^{-1}\| \|\nabla_{22}f(x,y)-\nabla_{22}f(x',y')\| \|[\nabla_{22}f(x,y)]^{-1}\| +L_1\mu^{-1}(L_2\|z'-z\|) \nonumber\\
    &\le L_2(1+2\kappa) \|z'-z\| + L_1^2\mu^{-1}(L_2\|z'-z\|)\mu^{-1} \nonumber\\
    &\le L_2(1+\kappa)^2\|z'-z\|. \nonumber
\end{align}

Next, we prove the item \ref{item: ddPhi}. Consider any fixed $x\in\mathbb{R}^m$, we know that $f(x,\cdot)$ achieves its maximum at $y^*(x)$, where the gradient vanishes, i.e., $\nabla_2 f(x,y^*(x))=\zero$. Thus, we further obtain that 
\begin{align}
    &\zero=\nabla_x \nabla_2 f(x,y^*(x))=\nabla_{21} f(x,y^*(x))+\nabla_{22} f(x,y^*(x))\nabla y^*(x), \nonumber
\end{align}
which implies that 
\begin{align}
    \nabla y^*(x)=-[\nabla_{22}f(x,y^*(x))]^{-1}\nabla_{21}f(x,y^*(x)). \label{eq: ystar_grad}
\end{align}

With the above equation, we take derivative of $\nabla \Phi(x)=\nabla_1 f(x,y^*(x))$ and obtain that
\begin{align}
    \nabla^2 \Phi(x) =& \nabla_{11} f(x,y^*(x)) + \nabla_{12} f(x,y^*(x)) \nabla y^*(x)\nonumber\\
    =& \nabla_{11} f(x,y^*(x)) - \nabla_{12} f(x,y^*(x)) [\nabla_{22}f(x,y^*(x))]^{-1}\nabla_{21}f(x,y^*(x))\\\nonumber
    =& G(x, y^*(x)). \nonumber
\end{align}
Moreover, we have that
\begin{align}
    \|\nabla^2 \Phi(x')-\nabla^2 \Phi(x)\|=& \|G(x',y^*(x'))-G(x,y^*(x))\| \nonumber\\
    \le& L_G \big[\|x'-x\|+\|y^*(x')-y^*(x)\|\big] \nonumber\\
    \le& L_G(1+\kappa) \|x'-x\|,
\end{align}
where the last step uses the item \ref{item: ystar_lipschitz} of \Cref{prop_1}. This proves the item \ref{item: ddPhi}. 

%Finally, we will prove the item \ref{item: H_Lsmooth}, i.e., the following partial gradients of function $H(x,x',y)$ is $L_H$-Lipschitz.
%\begin{align}
%    \nabla_1 H(x,x',y)=\nabla \Phi(x) + \frac{2L}{3}\|\|
%\end{align}

\end{proof}


==> proposition2proof.tex <==
\section{Proof of \Cref{prop: lyapunov}} \label{sec_prop2proof}

\proplya*

\begin{proof}
    The required number of inner gradient ascent steps for Output I is shown below. 
    \begin{align}
    \left\{ \begin{gathered}
        N_0\!\ge\! \kappa\ln\Big(\frac{\|y_0-y^*(x_0)\|}{(\alpha\|s_0\|/L_G)\wedge(\beta\|s_0\|^2/L_1)}\Big), \hfill \\
        N_t\!\ge\! \kappa \ln\frac{(\alpha\|s_{k-1}\|/L_G)\wedge (\beta\|s_{k-1}\|^2/L_1)+\kappa\|s_k\|}{(\alpha\|s_k\|/L_G)\wedge(\beta\|s_k\|^2/L_1)}; t\ge 1 \hfill 
    \end{gathered}  \right.. \label{eq: Nt1}
    \end{align}
    
    To prove eq. \eqref{eq: potential} for Output I, we first prove by induction that for any $t\ge 0$,
	\begin{align}
    \|y_{t+1}-y^*(x_t)\|\le& \min\Big(\frac{\alpha\|s_t\|}{L_G},\frac{\beta\|s_t\|^2}{L_1}\Big). \label{eq: yerr_t1}
    \end{align}

    Note that $y_{t+1}$ is obtained by applying $N_t$ gradient ascent steps starting from $y_t$. Hence, by the convergence rate of gradient ascent algorithm under strong concavity, we conclude that with learning rate $\eta_{y}=\frac{2}{L+\mu}$,
    \begin{align}
    	\|y_{t+1} - y^*(x_{t}) \| \le&  (1-\kappa^{-1})^{N_t}\|y_{t} - y^*(x_{t})\|. \label{eq: 8}
    \end{align}

    When $t=0$, eq. \eqref{eq: 8} implies that
    \begin{align}
        \|y_1-y^*(x_0)\|&\le \|y_0-y^*(x_0)\|\exp\big(N_0\ln(1-\kappa^{-1})\big) \nonumber\\
        &\overset{(i)}{\le} \|y_0-y^*(x_0)\|\exp\Big(-\ln\Big(\frac{\|y_0-y^*(x_0)\|}{\min\big(\alpha\|s_0\|/L_G,\beta\|s_0\|^2/L_1\big)}\Big)\Big) \le \min\Big(\frac{\alpha\|s_0\|}{L_G},\frac{\beta\|s_0\|^2}{L_1}\Big) \label{eq: yerr_0}
    \end{align}
    where (i) uses $\ln(1-x)\le -x<0$ for $x=\kappa^{-1}\in(0,1)$ and eq. \eqref{eq: Nt1}. Hence, eq. \eqref{eq: yerr_t1} holds for Output I when $t=0$.
        
    Suppose eq. \eqref{eq: yerr_t1} holds for $t=k-1$. Then, eq. \eqref{eq: 8} implies that
    \begin{align}
        &\|y_{k+1} - y^*(x_{k}) \| \nonumber\\
        &\le (1-\kappa^{-1})^{N_k}\|y_{k} - y^*(x_{k-1})\| + (1-\kappa^{-1})^{N_k}\|y^*(x_{k-1}) - y^*(x_{k})\| \nonumber\\
        &\overset{(i)}{\le} \exp\big(N_k\ln(1-\kappa^{-1})\big) \Big(\min\Big(\frac{\alpha\|s_{k-1}\|}{L_G},\frac{\beta\|s_{k-1}\|^2}{L_1}\Big)+\kappa\|s_k\|\Big) \nonumber\\
        &\overset{(ii)}{\le} \exp\Big(-\ln\frac{(\alpha\|s_{k-1}\|/L_G)\wedge (\beta\|s_{k-1}\|^2/L_1)+\kappa\|s_k\|}{(\alpha\|s_k\|/L_G)\wedge(\beta\|s_k\|^2/L_1)}\Big) \Big(\Big(\frac{\alpha\|s_{k-1}\|}{L_G}\wedge\frac{\beta\|s_{k-1}\|^2}{L_1}\Big)+\kappa\|s_k\|\Big) \nonumber\\
        &=\frac{\alpha\|s_k\|}{L_G} \wedge \frac{\beta\|s_k\|^2}{L_1}\label{eq: yerr_1a}
    \end{align}
    where (i) uses eq. \eqref{eq: yerr_t1} for $t=k-1$ and the fact that $y^*$ is $\kappa$-Lipschitz mapping (see \cite{lin2019gradient,chen2021proximal} for the proof) and (ii) uses $\ln(1-\kappa^{-1})\le -\kappa^{-1}$ and eq. \eqref{eq: Nt1}. Therefore, eq. \eqref{eq: yerr_t1} holds for $t=k$ and thus for all $t\in [0,T-1]$.
    
    Hence, eqs. \eqref{eq: grad_goal_noKL} \& \eqref{eq: Hess_goal_noKL} with $\epsilon'=0$ in Lemma \ref{lemma_ifErrSmall_noKL} can be proved as follows.
    \begin{align}
    \|\nabla\Phi(x_t)-\nabla_1 f(x_t, y_{t+1})\|&=\|\nabla_1 f(x_t,y^*(x_t))-\nabla_1 f(x_t, y_{t+1})\| \le L_1\|y_{t+1}-y^*(x_t)\| \le \beta\|s_t\|^2,\label{eq: dfKL}
    \end{align}
    \begin{align}
    \|\nabla^2\Phi(x_t)-G(x_t,y_{t+1})\|&=\|G(x_t,y^*(x_t))-G(x_t, y_{t+1})\| \le L_G\|y_{t+1}-y^*(x_t)\| \le\alpha\|s_t\|.\label{eq: dGKL}
    \end{align}
    Note that $\epsilon'=0$ implies that $T'=+\infty$, so eq. \eqref{eq: Hdec2_noKL} in Lemma \ref{lemma_ifErrSmall_noKL} holds for all $t\ge 0$. Therefore, eq. \eqref{eq: potential} holds for Output I of Algorithm \ref{algo: prox-minimax}. 
    
    The proof for Output II follows the same logic as that for Output I. The major difference is that the lower bound of $N_t$ changes as follows. 
    \begin{align}
        \left\{ \begin{gathered}
        N_0\ge \kappa\ln\big(L_1\|y_0-y^*(x_0)\|/(2\beta\epsilon'^2)\big)\hfill\\
	    N_t\ge \kappa\ln\Big(\frac{2L_1\alpha\|s_{t-1}\|+L_1(\alpha+L_G\kappa)\|s_t\|}{L_G\beta\epsilon'^2}\Big)=\mathcal{O}\Big(\kappa\ln \frac{L_1\alpha \|s_{t-1}\|+ L_1(\alpha+L_2\kappa)\|s_t\|}{L_G\beta\epsilon'^2}\Big); 1\le t\le T'.\\
	    \end{gathered}  \right., \label{eq: Nt2}
    \end{align}
    which by a similar induction argument yields that
	\begin{align}
    \|y_{t+1}-y^*(x_t)\|\le& \frac{\alpha(\|s_t\|+\epsilon')}{L_G}\wedge\frac{\beta(\|s_t\|^2+\epsilon'^2)}{L_1}; 0\le t\le T'-1. \label{eq: yerr_t2}
    \end{align}
    We briefly sketch the induction here. 
    
    When $t=0$, on one hand, eq. \eqref{eq: 8} implies that
    \begin{align}
        \|y_1-y^*(x_0)\|&\le \|y_0-y^*(x_0)\|\exp\big(N_0\ln(1-\kappa^{-1})\big) \nonumber\\
        &\overset{(i)}{\le} \|y_0-y^*(x_0)\|\exp\Big(-\ln\Big(\frac{L_1\|y_0-y^*(x_0)\|}{2\beta\epsilon'^2}\Big)\Big) \le \frac{2\beta\epsilon'^2}{L_1} \label{eq: yerr_0}
    \end{align}
    where (i) uses $\ln(1-x)\le -x<0$ for $x=\kappa^{-1}\in(0,1)$ and eq. \eqref{eq: Nt2}. On the other hand, the right side of eq. \eqref{eq: yerr_t2} is simplified as follows. 
    \begin{align}
        \frac{\alpha(\|s_0\|+\epsilon')}{L_G}\wedge\frac{\beta(\|s_0\|^2+\epsilon'^2)}{L_1} \overset{(i)}{=}  \frac{2\alpha\epsilon'}{L_G}\wedge\frac{2\beta\epsilon'^2}{L_1}\overset{(ii)}{=} \frac{2\beta\epsilon'^2}{L_1}, \label{eq: yerr_0b}
    \end{align}
    where (i) uses the definition $\|s_0\| = \epsilon'$ and (ii) uses the condition that $\epsilon'\le \frac{\alpha L_1}{\beta L_G}$.
    Hence, eq. \eqref{eq: yerr_t2} holds for Output I when $t=0$.
    
    If eq. \eqref{eq: yerr_t2} holds for $t=k-1\in[0,T'-2]$, then
    \begin{align}
        &\|y_{k+1} - y^*(x_{k}) \| \nonumber\\
        &\le  (1-\kappa^{-1})^{N_k}\|y_{k} - y^*(x_{k-1})\| + (1-\kappa^{-1})^{N_k}\|y^*(x_{k-1}) - y^*(x_{k})\| \nonumber\\
        &\overset{(i)}{\le} \exp\big(N_k\ln(1-\kappa^{-1})\big) \Big(\Big(\frac{\alpha(\|s_{k-1}\|+\epsilon')}{L_G}\wedge\frac{\beta(\|s_{k-1}\|^2+\epsilon'^2)}{L_1}\Big)+\kappa\|s_k\|\Big) \nonumber\\
        &\overset{(ii)}{\le} \exp\Big(-\ln\Big(\frac{2L_1\alpha\|s_{k-1}\|+L_1(\alpha+L_G\kappa)\|s_k\|}{L_G\beta\epsilon'^2}\Big)\Big) \Big(\frac{\alpha(\|s_{k-1}\|+\epsilon')}{L_G} + \kappa\|s_k\|\Big) \nonumber\\
        &\overset{(iii)}{\le}\frac{L_G\beta\epsilon'^2}{2L_1\alpha\|s_{k-1}\|+L_1(\alpha+L_G\kappa)\|s_k\|} \frac{\alpha(2\|s_{k-1}\|+\|s_k\|)+L_G\kappa\|s_k\|}{L_G}\nonumber\\ &=\frac{\beta\epsilon'^2}{L_1}\overset{(iv)}{=}\frac{\alpha\epsilon'}{L_G}\wedge\frac{\beta\epsilon'^2}{L_1}\le \frac{\alpha(\|s_k\|+\epsilon')}{L_G}\wedge\frac{\beta(\|s_k\|^2+\epsilon'^2)}{L_1} \nonumber
    \end{align}
    where (i) uses eq. \eqref{eq: yerr_t2} for $t=k-1$ and the fact that $y^*$ is $\kappa$-Lipschitz mapping (see \cite{lin2019gradient,chen2021proximal} for the proof), (ii) uses $\ln(1-\kappa^{-1})\le -\kappa^{-1}$ and eq. \eqref{eq: Nt2}, (iii) uses $\epsilon'\le \|s_{k-1}\|\vee\|s_k\|\le \|s_{k-1}\|+\|s_k\|$ for $k\le T'-1$, and (iv) uses the condition that $\epsilon'\le \frac{\alpha L_1}{\beta L_G}$. This proves eq. \eqref{eq: yerr_t2} holds for $t=k$ and thus for all $t\in[0,T'-1]$, which further implies eqs. \eqref{eq: grad_goal_noKL} \& \eqref{eq: Hess_goal_noKL}. Hence, by Lemma \ref{lemma_ifErrSmall_noKL}, we prove that eq. \eqref{eq: potential} holds for output II for all $0\le t\le T'-1$. 
\end{proof}



==> remove.tex <==
\section{Two Objective Functions (to remove)}
\begin{align}
    L(s,v):=&\nabla_{\!1}f(x_t,\! y_{t+1})^{\!\top}\!s +  \zeta_{x_t,y_{t+1}}(s,v)+\frac{1}{6\eta_x}\|s\|^3 \label{eq:inexact_CRobj}\\
    L^*(s):=&L(s,v^*(s))=\nabla_{\!1}f(x_t,\! y_{t+1})^{\!\top}\!s + \frac{1}{2} s^{\!\top}G(\!x_t,\! y_{t+1}\!)s+\frac{1}{6\eta_x}\|s\|^3 \label{eq:exact_CRobj}
\end{align}

\section{See GD step in GDA as GD of CR with approximate gradient (to remove)}
Approximate gradient using $v_h\approx v^*(s)$ obtained by $h$ gradient ascent steps:
\begin{align}
    g_h=\nabla_{\!1}f(x_t,\!y_{t+1}) + \nabla_{11}f(x_t,\!y_{t+1}) s + \nabla_{12}f(x_t,\!y_{t+1}) v_h +\frac{1}{2\eta_x}\|s\|s
\end{align}

True gradient (when $v=v^*(s)$ above): 
\begin{align}
	g=\nabla_{\!1}f(x_t,\!y_{t+1}) + G(x_t,\!y_{t+1})s +\frac{1}{2\eta_x}\|s\|s. 
\end{align}

Gradient error bound:
\begin{align}
    \|g_h-g\|&=\|\nabla_{12}f(x_t,\!y_{t+1}) (v_h-v^*(s))\|\nonumber\\
    &\le L(1-\kappa^{-1})^h\|v_0-v^*(s)\|\nonumber\\
    &\overset{(i)}{\le} L\kappa(1-\kappa^{-1})^h\|s\|,\nonumber
\end{align} 
where (i) uses $v_0=0$ and $\|v^*(s)\|=\|\nabla_{22}^{-1}f(x,y) \nabla_{21}f(x,y)s\|\le \kappa\|s\|$. 

The gradient pertrubation is reflected in eq. (8) and the beginning of Lemma A.2 proof in \cite{carmon2019gradient}

Question: 
Axact GD: $O(d^2$) to obtain exact $v^*$
Gradient Descent Efficiently Finds the Cubic-Regularized Non-Convex Newton Step.pdf 
From function value gap to (via eq. (5) with $\rho||s^*||>=\gamma$)

Approximate GD (GDA): $O(\ln(1-1/\kappa))$ to obtain approximate $v^*$. 

keep both? Also GD analysis is the basis of GDA analysis. 

\section{Exact GD (to remove)}
Convergence rate with $K$ GD iterations  (Theorems 3.1 and 3.2 of \cite{carmon2019gradient}):
\begin{align}
    L^*(s_K)-L^*(s^*)\le \widetilde{\mathcal{O}}(1/K). \nonumber
\end{align}
Then if $\frac{\|s^*\|}{2\eta_x}\ge \frac{\epsilon'}{2\eta_x}\ge -2\lambda_{\min}[G(x_t,y_{t+1})]\approx -2\mu$ (as $y_{t+1}\approx y^*(x_t)$), we have
\begin{align}
    L^*(s_K)-L^*(s^*)&=\frac{1}{2}(s_K-s^*)^{\top}\Big(G(x_t,y_{t+1})+\frac{\|s^*\|}{2\eta_x}I\Big)(s_K-s^*) + \frac{1}{12\eta_x}(\|s^*\|-\|s_K\|)^2(\|s^*\|+2\|s_K\|) \nonumber\\
    &\ge -\frac{1}{2}\lambda_{\min}[G(x_t,y_{t+1})]\|s_K-s^*\|^2 \nonumber
\end{align}
Then use $\|s_K-s^*\|\le \widetilde{\mathcal{O}}(K^{-1/2})$ to obtain 3 approximate optimality conditions for $s_K$.

Challenge: What if $\|s^*\|<\epsilon'$ for some outer iteration $t$? 

\section{Stationary point of CR minimax (to remove)}
\begin{align}
&\nabla_{\!1}f(x_t,\!y_{t+1}) + \nabla_{11}f(x_t,\!y_{t+1}) s + \nabla_{12}f(x_t,\!y_{t+1}) v +\frac{1}{2\eta_x}\|s\|s=0 \label{stat1}\\
&\nabla_{21}f(x_t,\!y_{t+1})s + \nabla_{22}f(x_t,\!y_{t+1}) v =0 \label{stat2}
\end{align}
Eq. \eqref{stat2} implies that $v=-\nabla_{22}f(x_t,\!y_{t+1})^{-1}\nabla_{21}f(x_t,\!y_{t+1})s$. Substitute that into eq. \eqref{stat1} yields that
\begin{align}
	\nabla_{\!1}f(x_t,\!y_{t+1}) + \nabla_{11}f(x_t,\!y_{t+1}) s - \nabla_{12}f(x_t,\!y_{t+1})\nabla_{22}f(x_t,\!y_{t+1})^{-1}\nabla_{21}f(x_t,\!y_{t+1})s +\frac{1}{2\eta_x}\|s\|s=0, \nonumber
\end{align}
i.e.,
\begin{align}
	\nabla_{\!1}f(x_t,\!y_{t+1}) + G(x_t,\!y_{t+1})s +\frac{1}{2\eta_x}\|s\|s=0, \nonumber
\end{align}
which is exactly the same as the stationary condition of the CR problem. 

\section{Inexact GD convergence analysis for cubic-regularization subproblem}
% \begin{assum}\label{assum: f}
% 	The minimax problem $\mathrm{(P)}$ satisfies:
% 	\begin{enumerate}[leftmargin=*,topsep=0mm,itemsep=1mm]
% 		\item Function $f(\cdot,\cdot)$ is $L_1$-smooth and function $f(x,\cdot)$ is $\mu$-strongly concave for any fixed $x$;
% 		\item The Jacobian mappings $\nabla_{11} f$, $\nabla_{12} f$, $\nabla_{21} f$, $\nabla_{22} f$ are $L_2$-Lipschitz continuous;
% 		\item Function $\Phi(x):=\max_{y\in \mathbb{R}^n} f(x,y)$ is bounded below and has compact sub-level sets.
% 	\end{enumerate}
% \end{assum} 

Denote 
\begin{align}
    R:=\sqrt{L_1^2L_2^2(1+\kappa)^2+4L_2\|g\|}-L_1L_2(1+\kappa)
\end{align}
\begin{align}
    \|G(x,y)\|\le 2L_1\kappa (=\beta in \cite{carmon2019gradient})
\end{align}

$2\rho$ in \cite{carmon2019gradient} corresponds to our $1/\eta_x$. 

$\text{gap}=\lambda_{\max}(A)-\lambda_{\min}(A)$ in \cite{carmon2019gradient} corresponds to our $\text{gap}\le 4L_1\kappa$. 

$\gamma=-\lambda_{\min}(A)$ in \cite{carmon2019gradient} corresponds to our $|\gamma|\in 2L_1\kappa$. 



\section{Try directly see the perturbation error of the final result (To remove later)}
\begin{align}
    f(s)=b^{\top}s+\frac{1}{2}s^{\top}As+\frac{\rho}{3}\|s\|^3\nonumber
\end{align}
Let $s_0=\widetilde{s}_0$ and stepsize $\eta=\frac{1}{4(\|A\|+\rho R)}$.
\begin{align}
	s_{t+1}=s_t-\eta \nabla f(s_t), \quad \widetilde{s}_{t+1}=\widetilde{s}_t-\eta \big(\nabla f(\widetilde{s}_t)+d_t\big).\nonumber
\end{align}

% \subsection{Find $s_{\max}$ such that $\|\widetilde{s}_t\|\le s_{\max}$}
% Let $0\le s_{\text{in}}\le s_{\max}$ be such that
% \begin{align}
%     &s_{\text{in}}+\eta (\|b\|+\|A\|s_{\text{in}}+\rho s_{\text{in}}^2) \le s_{\max} \nonumber\\
%     &d 
% \end{align}

% \subsection{Proof of convergence rate}
Suppose the $t$-th CR-GD iteration takes $h_t$ maximum steps, then 
\begin{align}
\|d_t\|\le L\kappa(1-\kappa^{-1})^{h_t} s_{\max}. \nonumber
\end{align}

Therefore,
\begin{align}
	&\|\widetilde{s}_1-s_1\|=\eta\|d_0\|.\nonumber	
\end{align}
\begin{align}
	\|\widetilde{s}_{t+1}-s_{t+1}\|&\le \|\widetilde{s}_t-s_t\|+\eta\|\nabla f(s_t)-\nabla f(\widetilde{s}_t)\|+\eta\|-d_t\| \nonumber\\
	&\le (1+\eta L_{CR})\|\widetilde{s}_t-s_t\|+\eta\|d_t\| \nonumber
\end{align}
where $f(s)$ is $L_{CR}:=\|A\|+2\rho s_{\max}$-smooth when $\|s\|\le s_{\max}$. 
\begin{align}
	\|\widetilde{s}_t-s_t\|&\le \eta \sum_{t'=0}^{t-1} (1+\eta L_{CR})^{t-1-t'}\|d_{t'}\|\nonumber\\
	&\le L\kappa\eta s_{\max}\sum_{t'=0}^{t-1} (1+\eta L_{CR})^{t-1-t'}(1-\kappa^{-1})^{h_{t'}}\label{ds_general}
\end{align}
The CR-GD paper proved that
\begin{align}
	f(s_t)-f(s^*)\le \frac{\epsilon}{2} \label{CRGD_eps}
\end{align}
if 
\begin{align}
    t\ge \frac{120\|s^*\|^2}{\eta\epsilon} \ln\Big(\frac{2\|s^*\|^2(\|A\|+2\rho\|s^*\|)}{\epsilon}\Big(1+\frac{\lambda_1^2}{4\rho|b^{\top}q_1|}\Big)\Big):=C\epsilon^{-1}\ln(\epsilon^{-1})\nonumber
\end{align}
where $Aq_j=\lambda_jq_j$ with $\lambda_1\le\ldots\le\lambda_d$ and $\|q_j\|=1$. ($|b^{\top}q_1|\ge \epsilon$ with high probability after uniform perturbation.) 

Based on eq. \eqref{CRGD_eps}, to ensure that $f(\widetilde{s}_t)-f(s^*)\le\epsilon$, we simply need $\|\widetilde{s}_t-s_t\|\le \frac{\epsilon}{2\ell_{CR}}$ where $f(s)$ is $\ell_{CR}:=\|b\|+\|A\|s_{\max}+\rho s_{\max}^2$-Lipschitz when $\|s\|\le s_{\max}$. This combined with eq. \eqref{ds_general} yields the condition that
\begin{align}
    \sum_{t'=0}^{t-1} (1+\eta L_{CR})^{t-1-t'}(1-\kappa^{-1})^{h_{t'}} \le \frac{\epsilon}{2\ell_{CR}L\kappa\eta s_{\max}}. \nonumber
\end{align}
The following choice of $h_t$ satisfies the above.
\begin{align}
    h_{t'}=\Big\lceil \frac{\kappa}{2}\big(\ln(2\ell_{CR}L\kappa\eta s_{\max}\epsilon^{-1})+(t-1-t')\ln(1+\eta L_{CR})\big)\Big\rceil
\end{align}





==> stochastic.tex <==
\section{Sub-Sampled Stochastic Cubic-GDA }\label{sec: stoc}

In this section, we apply stochastic sub-sampling to further improve the performance and complexity of Cubic-GDA in large-scale nonconvex minimax optimization with big data. Specifically, we consider the following stochastic finite-sum minimax optimization problem (Q). 
\begin{align}
	\min_{x\in \mathbb{R}^m}\max_{y\in \mathbb{R}^n}~ f(x,y):= \frac{1}{N}\sum_{i=1}^N f_i(x,y), \tag{Q}
\end{align} 
where $N$ denotes the total number of training samples and $f_i$ corresponds to the loss function on the $i$-th sample. We adopt the following assumptions. 

\begin{assum}\label{assum: fi}
	The stochastic minimax optimization problem $\mathrm{(Q)}$ satisfies:
	\begin{enumerate}[leftmargin=*,topsep=0mm,itemsep=1mm]
		\item For any sample $i$, function $f_i(\cdot,\cdot)$ is $L_1$-smooth, function $f_i(\cdot,y)$ is $L_0$-Lipschitz for any fixed $y$, and function $f_i(x,\cdot)$ is $\mu$-strongly concave for any fixed $x$;
		\item For any sample $i$, the Jacobian mappings $\nabla_{11} f_i$, $\nabla_{12} f_i$, $\nabla_{21} f_i$, $\nabla_{22} f_i$ are $L_2$-Lipschitz continuous;
		\item Function $\Phi(x):=\max_{y\in \mathbb{R}^n} f(x,y)$ is bounded below and has compact sub-level sets.
	\end{enumerate}
\end{assum} 

Applying Cubic-GDA to solve the above problem (Q) would require querying full partial gradients and full Jacobian matrices that involve all the training samples. Instead, it is more efficient to approximate these quantities via stochastic sub-sampling. Therefore, we propose a \textbf{stochastic Cubic-GDA} algorithm, which replaces the exact quantities $\nabla_1 f$ and $G$ involved in the cubic update by their corresponding stochastic approximations. 

Specifically, to approximate the partial gradient $\nabla_1 f$, we sub-sample a mini-batch of samples $B_1$ with replacement from the training set and construct the following sample average approximation. 
\begin{align}
    \widehat{\nabla}_1 f(x,y) &= \frac{1}{|B_1|} \sum_{i \in B_1} \nabla_1 f_i(x,y). \label{eq: stoc_f1}
\end{align}
On the other hand, to approximate the matrix $G$, we sub-sample mini-batches of samples $B_{11}, B_{12}, B_{21}, B_{22}$ with replacement and construct approximated Jacobian matrices $\widehat{\nabla}_{11} f, \widehat{\nabla}_{12} f, \widehat{\nabla}_{21} f, \widehat{\nabla}_{22} f$ in the same way as above. Then, we construct the following approximation of $G$.
\begin{align}
    \widehat{G}(x,y) = \big[\widehat{\nabla}_{11} f - \widehat{\nabla}_{12} f (\widehat{\nabla}_{22}f)^{-1} \widehat{\nabla}_{21} f\big](x,y). \label{eq: stocG}
\end{align}
We summarize the update rule of stochastic Cubic-GDA in \Cref{algo: prox-minimax-stoc} below.
In particular, we run stochastic gradient ascent in the inner iterations to obtain the approximated maximizer $y_{t+1}$, and its high-probability convergence rate has been established in the stochastic optimization literature \citep{harvey2019simple}. 

\begin{algorithm}
	\caption{Stochastic Cubic-GDA}\label{algo: prox-minimax-stoc}
	{\bf Input:} Initialize $x_0,y_0$, learning rates $\eta_{x}$, threshold $\epsilon'$ \\
	{Define $\|s_0\|=\epsilon'$} \\
	\For{ $t=0,1, 2,\ldots, T-1$}{
	    Initialize $\widetilde{y}_0 = y_t$
	    
        \For{$k=0,1, 2,\ldots, N_t-1$}{
            Query a sample $\xi$ to compute $\nabla_2 f_{\xi}(x_t, \widetilde{y}_k)$\\
            $\widetilde{y}_{k+1} = \widetilde{y}_k + \frac{2}{\mu(k+1)} \nabla_2 f_{\xi}(x_t, \widetilde{y}_k)$
        }
        
        Set $y_{t+1} = \sum_{k=0}^{N_t-1}\frac{2k}{N_t(N_t-1)}\widetilde{y}_{k}$
        
        Sample minibatch $B_1(t),B_{11}(t),B_{12}(t),B_{21}(t),B_{22}(t)$ to compute \cref{eq: stoc_f1} and \cref{eq: stocG}. Then, solve the following cubic problem for $s_{t+1}$:
        
        $\mathop{\arg\!\min}_s \!\widehat{\nabla}_{\!1}f(x_t,\! y_{t+1})^{\!\top}\!s + \frac{1}{2} s^{\!\top}\widehat{G}(x_t,\! y_{t+1}\!)s+\frac{1}{6\eta_x}\|s\|^3$
        
        Update $x_{t+1}=x_t+s_{t+1}$
	}
	\textbf{Output:}  $x_{T'},y_{T'}$ with 
	$T'=\min\{t: \|s_{t-1}\|\vee\|s_t\|\le\epsilon'\}$
\end{algorithm}

The following lemma characterizes the sample complexities of all the stochastic approximators for achieving a certain approximation accuracy.


\begin{restatable}{lemma}{lemmaBatch}\label{lemma: batch}
    Fix any $0<\epsilon_1 \le 2L_0$, $0<\epsilon_2{\le 4L_1}$ and choose the following batch sizes
    \begin{align}
    |B_1| &\ge \mathcal{O}\Big(\frac{L_0^2}{\epsilon_1^{2}}\ln\frac{m}{\delta} \Big), \label{eq: b1}\\  
    |B_{11}|,|B_{12}|,|B_{21}|,|B_{22}|&\ge \mathcal{O}\Big(\frac{L_1^2}{\epsilon_2^{2}} \ln\frac{m+n}{\delta}\Big). \label{eq: b2}
    \end{align}
    Then, the stochastic approximators satisfy the following error bounds with probability at least $1-\delta$.
    \begin{align}
        &\|\widehat{\nabla}_1 f(x,y)-\nabla_1 f(x,y)\|\le \epsilon_1,\label{eq: stoc_err1}\\ 
        &\|\widehat{\nabla}_{k\ell}^2 f(x,y) \!-\! \nabla_{k\ell}^2 f(x,y)\|\le \epsilon_2, ~ \forall k,\ell \in \{1,2\},\label{eq: stoc_err2}\\ 
        &\|\widehat{G}(x,y)-G(x,y)\|\le (\kappa+1)^2\epsilon_2.\label{eq: stoc_err3}
    \end{align}
\end{restatable}

Therefore, by choosing proper batch sizes, the inexactness of the stochastic gradient, Jacobian and Hessian estimators can be controlled within a desired range. From this perspective, stochastic Cubic-GDA can be viewed as an inexact version of the Cubic-GDA algorithm. 

To characterize the convergence and sample complexity of stochastic Cubic-GDA, we adopt an adaptive inexactness criterion for the sub-sampling scheme. Specifically, we choose time-varying batch sizes in a way such that the gradient and Jacobian inexactness in iteration $t$ are proportional to the previous increment, i.e., $\epsilon_1(t)\propto \|s_t\|^2, \epsilon_2(t)\propto \|s_t\|$. Such an
adaptive inexact criterion is justified in the cubic regularization literature \citep{wang2018note,wang2019stochastic} with the following advantages: 1) it is adapted to the optimization increment and hence leads to reduced batch sizes when the increment is large in the early iterations; 2) it makes the batch size scheduling scheme in \Cref{lemma: batch} practical, as the batch sizes in iteration $t$ now depend on the increment $\|s_t\|$ obtained in the previous iteration $t-1$. We also note that since the sub-sampling scheme is adapted to the previous increment, the output rule of \Cref{algo: prox-minimax-stoc} is designed to control the value of both the current and the previous increments. This termination rule is critical to bound the adapted gradient and Jacobian inexactness in the analysis. 


We obtain the following global convergence and sample complexity result of stochastic Cubic-GDA.

\begin{restatable}[Convergence and sample complexity]{thm}{thmstoc}\label{thm: 5}
    Let Assumption \ref{assum: fi} and \Cref{lemma: SGA} hold. For $0<\epsilon\le \frac{L_1\sqrt{33L_{\Phi}}}{L_G}$, choose $\epsilon'=\frac{\epsilon}{\sqrt{33L_{\Phi}}}$, $\eta_x\le \frac{1}{55L_{\Phi}}$, $T\ge \frac{\Phi(x_0)-\Phi^*+8L_{\Phi}\epsilon'^2}{3L_{\Phi}\epsilon'^3}$ and $N_t\ge\mathcal{O}\big(\frac{L_0\ln(1/\delta)+L_0^2}{\kappa^{-2}(L_{\Phi}^2\|s_t\|^4+\epsilon^4)\wedge L_1^2(\|s_t\|^2+\epsilon^2/L_{\Phi})}\big)$. Moreover, in iteration $t$, choose the batch sizes according to \cref{eq: b1,eq: b2} with the inexactness given by
    \begin{align}
        \epsilon_1(t)=&\frac{L_{\Phi}}{2}\Big(\|s_t\|^2+\frac{\epsilon^2}{33L_{\Phi}}\Big)\wedge 2L_0, \nonumber\\
        \epsilon_2(t)=&\frac{L_{\Phi}}{2(\kappa+1)^2}\Big(\|s_t\|+\frac{\epsilon}{\sqrt{33L_{\Phi}}}\Big)\wedge 4L_1. \nonumber
\end{align}
    Then, the output of {Stochastic Cubic-GDA} satisfies
    \begin{align}
       \mu(x_{T'}) \le \epsilon. \label{eq: gH_rate2}
    \end{align}
    Consequently, the total number of cubic iterations satisfies $T'\le \mathcal{O}(\sqrt{L_2}\kappa^{1.5}\epsilon^{-3})$, the total number of queried gradient samples satisfies $\sum_{t'=0}^{T'}\big(N_t+|B_1(t)|\big)\le\mathcal{O}\Big(\frac{L_0^2\kappa^{3.5}\sqrt{L_2}}{\epsilon^7}\ln\frac{m}{\delta}\Big)$, and the total number of queried Jacobian samples satisfies  $\sum_{t=0}^{T'-1}\sum_{k=1}^2\sum_{\ell=1}^2|B_{k,\ell}(t)|\le \mathcal{O}\big( \frac{L_1^2\kappa^{2.5}}{\sqrt{L_2}\epsilon^5}\ln\frac{m+n}{\delta}\big)$. 
\end{restatable}
Therefore, under adaptive sub-sampling, the induced gradient and Jacobian inexactness $\epsilon_1(t), \epsilon_2(t)$ are properly controlled so that the iteration complexity $T'$ of stochastic Cubic-GDA remains in the same level as that of Cubic-GDA. Moreover, as opposed to the sample complexity of Cubic-GDA that scales linearly with regard to the data size $N$, the sample complexity of stochastic Cubic-GDA is independent of $N$. For example, by comparing the 
more expensive Jacobian sample complexity between Cubic-GDA and stochastic Cubic-GDA, we conclude that stochastic sub-sampling helps reduce the sample complexity so long as the data size is large enough, i.e., $N\ge \widetilde{\mathcal{O}}\Big(\frac{L_1^2\kappa}{L_2\epsilon^2}\Big)$.

%We compare the above complexity result of stochastic Cubic-GDA with that of Cubic-GDA on the finite-sum minimax optimization problem (Q). Note that Cubic-GDA computes full gradients and Hessians, each of which requires to compute $N$ samples. Therefore, based on Theorem \ref{thm: 1b}, to achieve $\mu(x_{T'}) \le \epsilon$, the total numbers of required gradient and Hessian computations for Cubic-GDA are respectively $N+N\sum_{t=0}^{T'} N_t\le \mathcal{O}(N\sqrt{L_2}\kappa^{2.5}\epsilon^{-3})$ and $4NT'\le \mathcal{O}(N\sqrt{L_2}\kappa^{1.5}\epsilon^{-3})$, which are respectively larger than those required by stochastic Cubic-GDA when the number of training samples is sufficiently large, i.e., $N\ge \widetilde{\mathcal{O}}\Big(\frac{L_0^2\kappa}{\epsilon^4}\vee \frac{L_1^2\kappa}{L_2\epsilon^2}\Big)$. 




==> thm1bproof.tex <==
\section{Proof of Theorem \ref{thm: 1b}}\label{sec: thm2}
\thmglobalrate*

% [to remove] Let \Cref{assum: f} hold. For any $\alpha, \beta>0$, choose $\epsilon'\le \frac{\alpha L_1}{\beta L_G}$, $\eta_x\le (9L_{\Phi}+18\alpha+28\beta)^{-1}$ and $\eta_y\le \frac{2}{L+\mu}$. Then, Outputs I $\&$ II of \Cref{algo: prox-minimax} satisfy the following potential decrease property respectively in the cases listed below.
% \begin{align}
%     H_{t+1}-H_t \le -(L_{\Phi}+\alpha+\beta)(\|s_{t+1}\|^3+\|s_t\|^3). 
% \end{align}
% \begin{itemize}[leftmargin=*,topsep=0mm,itemsep=1mm]
%     \item Output I: choose $N_t \ge \mathcal{O} \big( \kappa\ln \frac{t\alpha\|s_{t-1}\|+t^{1/4}\alpha\epsilon'+ t\kappa\|s_t\|}{\beta\epsilon'^2} \big)$, \red{$T\ge \frac{\Phi(x_0)-\Phi^*+8L_{\Phi}\epsilon'^2}{\epsilon'^3(L_{\Phi}+\alpha+\beta)}$}. Then, for all $0\le t~\le T-1$, \cref{eq: potential}
%     holds with $H_t=\Phi(x_t)+(L_{\Phi}+2\alpha+3\beta)\|s_t\|^2+a_t\epsilon'^3\big(\frac{\alpha}{2}+\beta\big)$, where $a_t = 6\pi^{-2} - \sum_{k=1}^{t-1}k^{-2} \downarrow 0$;
%     \item Output II: choose $N_t\ge \mathcal{O}\big(\kappa\ln \frac{\alpha \|s_{t-1}\|+ (\alpha+\kappa)\|s_t\|}{\beta\epsilon'^2}\big)$. Then, for all $0\le t\le T'-1$, \cref{eq: potential}
%     holds with $H_t:=\Phi(x_t)+(L_{\Phi}+2\alpha+3\beta)\|s_t\|^2$.
% \end{itemize}

\begin{proof}%[Proof of Theorem \ref{thm: 1b}]
Substituting $\alpha=\beta=L_{\Phi}=L_2(1+\kappa)^3$ and $\epsilon'=\frac{\epsilon}{\sqrt{33L_{\Phi}}}$ into Lemma \ref{lemma_general_rate} yields that when $T\ge \sqrt{33L_{\Phi}}\frac{33(\Phi(x_0)-\Phi^*)+8\epsilon^2}{3\epsilon^3}$ and $\eta_x=(55L_{\Phi})^{-1}$, we have $T'\le \sqrt{33L_{\Phi}}\frac{33(\Phi(x_0)-\Phi^*)+8\epsilon^2}{3\epsilon^3}=\mathcal{O}\big(\sqrt{L_2}\kappa^{1.5}\epsilon^{-3}\big)\le T$, and moreover,
\begin{align}
    &\|\nabla \Phi(x_{T'})\| \le \Big(\frac{1}{2\eta_x}+L_{\Phi}+2\alpha+2\beta\Big) \epsilon'^2 \le \epsilon^2, \nonumber\\
    &\lambda_{\min}\big(\nabla^2 \Phi(x_{T'})\big) \ge -\Big(\frac{1}{2\eta_x}+L_{\Phi}+2\alpha\Big)\epsilon' \ge -\sqrt{33L_{\Phi}}\epsilon. \nonumber
\end{align}
This proves eq. \eqref{eq: gH_rate1}. 

Note that the number of gradient ascent iterations $N_t$ should satisfy eq. \eqref{eq: Nt2}. Substituting $\alpha=\beta=L_{\Phi}=L_2(1+\kappa)^3$ and $\epsilon'=\frac{\epsilon}{\sqrt{33L_{\Phi}}}$ into eq. \eqref{eq: Nt2} yields that
\begin{align}
    \left\{ \begin{gathered}
    N_0\ge \kappa\ln\big(L_1\|y_0-y^*(x_0)\|/(2\beta\epsilon'^2)\big) = \kappa\ln\big(33L_1\|y_0-y^*(x_0)\|/(2\epsilon^2)\big) \hfill\\
    N_t\ge \kappa\ln\Big(\frac{2L_1\alpha\|s_{t-1}\|+L_1(\alpha+L_G\kappa)\|s_t\|}{L_G\beta\epsilon'^2}\Big)\overset{(i)}{=}\kappa\ln\Big(\frac{66L_1(1+\kappa)\|s_{t-1}\|+33L_1(2+\kappa)\|s_t\|}{\epsilon^2}\Big); 1\le t\le T'\\
    \end{gathered}  \right., \nonumber
\end{align}
where (i) uses $L_G=L_2(1+\kappa)^2$ and $L_{\Phi}=L_2(1+\kappa)^3$ in \Cref{prop_Phiystar}. 

When we select $N_t$ such that the above holds with equality, then the total number of gradient ascent iterations is upper bounded as follows
\begin{align}
    \sum_{t=0}^{T'-1} N_t&= \kappa\ln\big(33L_1\|y_0-y^*(x_0)\|/(2\epsilon^2)\big) + \kappa\sum_{t=0}^{T'-1} \ln\Big(\frac{66L_1(1+\kappa)\|s_{t-1}\|+33L_1(2+\kappa)\|s_t\|}{\epsilon^2}\Big) \nonumber\\
    &\le \kappa\ln\big(33L_1\|y_0-y^*(x_0)\|/(2\epsilon^2)\big) + \kappa \sum_{t=0}^{T'-1} \ln\big(\|s_{t-1}\|+\|s_t\|\big)  +\kappa T'\ln \big(66L_1\epsilon^{-2}(1+\kappa)\big) \nonumber\\
    &\overset{(i)}{\le} \kappa\ln\big(33L_1\|y_0-y^*(x_0)\|/(2\epsilon^2)\big) + \frac{\kappa T'}{3} \frac{1}{T'}\sum_{t=0}^{T'-1} \ln\big(4\|s_{t-1}\|^3+4\|s_t\|^3\big) +\kappa T'\ln \big(66L_1\epsilon^{-2}(1+\kappa)\big) \nonumber\\
    &\overset{(ii)}{\le} \kappa\ln\big(33L_1\|y_0-y^*(x_0)\|/(2\epsilon^2)\big) + \frac{\kappa T'}{3} \ln\Big(\frac{4}{T'}\sum_{t=0}^{T'-1} \big(\|s_{t-1}\|^3+\|s_t\|^3\big)\Big) +\kappa T'\ln \big(66L_1\epsilon^{-2}(1+\kappa)\big) \nonumber\\
    &\overset{(iii)}{\le} \kappa\ln\big(33L_1\|y_0-y^*(x_0)\|/(2\epsilon^2)\big) + \frac{\kappa T'}{3} \ln\Big(\frac{4(H_0-H^*)}{3L_{\Phi}T'}\Big) +\kappa T'\ln \big(66L_1\epsilon^{-2}(1+\kappa)\big)  \nonumber\\
    &=\widetilde{\mathcal{O}}(\kappa T') \le \widetilde{\mathcal{O}} \big(\sqrt{L_2}\kappa^{2.5}\epsilon^{-3}\big)
\end{align}
where (i) uses $(a+b)^3\le 4(a^3+b^3)$ for any $a,b\ge 0$, (ii) applies Jensen's inequality to the concave function $\ln(\cdot)$, and (iii) telescopes eq. \eqref{eq: potential} over $t=0,1,\ldots,T'-1$.
\end{proof}


==> thm1proof.tex <==
\section{Proof of \Cref{thm: 1}} \label{sec_thm1proof}
\thmconv*

\begin{proof}
    We first prove item \ref{item: Phi_lim}. We have shown in \Cref{prop: lyapunov} that $\{H_t\}_t$ is monotonically decreasing. 
    {Also, \Cref{assum: f} implies that  $H_t=\Phi(x_t)+(L_{\Phi}+2\alpha+3\beta)\|s_t\|^3\ge \Phi^*>-\infty$ for Output I of Algorithm \ref{algo: prox-minimax}. Therefore, we conclude that $\{H_t\}_t$ converges to a finite limit $H^*>-\infty$.}
    
    Telescoping eq. \eqref{prop: lyapunov} over $t=0,1,\ldots,T-1$ yields that 
    \begin{align}
        \sum_{t=0}^{T-1}(\|s_{t+1}\|^3+\|s_t\|^3)\le& \frac{H_0-H_T}{L_{\Phi}+\alpha+\beta} \le \frac{H_0-H^*}{L_{\Phi}+\alpha+\beta} < +\infty, \label{eq: sum_s_cubic}
    \end{align}
    which by letting $T\to +\infty$ yields that $\sum_{t=0}^{\infty}(\|s_{t+1}\|^3+\|s_t\|^3)\le \frac{H_0-H^*}{L_{\Phi}+\alpha+\beta}<+\infty$ and thus $\|s_t\|\to 0$. Therefore
    \begin{align}
        \Phi(x_t)=H_t-(L_{\Phi}+2\alpha+3\beta)\|s_t\|^3 \to H^*.\nonumber
    \end{align}
    This proves item \ref{item: Phi_lim}.
    
    Next, we prove item \ref{item: compact}. Note that $\Phi$ has compact sub-level sets. Moreover, for all $t$, we have
    \begin{align}
        \Phi(x_t)\le H_t\le H_0<+\infty.
    \end{align}
    Hence, the sequence $\{x_t\}_t$ is bounded and thus has a compact set of limit points. Since $y^*$ is Lipschitz continuous by Proposition \ref{prop_Phiystar}, $\{\|y^*(x_t)\|\}_t$ is also bounded. Note that the proof of \Cref{prop: lyapunov} for Output I of Algorithm \ref{algo: prox-minimax} proves eq. \eqref{eq: yerr_t1}, which by $\|s_t\|\to 0$ implies that $\|y_{t+1} - y^*(x_t)\| \to 0$. Therefore, $\|y_{t+1}\|\le \|y^*(x_t)\|+\|y_{t+1} - y^*(x_t)\|$ is also bounded and thus also has a compact set of limit points. This proves item \ref{item: compact}.
    
    Finally, we will prove item \ref{item: 2ndCritical}. Suppose that $x_{t_k}\stackrel{k}{\to} x^*$ along a certain sub-sequence $\{x_{t_k}\}_k$. We have that $y_{t_k+1}\stackrel{k}{\to} y^*(x^*)$ based on \Cref{prop: lyapunov} and the continuity of $y^*$. In addition, \Cref{prop_Phiystar} implies that $\Phi$, $\nabla \Phi$, $\nabla^2 \Phi$ and $G$ are continuous. Therefore, for every limit point $x^*$,
    \begin{align}
        \Phi(x^*) =& \lim_{t_k\to\infty} \Phi(x_{t_k}) = H^* . \nonumber\\
        \|\nabla \Phi(x^*)\| =& \lim_{t_k\to\infty} \|\nabla \Phi(x_{t_k}) \| = \lim_{t_k\to\infty} \|\nabla f(x_{t_k},y^*(x_{t_k})) \|= \lim_{t_k\to\infty} \|\nabla f(x_{t_k},y_{t_k+1}) \| \nonumber\\
        \stackrel{(i)}{=}& \lim_{t_k\to\infty}\Big\|G(x_{t_k}, y_{t_k+1})(s_{t_k+1}) + \frac{1}{2\eta_x}\|s_{t_k+1}\| (s_{t_k+1})\Big\|=0 \nonumber\\
        \lambda_{\min} \big[\nabla^2 \Phi(x^*)\big]=& \lim_{t_k\to\infty} \lambda_{\min} \big[\nabla^2 \Phi(x_{t_k}) \big] = \lim_{t_k\to\infty} \lambda_{\min} \big[G(x_{t_k},y^*(x_{t_k})) \big] \nonumber\\
        =& \lim_{t_k\to\infty} \lambda_{\min} \big[G(x_{t_k},y_{t_k+1})\big] \stackrel{(ii)}{\ge} -\frac{1}{2\eta_x}\lim_{t_k\to\infty}\|s_{t_k+1}\| = 0 \nonumber
    \end{align}
    where (i) uses eq. \eqref{eq: CRcond1}, and (ii) uses eq. \eqref{eq: CRcond2}. Therefore, $x^*$ is a second-order stationary point of $\Phi$. Consequently, $(x^*, y^*(x^*))$ is a local minimax point due to \Cref{coro: 1}. 
    This proves item \ref{item: 2ndCritical}. 
\end{proof}



==> thm2proof.tex <==
\section{Proof of \Cref{thm: 2}} \label{sec_thm2proof}

%\thmvarconv*

\begin{proof}
    For the potential function $H(x,x')=\Phi(x)+(L_{\Phi}+2\alpha+3\beta)\|x'-x\|^2$, we first derive a bound on its gradient $\|\nabla H(x,x')\|=\sqrt{\|\nabla_1 H(x,x')\|^2+\|\nabla_2 H(x,x')\|^2}$ as follows. 
    \begin{align}
        &\|\nabla H(x_t,x_{t-1})\|\nonumber\\
        &\le \|\nabla_1 H(x_t,x_{t-1})\|+\|\nabla_2 H(x_t,x_{t-1})\| \nonumber\\
        &= \Big\|\nabla \Phi(x_t)+2(L_{\Phi}+2\alpha+3\beta)(x_t-x_{t-1}) \Big\| + \Big\|2(L_{\Phi}+2\alpha+3\beta)(x_t-x_{t-1})\Big\|\nonumber\\
        &\le \|\nabla\Phi(x_t)\|+4(L_{\Phi}+2\alpha+3\beta)\|s_t\| \label{eq: 12}
    \end{align}
%    $\nabla_1 f(x_t, y_{t+1})+G(x_t, y_{t+1})(x_{t+1}-x_t) + \frac{\eta_x}{2}\|x_{t+1}-x_t\| (x_{t+1}-x_t) =0$
    where (i) uses eq. (2.2) of \cite{Nesterov2006}, the fact that $\nabla^2\Phi$ is $L_{\Phi}$-Lipschitz, and eq. \eqref{eq: ystar_grad}, (ii) uses Lemma \ref{lemma_HessBound} and $\nabla^2 \Phi(x)=G(x,y^*(x))$ from item 4 of Proposition \ref{prop_Phiystar}, (iii) uses eq. \eqref{eq: stationary}, $\nabla\Phi(x)=\nabla_1 f(x,y^*(x))$ from item 2 of Proposition \ref{prop_Phiystar} and the inequality that $1+\kappa\le 2\kappa$, (iv) and (v) use eq. \eqref{eq: 8b}, \red{and (v) uses $L_G=L_2(1+\kappa)^2\le 4L_2\kappa^2$, $L_{\Phi}=L_2(1+\kappa)^3\le 8L_2\kappa^3$.} 
    %$\nabla_1 f(x_t, y_{t+1})+G(x_t, y_{t+1})(x_{t+1}-x_t) + \frac{\eta_x}{2}\|x_{t+1}-x_t\| (x_{t+1}-x_t) =0$

%\begin{align}
%	\|y_{t+1} - y^*(x_{t}) \| \le&  (1-\kappa^{-1})^{N_t/2}\|y_{t} - y^*(x_{t})\|\\ %\label{eq: 8} \\
%	\le& \|x_t-x_{t-1}\|^2 %\label{eq: 8b}
%\end{align}

    Next, we prove the convergence of the sequence $\{x_t\}_t$ under the assumption that $H(x,x',y)$ satisfies the {\L}ojasiewicz gradient geometry. 
    Recall that we have shown in the proof of \Cref{thm: 1} that: 1) $\{H_t\}_t$ decreases monotonically to the finite limit $H^*$; 2) for any limit point $x^*, y^*$ of $\{x_t\}_t, \{y_t\}_t$, $\Phi(x^*)=H^*$. Hence, the {\L}ojasiewicz gradient inequality (see \Cref{def: KL}) holds after sufficiently large number of iterations, i.e., there exists $t_1\in \mathbb{N}^+$ such that for all $t\ge t_1$, $H(x_t,x_{t-1},y_{t+1})-H^*\le c\|\nabla H(x_t,x_{t-1},y_{t+1})\|^{\theta}$. Equivalently,
    \begin{align}
    	\varphi'(H_t -H^*) \|\nabla H(x_t,x_{t-1},y_{t+1})\|\ge 1. \nonumber
    \end{align}
    where we define the concave function that $\varphi(s):=\frac{c^{1/\theta}}{1-1/\theta}s^{1-1/\theta} (\theta>1, s>0)$. 
    
    In addition, since $\|x_t-x_{t-1}\|\stackrel{t}{\to} 0$ (Proposition \ref{prop: lyapunov}), there exists $t_2\in\mathbb{N}^{+}$ such that for all $t\ge t_2$, $\|x_t-x_{t-1}\|\le 1$. Hence, rearranging the above inequality and utilizing \cref{eq: 12}, we obtain that for all $t\ge t_0:=\max(t_1,t_2)$, 
    \begin{align}
    	&\varphi'(H_t -H^*) \nonumber\\
    	&\ge \|\nabla H(x_t,x_{t-1},y_{t+1})\|^{-1} \nonumber\\
    	&\ge \Big[\Big(\red{\frac{4L_2^2\kappa^2}{L_1}+L_2}\Big)\|x_{t-1}-x_{t-2}\|^2 + \Big(\red{10L_2\kappa^3 + \frac{24 L_2^3\kappa}{L_1^2}}+\frac{1}{2\eta_x}\Big) \|x_t-x_{t-1}\|^2 \Big]^{-1}\label{eq: 13}
    \end{align}
    
    By concavity of the function $\varphi(s):=\frac{c^{1/\theta}}{1-1/\theta}s^{1-1/\theta} (\theta>1, s>0)$, we know that 
    \begin{align}
    	&\varphi(H_t -H^*) - \varphi(H_{t+1} -H^*) \nonumber\\
    	&\ge \varphi'(H_t -H^*) (H_t - H_{t+1}) \nonumber\\
    	&\stackrel{(i)}{\ge} \frac{\red{L_2\kappa^3} \|x_{t+1}-x_t\|^3}{\Big(\red{\frac{4L_2^2\kappa^2}{L_1}+L_2}\Big)\|x_{t-1}-x_{t-2}\|^2 + \Big(\red{10L_2\kappa^3 + \frac{24 L_2^3\kappa}{L_1^2}}+\frac{1}{2\eta_x}\Big) \|x_t-x_{t-1}\|^2} \label{eq: phidiff}\\
    	&\stackrel{(ii)}{\ge} \frac{\red{L_2\kappa^3} \|x_{t+1}-x_t\|^3}{\Big(\sqrt{\red{\frac{4L_2^2\kappa^2}{L_1}+L_2}}\|x_{t-1}-x_{t-2}\| + \sqrt{\red{10L_2\kappa^3 + \frac{24 L_2^3\kappa}{L_1^2}}+\frac{1}{2\eta_x}} \|x_t-x_{t-1}\|\Big)^2}, \nonumber
    \end{align}
    where (i) uses \Cref{prop: lyapunov} and \cref{eq: 13}, (ii) uses the inequality that $a^2+b^2\le (a+b)^2$ for any $a,b\ge 0$. 
    
    Rearranging the above inequality yields that
    \begin{align}
        &\red{L_2\kappa^3} \|x_{t+1}-x_t\|^3  \nonumber\\
        &\le [\varphi(H_t -H^*) - \varphi(H_{t+1} -H^*)]\nonumber\\ 
        &\quad \Bigg(\sqrt{\red{\frac{4L_2^2\kappa^2}{L_1}+L_2}}\|x_{t-1}-x_{t-2}\| + \sqrt{\red{10L_2\kappa^3 + \frac{24 L_2^3\kappa}{L_1^2}}+\frac{1}{2\eta_x}} \|x_t-x_{t-1}\|\Bigg)^2 \nonumber\\
        &\le \frac{1}{27}\Bigg(C^2[\varphi(H_t -H^*) - \varphi(H_{t+1} -H^*)]+\frac{2}{C}\sqrt{\red{\frac{4L_2^2\kappa^2}{L_1}+L_2}}\|x_{t-1}-x_{t-2}\|  \nonumber\\
        &\quad +\frac{2}{C}\sqrt{\red{10L_2\kappa^3 + \frac{24 L_2^3\kappa}{L_1^2}}+\frac{1}{2\eta_x}} \|x_t-x_{t-1}\|\Bigg)^3
    \end{align}
    where the final step uses the AM-GM inequality that $ab^2=\big[\sqrt[3]{(C^2a)(b/C)(b/C)}\big]^3\le \frac{1}{27}(C^2a+\frac{2b}{C})^3$ for any $a,b\ge 0$ and $C>0$ (the value of $C$ will be assigned later). Taking cubic root of both sides of the above inequality and telescoping it over {$t=t_0,\ldots,T-1$}, we obtain that
    \begin{align}
    	&\red{\kappa\sqrt[3]{L_2}}\sum_{t=t_0}^{T-1}\|x_{t+1}-x_t\|\nonumber\\
    	&\le \frac{C^2}{3}[\varphi(H_{t_0} -H^*) - \varphi(H_T -H^*)]+\frac{2}{3C}\sqrt{\red{\frac{4L_2^2\kappa^2}{L_1}+L_2}}\sum_{t=t_0}^{T-1}\|x_{t-1}-x_{t-2}\| \nonumber\\
        &\quad + \frac{2}{3C}\sqrt{\red{10L_2\kappa^3 + \frac{24 L_2^3\kappa}{L_1^2}}+\frac{1}{2\eta_x}} \sum_{t=t_0}^{T-1}\|x_t-x_{t-1}\|\nonumber\\
    	&\le \frac{C^2}{3}\varphi(H_{t_0} -H^*) + \frac{2}{3C}\sqrt{\red{\frac{4L_2^2\kappa^2}{L_1}+L_2}}\sum_{t=t_0}^{T-1}\|x_{t-1}-x_{t-2}\| \nonumber\\
        &\quad + \frac{2}{3C}\sqrt{\red{10L_2\kappa^3 + \frac{24 L_2^3\kappa}{L_1^2}}+\frac{1}{2\eta_x}} \sum_{t=t_0}^{T-1}\|x_t-x_{t-1}\|\nonumber
    \end{align}
    where the final step uses the facts that $H_t-H^*\ge 0$ and that $\varphi(s)$ is monotonically increasing. Since the value of $C>0$ is arbitrary, we can select large enough $C$ such that $\frac{2}{3C}\sqrt{\red{\frac{4L_2^2\kappa^2}{L_1}+L_2}}, \frac{2}{3C}\sqrt{\red{10L_2\kappa^3 + \frac{24 L_2^3\kappa}{L_1^2}}+\frac{1}{2\eta_x}}<\frac{\red{\kappa\sqrt[3]{L_2}}}{3}$. Hence, the inequality above further implies that
    \begin{align}
        \frac{\red{\kappa\sqrt[3]{L_2}}}{3}\sum_{t=t_0}^{T-1}\|x_{t+1}-x_t\| \le& \frac{C^2}{3}\varphi(H_{t_0} -H^*) \nonumber\\
        & +\frac{\red{\kappa\sqrt[3]{L_2}}}{3} \big[\|x_{t_0-1}-x_{t_0-2}\|+2\|x_{t_0}-x_{t_0-1}\|\big] < +\infty. \label{eq: sum_dx_upperbound}
    \end{align}
    Letting $T\to\infty$ concludes that
    $$\sum_{t=1}^{\infty}\|x_{t+1} - x_t\| {<} +\infty.$$ 
    Moreover, this implies that $\{x_t\}_t$ is a Cauchy sequence and therefore converges to a certain limit, i.e., $x_t \overset{t}{\to} x^*$. We have shown in \Cref{thm: 1} that any such limit point must be a second-order critical point of $\Phi$. Hence, we conclude that $\{x_t\}_t$ converges to a certain second-order critical point $x^*$ of $\Phi(x)$. Also, note that $\|y^*(x_{t})-y_{t}\| \overset{t}{\to} 0$, $x_t\overset{t}{\to} x^*$ and $y^*$ is a Lipschitz mapping, so we conclude that $\{y_t\}_t$ converges to $y^*(x^*)$.  Finally, the item \ref{item: 2ndCritical} of \Cref{thm: 1} implies that $x^*$ is a second-order critical point of $\Phi(x)$. 
\end{proof}


==> thm3proof.tex <==
\section{Proof of \Cref{thm: 3}} \label{sec_thm3proof}

\thmconvrate*

\begin{proof}
    We redefine the potential function $H(x,x')=\Phi(x)+(L_{\Phi}+2\alpha+3\beta)\|x-x'\|^3$ to make the dependence on $x,x'$ explicit. Then, the potential function in \Cref{prop: lyapunov} can be rewritten as $H_t=H(x_t, x_{t-1})$. 
    Recall that we have shown in the proof of \Cref{thm: 1} that: 1) $\{H_t\}_t$ decreases monotonically to the finite limit $H^*$; 2) for any limit point $x^*, y^*$ of $\{x_t\}_t, \{y_t\}_t$, $\Phi(x^*)=H^*$. Hence, the {\L}ojasiewicz gradient inequality (see \Cref{def: KL}) holds after sufficiently large number of iterations, i.e., there exists $t_0\in \mathbb{N}^+$ such that for all $t\ge t_0$, $H(x_t,x_{t-1})-H^*\le c\|\nabla H(x_t,x_{t-1})\|^{\theta}$. By denoting $d_t=H(x_t,x_{t-1})-H^*=H_t-H^*$, this inequality implies that
    \begin{align}
    &c^{-1/\theta}d_t^{1/\theta} \nonumber\\
    &\le \|\nabla H(x_t,x_{t-1})\| \nonumber\\
    &\le \|\nabla_1 H(x_t,x_{t-1})\| + \|\nabla_2 H(x_t,x_{t-1})\| \nonumber\\
    &\le \Big\|\nabla \Phi(x_t)+3(L_{\Phi}+2\alpha+3\beta)\|x_t-x_{t-1}\|(x_t-x_{t-1})\Big\| + \big\|3(L_{\Phi}+2\alpha+3\beta)\|x_t-x_{t-1}\|(x_t-x_{t-1})\big\| \nonumber\\
    &\le \|\nabla \Phi(x_t)\| +6(L_{\Phi}+2\alpha+3\beta)\|s_t\|^2 \nonumber\\
    &\overset{(i)}{=}\Big\|\nabla \Phi(x_{t})-\nabla f(x_{t-1},y_{t}) -G(x_{t-1},y_{t}) s_{t} -\frac{1}{2\eta_x}\|s_{t}\|s_{t}\Big\| + 6(L_{\Phi}+2\alpha+3\beta)\|s_t\|^2 \nonumber\\
    &\le \|\nabla \Phi(x_{t})-\nabla \Phi(x_{t-1})-\nabla^2 \Phi(x_{t-1})s_{t}\| + \|\nabla \Phi(x_{t-1})-\nabla f(x_{t-1},y_{t})\|\nonumber\\
    &\quad + \|\nabla^2 \Phi(x_{t-1})s_{t}-G(x_{t-1},y_{t}) s_{t}\| + \frac{1}{2\eta_x}\|s_{t}\|^2 +6(L_{\Phi}+2\alpha+3\beta)\|s_t\|^2 \nonumber\\
    &\overset{(ii)}{\le} \Big(7L_{\Phi}+12\alpha+18\beta+\frac{1}{2\eta_x}\Big)\|s_{t}\|^2  +\beta\|s_{t-1}\|^2 +\alpha\|s_{t-1}\|\|s_{t}\| \nonumber\\
    &\overset{(iii)}{\le} \Big(7L_{\Phi}+13\alpha+18\beta+\frac{1}{2\eta_x}\Big)\|s_{t}\|^2  +(\alpha+\beta)\|s_{t-1}\|^2\nonumber\\
    &\le \Big(7L_{\Phi}+13\alpha+18\beta+\frac{1}{2\eta_x}\Big)\big(\|s_{t}\|^2+\|s_{t-1}\|^2\big)\nonumber\\
    &\overset{(iv)}{\le} (14L_{\Phi}+26\alpha+36\beta+\frac{1}{\eta_x}\Big) (\|s_{t}\|^3+\|s_{t-1}\|^3)^{2/3} \nonumber\\
    &\overset{(v)}{\le} \frac{14L_{\Phi}+26\alpha+36\beta+1/\eta_x}{(L_{\Phi}+\alpha+\beta)^{2/3}} (H_{t-1}-H_t)^{2/3}.\nonumber\\
    &=\frac{14L_{\Phi}+26\alpha+36\beta+1/\eta_x}{(L_{\Phi}+\alpha+\beta)^{2/3}} (d_{t-1}-d_t)^{2/3}. \nonumber
    \end{align}
    where (i) uses eq. \eqref{eq: CRcond1}, (ii) uses eqs. \eqref{eq: dfKL} \& \eqref{eq: dGKL} and the item \ref{item: ddPhi} of \Cref{prop_Phiystar} that $\nabla^2\Phi$ is $L_{\Phi}$-Lipschitz, (iii) uses $ab\le (a^2+b^2)/2$ for all $a,b\ge 0$, (iv) uses $a^2+b^2 \le 2(a^3+b^3)^{2/3}$ for all $a,b\ge 0$, (v) uses Proposition \ref{prop: lyapunov}. The above inequality can be rearranged as follows.
    \begin{align}
        d_{t-1}\ge d_t+Cd_t^{\frac{3}{2\theta}} \label{eq: 16} 
    \end{align}
    where $C=\frac{L_{\Phi}+\alpha+\beta}{c^{\frac{3}{2\theta}}(14L_{\Phi}+26\alpha+36\beta+1/\eta_x)^{3/2}}$. 
    
    Next, we prove the convergence rates case by case.
    
    (Case 1) If $\theta\in (\frac{3}{2}, +\infty)$, since $d_t \ge 0$, eq. \eqref{eq: 16} implies that for $t\ge t_0$,
    \begin{align}
        d_{t-1}\ge Cd_t^{\frac{3}{2\theta}},\nonumber
    \end{align}
    which is equivalent to that
    \begin{align}
    	C^{-\frac{2\theta}{2\theta-3}}d_t\le \big(C^{-\frac{2\theta}{2\theta-3}}d_{t-1}\big)^{2\theta/3} \label{eq: HdecSuper}
    \end{align}
    
    Since $d_t\downarrow 0$, $C^{-\frac{3\theta}{2\theta-3}}d_{t_0} \le e^{-1}$ for sufficiently large $t_0\in \mathbb{N}^+$. Hence, eq. \eqref{eq: HdecSuper} implies that for any $k\in\mathbb{N}^+$
    \begin{align}
    	C^{-\frac{3\theta}{2\theta-3}}d_{t}\le& \big[C^{-\frac{3\theta}{2\theta-3}}d_{t_0}\big]^{[(2\theta/3)^{t-t_0}]} \le \exp\Big[-\Big(\frac{2\theta}{3}\Big)^{t-t_0}\Big].\nonumber
    \end{align}
    Note that $\theta\in (\frac{3}{2}, +\infty)$ implies that $\frac{2\theta}{3}>1$, and thus the above inequality implies that $d_t\downarrow 0$ (i.e., $H(z_t) \downarrow H^*$) at the super-linear rate given by eq. \eqref{eq: HsuperConverge}. 

    (Case 2) If $\theta=\frac{3}{2}$, eq. \eqref{eq: 16} implies that for $t\ge t_0$,
    \begin{align}
        d_{t-1}\ge (1+C)d_t.\label{eq: HdecLinear}
    \end{align}
    Note that $d_{t_0}\le 1$ for sufficiently large $t_0$. Therefore, $d_t\downarrow 0$ (i.e., $H(z_t) \downarrow H^*$) at the linear rate given by eq. \eqref{eq: HlinearConverge}. 

    (Case 3) If $\theta\in (1, \frac{3}{2})$, consider the following two subcases.
    
    If $d_{t-1}\le 2d_t$, denote $\psi(s)=\frac{2\theta}{3-2\theta}s^{1-\frac{3}{2\theta}}$, then for any $t\ge t_0$,
    \begin{align}
    	\psi(d_t)-\psi(d_{t-1})=&\int_{d_{t}}^{d_{t-1}} -\psi'(s)ds = \int_{d_{t}}^{d_{t-1}} s^{-\frac{3}{2\theta}}ds \stackrel{(i)}{\ge} d_{t-1}^{-\frac{3}{2\theta}} (d_{t-1}-d_t) \nonumber\\
    	\stackrel{(ii)}{\ge}& C \Big(\frac{d_t}{d_{t-1}}\Big)^{\frac{3}{2\theta}} \stackrel{(iii)}{\ge} 2^{-\frac{3}{2}}C \ge \frac{C}{4} \label{eq: subcase1}
    \end{align}
    where (i) uses $d_t\le d_{t-1}$ and $-\frac{3}{2}\theta<0$, (ii) uses eq. \eqref{eq: 16}, and (iii) uses $\frac{d_t}{d_{t-1}} \ge \frac{1}{2}$ and $\frac{3}{2\theta}\in \big(1,\frac{3}{2}\big)$. 
    
    If $d_{t-1}>2d_t$, then for any $t\ge t_0$,
    \begin{align}
    	\psi(d_t)-\psi(d_{t-1})=&\frac{2\theta}{3-2\theta}(d_t^{1-\frac{3}{2\theta}}-d_{t-1}^{1-\frac{3}{2\theta}}) \stackrel{(i)}{\ge} \frac{2\theta}{3-2\theta}\big[d_t^{1-\frac{3}{2\theta}}-(2d_t)^{1-\frac{3}{2\theta}}\big] \nonumber\\
    	\ge& \frac{2\theta\big(1-2^{1-\frac{3}{2\theta}}\big)}{3-2\theta} d_t^{1-\frac{3}{2\theta}} \stackrel{(ii)}{\ge} \frac{C}{4}. \label{eq: subcase2}
    \end{align}
    where (i) uses $d_{t-1}>2d_t$ and $1-\frac{3}{2\theta}\in \big(-\frac{1}{2},0\big)$, $\frac{2\theta}{3-2\theta}>0$, and (ii) uses $1-\frac{3}{2\theta}\in \big(-\frac{1}{2},0\big)$ and $d_t\le d_{t_0} \le \Big(\frac{8\theta\big(1-2^{1-\frac{3}{2\theta}}\big)}{C(3-2\theta)}\Big)^{\frac{2\theta}{3-2\theta}}$ for sufficiently large $t_0\in\mathbb{N}^+$. 

Since at least one of eqs. \eqref{eq: subcase1} \& \eqref{eq: subcase2} holds, we have $\psi(d_t) \ge \psi(d_{t_0})+C(t-t_0)/4 \ge C(t-t_0)/4$. By substituting the definition of $\psi$, this inequality implies that $d_t\downarrow 0$ (i.e., $H(z_t) \downarrow H^*$) in a sub-linear rate given by eq. \eqref{eq: HsubConverge}. 
\end{proof}


==> thm4proof.tex <==
\section{Convergence Rate of SGA} \label{sec_thm4proof}
The following high-probability convergence rate of SGA is a direct application of the Theorem 3.1 of \cite{harvey2019simple}.

\begin{restatable}{thm}{lemmaSGA}\label{lemma: SGA}
    Let Assumption \ref{assum: fi} hold. For all $t,k$, assume that $\|\nabla_2 f(x_t,\widetilde{y}_k)\|\le L_0$ and $\|\widehat{\nabla}_2 f(x_t,\widetilde{y}_k)-\nabla_2 f(x_t,\widetilde{y}_k)\|\le 1$ almost surely.
    The inner stochastic gradient ascent steps in \Cref{algo: prox-minimax-stoc} converges at the following rate with probability at least $1-\delta$.
    \begin{align}
        \|y_{t+1}-y^*(x_t)\|\le \mathcal{O}\Big(\sqrt\frac{L_0\ln(1/\delta)+L_0^2}{\mu^2 N_t}\Big).\nonumber
    \end{align}
\end{restatable}

\begin{proof}
    Based on Theorem 3.1 of \cite{harvey2019simple}, the inner SGA steps in Algorithm \ref{algo: prox-minimax-stoc} has the following convergence rate with probability at least $1-\delta$.
    \begin{align}
        f(x_t,y^*(x_t))-f(x_t,y_{t+1})\le \mathcal{O}\Big(\frac{L_0\ln(1/\delta)+L_0^2}{\mu N_t}\Big),
    \end{align}
    which by $\mu$-strong concavity of $f(x_t,\cdot)$ proves the following convergence rate.
    \begin{align}
        \|y_{t+1}-y^*(x_t)\|\le \sqrt{2\big(f(x_t,y^*(x_t))-f(x_t,y_{t+1})\big)/\mu} \le \mathcal{O}\Big(\sqrt\frac{L_0\ln(1/\delta)+L_0^2}{\mu^2 N_t}\Big).\nonumber
    \end{align}
\end{proof}

==> thm5proof.tex <==
\section{Proof of \Cref{thm: 5}} \label{sec_thm5proof}
\thmstoc*

\begin{proof}
    In Lemma \ref{lemma: batch}, replace $x, y$ with $x_t, y_t$, $B_1$ with $B_1(t)$, and $B_{k,\ell}$ with $B_{k,\ell}(t)$ for any $k,\ell\in\{1,2\}$, and substitute the following hyperparameters.
    \begin{align}
        \epsilon_1(t)=&\frac{L_{\Phi}}{2}\Big(\|s_t\|^2+\frac{\epsilon^2}{33L_{\Phi}}\Big)\wedge 2L_0=\mathcal{O}(L_{\Phi}\|s_t\|^2+\epsilon^2), \nonumber\\
        \epsilon_2(t)=&\frac{L_{\Phi}}{2(\kappa+1)^2}\Big(\|s_t\|+\frac{\epsilon}{\sqrt{33L_{\Phi}}}\Big)\wedge 4L_1=\mathcal{O}\big(\kappa^{-2}(L_{\Phi}\|s_t\|+\sqrt{L_{\Phi}}\epsilon)\big). \nonumber
    \end{align}
    Then, we obtain that using the following batchsizes 
    \begin{align}
        \left\{ \begin{gathered}
           |B_1(t)|\ge \mathcal{O}\Big(\frac{L_0^2}{(L_{\Phi}^2\|s_t\|^4 + \epsilon^4)}\ln\frac{m}{\delta}\Big) \hfill \\
           |B_{k,\ell}(t)|\ge \mathcal{O}\Big(\frac{L_1^2\kappa^4}{L_{\Phi}(L_{\Phi}\|s_t\|^2 + \epsilon^2)}\ln\frac{m+n}{\delta}\Big) \hfill 
        \end{gathered}  \right.,\label{eq: batchsizes}
    \end{align}
    the stochastic approximators satisfy the following error bounds with probability at least $1-\delta$.
    \begin{align}
        \|\widehat{\nabla}_1 f(x_t,y_t)-\nabla_1 f(x_t,y_t)\|&\le \epsilon_1(t) \le\frac{L_{\Phi}}{2}\Big(\|s_t\|^2+\frac{\epsilon^2}{33L_{\Phi}}\Big),\label{eq: stoc_err1_detail}\\ 
        \|\widehat{G}(x_t,y_t)-G(x_t,y_t)\|&\le  \epsilon_2(t)\le \frac{L_{\Phi}}{2}\Big(\|s_t\|+\frac{\epsilon}{\sqrt{33L_{\Phi}}}\Big).\label{eq: stoc_err3_detail}
    \end{align}
    Based on Theorem \ref{lemma: SGA}, using the following number of stochastic gradient ascent steps
    \begin{align}
        N_t&\ge \mathcal{O}\Big(\frac{L_0\ln(1/\delta)+L_0^2}{\mu^2L_{\Phi}^2\big(([\|s_t\|^2+\epsilon^2/(33L_{\Phi})]/L_1) \wedge ([\|s_t\|+\epsilon/\sqrt{33L_{\Phi}}]/L_G)\big)^2}\Big)\nonumber\\
        &\overset{(i)}{=}\mathcal{O}\Big(\frac{L_0\ln(1/\delta)+L_0^2}{\big(([L_{\Phi}\|s_t\|^2+\epsilon^2]/\kappa)\wedge L_1(\|s_t\|+\epsilon/\sqrt{L_{\Phi}})\big)^2}\Big)\nonumber\\
        &=\mathcal{O}\Big(\frac{L_0\ln(1/\delta)+L_0^2}{\kappa^{-2}(L_{\Phi}^2\|s_t\|^4+\epsilon^4)\wedge L_1^2(\|s_t\|^2+\epsilon^2/L_{\Phi})}\Big), \label{eq: Ntstoc}
    \end{align} 
    where (i) uses $\kappa=L_1/\mu$ and $L_{\Phi}=L_G(1+\kappa)$ (\Cref{prop_Phiystar}). 
    we have
    \begin{align}
        \|y_{t+1}-y^*(x_t)\|\le \mathcal{O}\Big(\sqrt\frac{L_0\ln(1/\delta)+L_0^2}{\mu^2 N_t}\Big)\le \frac{L_{\Phi}}{2}\min\Big(\frac{1}{L_1}\Big(\|s_t\|^2+\frac{\epsilon^2}{33L_{\Phi}}\Big), \frac{1}{L_G}\Big(\|s_t\|+\frac{\epsilon}{\sqrt{33L_{\Phi}}}\Big)\Big). \label{eq: yerr_stoc}
    \end{align}
    Therefore, 
    \begin{align}
        &\|\nabla\Phi(x_t)-\widehat{\nabla}_1 f(x_t, y_{t+1})\|\nonumber\\
        &\overset{(i)}{\le}\|\nabla_1 f(x_t,y^*(x_t))-\nabla_1 f(x_t, y_{t+1})\|+\|\widehat{\nabla}_1 f(x_t, y_{t+1})-\nabla_1 f(x_t, y_{t+1})\|\nonumber\\
        &\overset{(ii)}{\le} L_1\|y_{t+1}-y^*(x_t)\| + \frac{L_{\Phi}}{2}\Big(\|s_t\|^2+\frac{\epsilon^2}{33L_{\Phi}}\Big) \nonumber\\
        &\overset{(iii)}{\le} L_{\Phi}\Big(\|s_t\|^2+\frac{\epsilon^2}{33L_{\Phi}}\Big),\label{eq: dfstoc}
    \end{align}
    where (i) uses $\nabla\Phi(x)=\nabla_1 f(x,y^*(x))$ in \Cref{prop_1}, (ii) uses eq. \eqref{eq: stoc_err1_detail} and \Cref{assum: f}, and (iii) uses eq. \eqref{eq: yerr_stoc}. 
    \begin{align}
        &\|\nabla^2\Phi(x_t)-\widehat{G}(x_t,y_{t+1})\|\nonumber\\
        &\overset{(i)}{\le}\|G(x_t,y^*(x_t))-G(x_t,y_{t+1})\|+\|\widehat{G}(x_t,y_{t+1})-G(x_t,y_{t+1})\|\nonumber\\
        &\overset{(ii)}{\le} L_G\|y_{t+1}-y^*(x_t)\| + \frac{L_{\Phi}}{2}\Big(\|s_t\|+\frac{\epsilon}{\sqrt{33L_{\Phi}}}\Big) \nonumber\\
        &\overset{(iii)}{\le} L_{\Phi}\Big(\|s_t\|+\frac{\epsilon}{\sqrt{33L_{\Phi}}}\Big),\label{eq: dGstoc}
    \end{align}
    where (i) uses $\nabla^2\Phi(x)=G(x,y^*(x))$ in \Cref{prop_Phiystar}, (ii) uses eq. \eqref{eq: stoc_err3_detail} and the item \ref{item: G_lipschitz} of \Cref{prop_Phiystar}, and (iii) uses eq. \eqref{eq: yerr_stoc}. Eqs. \eqref{eq: dfstoc} \& \eqref{eq: dGstoc} imply that the conditions \eqref{eq: grad_goal_noKL} \& \eqref{eq: Hess_goal_noKL} hold with $\alpha=\beta=L_{\Phi}=L_2(1+\kappa)^3$ and $\epsilon'=\frac{\epsilon}{\sqrt{33L_{\Phi}}}$. In Lemma \ref{lemma_general_rate}, by substituting these values of $\alpha$, $\beta$, $\epsilon'$ and $\eta_x=(55L_{\Phi})^{-1}$, we obtain that when $T\ge \frac{\Phi(x_0)-\Phi^*+8L_{\Phi}\epsilon'^2}{3L_{\Phi}\epsilon'^3}$,  we have $T'\le \sqrt{33L_{\Phi}}\frac{33(\Phi(x_0)-\Phi^*)+8\epsilon^2}{3\epsilon^3}=\mathcal{O}\big(\sqrt{L_2}\kappa^{1.5}\epsilon^{-3}\big)\le T$, and moreover,
    \begin{align}
        &\|\nabla \Phi(x_{T'})\| \le \Big(\frac{1}{2\eta_x}+L_{\Phi}+2\alpha+2\beta\Big) \epsilon'^2 \le \epsilon^2, \nonumber\\
        &\lambda_{\min}\big(\nabla^2 \Phi(x_{T'})\big) \ge -\Big(\frac{1}{2\eta_x}+L_{\Phi}+2\alpha\Big)\epsilon' \overset{(i)}{\ge} -\sqrt{33L_{\Phi}}\epsilon, \nonumber
    \end{align}
    This proves that eq. \eqref{eq: gH_rate2} holds with probability at least $1-\delta$. 
    
    Choosing both $N_t$ in eq. \eqref{eq: Ntstoc} and the batchsizes in eq. \eqref{eq: batchsizes} with equality, the number of gradient computations has the following upper bound. 
    \begin{align}
        &\sum_{t=0}^{T'-1} \big(N_t+|B_1(t)|\big)\nonumber\\
        &=\sum_{t=0}^{T'-1}\mathcal{O} \Big( \frac{L_0\ln(1/\delta)+L_0^2}{\kappa^{-2}(L_{\Phi}^2\|s_t\|^4+\epsilon^4)\wedge L_1^2(\|s_t\|^2+\epsilon^2/L_{\Phi})} + \frac{L_0^2}{L_{\Phi}^2\|s_t\|^4 + \epsilon^4}\ln\frac{m}{\delta}\Big) \nonumber\\
        &\le \sum_{t=0}^{T'-1}\mathcal{O} \Big( \frac{L_0\ln(1/\delta)+L_0^2}{\epsilon^4\kappa^{-2}\wedge L_1^2\epsilon^2/L_{\Phi}} + \frac{L_0^2}{\epsilon^4}\ln\frac{m}{\delta}\Big) \nonumber\\
        &\overset{(i)}{\le} 
        T'\mathcal{O}\Big(\frac{L_0\kappa^2}{\epsilon^4}\big(\ln(1/\delta)+L_0\big) + \frac{L_0^2}{\epsilon^4}\ln\frac{m}{\delta}\Big) \nonumber\\
        &\overset{(ii)}{\le} \mathcal{O}\big(\sqrt{L_2}\kappa^{1.5}\epsilon^{-3}\big) \mathcal{O}\Big(\frac{L_0^2\kappa^2}{\epsilon^4}\ln\frac{m}{\delta}\Big) \nonumber\\
        &\le \mathcal{O}\Big(\frac{L_0^2\kappa^{3.5}\sqrt{L_2}}{\epsilon^7}\ln\frac{m}{\delta}\Big)
    \end{align}
    where (i) uses $\epsilon'=\frac{\epsilon}{\sqrt{33L_{\Phi}}}\le \frac{L_1}{L_G}=\frac{L_1(1+\kappa)}{L_{\Phi}}$ which implies that $\epsilon^4\kappa^{-2} \le \mathcal{O}(L_1^2\epsilon^2/L_{\Phi})$, (ii) uses $T'\le\mathcal{O}\big(\sqrt{L_2}\kappa^{1.5}\epsilon^{-3}\big)$ we proved above. The number of Hessian computations has the following upper bound.
    \begin{align}
        &\sum_{t=0}^{T'-1} \sum_{k=1}^2\sum_{\ell=1}^2|B_{k,\ell}(t)|\nonumber\\
        &=\sum_{t=0}^{T'-1}\mathcal{O} \Big(\frac{L_1^2\kappa^4}{L_{\Phi}(L_{\Phi}\|s_t\|^2 + \epsilon^2)}\ln\frac{m+n}{\delta}\Big) \nonumber\\
        &\le \sum_{t=0}^{T'-1}\mathcal{O} \Big(\frac{L_1^2\kappa^4}{L_{\Phi}\epsilon^2}\ln\frac{m+n}{\delta}\Big) \nonumber\\
        &\overset{(i)}{\le} 
        T'\mathcal{O}\Big( \frac{L_1^2\kappa}{L_2\epsilon^2}\ln\frac{m+n}{\delta}\Big) \nonumber\\
        &\overset{(ii)}{\le} \mathcal{O}\Big( \frac{L_1^2\kappa^{2.5}}{\sqrt{L_2}\epsilon^5}\ln\frac{m+n}{\delta}\Big)
    \end{align}
    where (i) uses $L_{\Phi}=L_2(1+\kappa)^3=\mathcal{O}(L_2\kappa^3)$, (ii) uses $T'\le \sqrt{33L_{\Phi}}\frac{33(\Phi(x_0)-\Phi^*)+8\epsilon^2}{3\epsilon^3}=\mathcal{O}\big(\sqrt{L_2}\kappa^{1.5}\epsilon^{-3}\big)$ we proved above. 
\end{proof}


